Skew Class-balanced Re-weighting for Unbiased Scene Graph Generation

An unbiased scene graph generation (SGG) algorithm referred to as Skew Class-balanced Re-weighting (SCR) is proposed for considering the unbiased predicate prediction caused by the long-tailed distribution. The prior works focus mainly on alleviating the deteriorating performances of the minority predicate predictions, showing drastic dropping recall scores, i.e., losing the majority predicate performances. It has not yet correctly analyzed the trade-off between majority and minority predicate performances in the limited SGG datasets. In this paper, to alleviate the issue, the Skew Class-balanced Re-weighting (SCR) loss function is considered for the unbiased SGG models. Leveraged by the skewness of biased predicate predictions, the SCR estimates the target predicate weight coefficient and then re-weights more to the biased predicates for better trading-off between the majority predicates and the minority ones. Extensive experiments conducted on the standard Visual Genome dataset and Open Image V4 \& V6 show the performances and generality of the SCR with the traditional SGG models.

==> Definitions/journalnames.tex <==
%%Updated on 17 November 2022
%,% Website Name,%,%,% Website Name,%%,% Full Name,%%,% Short Name,%%,% DOI abbr,%%,% ISSN,% \continuouspages
%\DeclareOption{}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{acoustics}{\gdef\@journal{acoustics}\gdef\@journalfull{Acoustics}\gdef\@journalshort{Acoustics}\gdef\@doiabbr{acoustics}\gdef\@ISSN{2624-599X}\gdef\@continuouspages{yes}}
\DeclareOption{actuators}{\gdef\@journal{actuators}\gdef\@journalfull{Actuators}\gdef\@journalshort{Actuators}\gdef\@doiabbr{act}\gdef\@ISSN{2076-0825}}
\DeclareOption{addictions}{\gdef\@journal{addictions}\gdef\@journalfull{Addictions}\gdef\@journalshort{Addictions}\gdef\@doiabbr{}\gdef\@ISSN{0006-0006}}
\DeclareOption{admsci}{\gdef\@journal{admsci}\gdef\@journalfull{Administrative Sciences}\gdef\@journalshort{Adm. Sci.}\gdef\@doiabbr{admsci}\gdef\@ISSN{2076-3387}}
\DeclareOption{adolescents}{\gdef\@journal{adolescents}\gdef\@journalfull{Adolescents}\gdef\@journalshort{Adolescents}\gdef\@doiabbr{adolescents}\gdef\@ISSN{2673-7051}\gdef\@continuouspages{yes}}
\DeclareOption{aerobiology}{\gdef\@journal{aerobiology}\gdef\@journalfull{Aerobiology}\gdef\@journalshort{Aerobiology}\gdef\@doiabbr{aerobiology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{aerospace}{\gdef\@journal{aerospace}\gdef\@journalfull{Aerospace}\gdef\@journalshort{Aerospace}\gdef\@doiabbr{aerospace}\gdef\@ISSN{2226-4310}}
\DeclareOption{agriculture}{\gdef\@journal{agriculture}\gdef\@journalfull{Agriculture}\gdef\@journalshort{Agriculture}\gdef\@doiabbr{agriculture}\gdef\@ISSN{2077-0472}}
\DeclareOption{agriengineering}{\gdef\@journal{agriengineering}\gdef\@journalfull{AgriEngineering}\gdef\@journalshort{AgriEngineering}\gdef\@doiabbr{agriengineering}\gdef\@ISSN{2624-7402}\gdef\@continuouspages{yes}}
\DeclareOption{agrochemicals}{\gdef\@journal{agrochemicals}\gdef\@journalfull{Agrochemicals}\gdef\@journalshort{Agrochemicals}\gdef\@doiabbr{agrochemicals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{agronomy}{\gdef\@journal{agronomy}\gdef\@journalfull{Agronomy}\gdef\@journalshort{Agronomy}\gdef\@doiabbr{agronomy}\gdef\@ISSN{2073-4395}}
\DeclareOption{ai}{\gdef\@journal{ai}\gdef\@journalfull{AI}\gdef\@journalshort{AI}\gdef\@doiabbr{ai}\gdef\@ISSN{2673-2688}\gdef\@continuouspages{yes}}
\DeclareOption{air}{\gdef\@journal{air}\gdef\@journalfull{Air}\gdef\@journalshort{Air}\gdef\@doiabbr{air}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{algorithms}{\gdef\@journal{algorithms}\gdef\@journalfull{Algorithms}\gdef\@journalshort{Algorithms}\gdef\@doiabbr{a}\gdef\@ISSN{1999-4893}}
\DeclareOption{allergies}{\gdef\@journal{allergies}\gdef\@journalfull{Allergies}\gdef\@journalshort{Allergies}\gdef\@doiabbr{allergies}\gdef\@ISSN{2313-5786}}
\DeclareOption{alloys}{\gdef\@journal{alloys}\gdef\@journalfull{Alloys}\gdef\@journalshort{Alloys}\gdef\@doiabbr{alloys}\gdef\@ISSN{2674-063X}\gdef\@continuouspages{yes}}
\DeclareOption{analytica}{\gdef\@journal{analytica}\gdef\@journalfull{Analytica}\gdef\@journalshort{Analytica}\gdef\@doiabbr{analytica}\gdef\@ISSN{2673-4532}\gdef\@continuouspages{yes}}
\DeclareOption{analytics}{\gdef\@journal{analytics}\gdef\@journalfull{Analytics}\gdef\@journalshort{Analytics}\gdef\@doiabbr{analytics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{anatomia}{\gdef\@journal{anatomia}\gdef\@journalfull{Anatomia}\gdef\@journalshort{Anatomia}\gdef\@doiabbr{anatomia}\gdef\@ISSN{2813-0545}\gdef\@continuouspages{yes}}
\DeclareOption{animals}{\gdef\@journal{animals}\gdef\@journalfull{Animals}\gdef\@journalshort{Animals}\gdef\@doiabbr{ani}\gdef\@ISSN{2076-2615}}
\DeclareOption{antibiotics}{\gdef\@journal{antibiotics}\gdef\@journalfull{Antibiotics}\gdef\@journalshort{Antibiotics}\gdef\@doiabbr{antibiotics}\gdef\@ISSN{2079-6382}}
\DeclareOption{antibodies}{\gdef\@journal{antibodies}\gdef\@journalfull{Antibodies}\gdef\@journalshort{Antibodies}\gdef\@doiabbr{antib}\gdef\@ISSN{2073-4468}}
\DeclareOption{antioxidants}{\gdef\@journal{antioxidants}\gdef\@journalfull{Antioxidants}\gdef\@journalshort{Antioxidants}\gdef\@doiabbr{antiox}\gdef\@ISSN{2076-3921}}
\DeclareOption{applbiosci}{\gdef\@journal{applbiosci}\gdef\@journalfull{Applied Biosciences}\gdef\@journalshort{Appl. Biosci.}\gdef\@doiabbr{applbiosci}\gdef\@ISSN{2813-0464}\gdef\@continuouspages{yes}}
\DeclareOption{appliedchem}{\gdef\@journal{appliedchem}\gdef\@journalfull{AppliedChem}\gdef\@journalshort{AppliedChem}\gdef\@doiabbr{appliedchem}\gdef\@ISSN{2673-9623}\gdef\@continuouspages{yes}}
\DeclareOption{appliedmath}{\gdef\@journal{appliedmath}\gdef\@journalfull{AppliedMath}\gdef\@journalshort{AppliedMath}\gdef\@doiabbr{appliedmath}\gdef\@ISSN{2673-9909}\gdef\@continuouspages{yes}}
\DeclareOption{applmech}{\gdef\@journal{applmech}\gdef\@journalfull{Applied Mechanics}\gdef\@journalshort{Appl. Mech.}\gdef\@doiabbr{applmech}\gdef\@ISSN{2673-3161}\gdef\@continuouspages{yes}}
\DeclareOption{applmicrobiol}{\gdef\@journal{applmicrobiol}\gdef\@journalfull{Applied Microbiology}\gdef\@journalshort{Appl. Microbiol.}\gdef\@doiabbr{applmicrobiol}\gdef\@ISSN{2673-8007}\gdef\@continuouspages{yes}}
\DeclareOption{applnano}{\gdef\@journal{applnano}\gdef\@journalfull{Applied Nano}\gdef\@journalshort{Appl. Nano}\gdef\@doiabbr{applnano}\gdef\@ISSN{2673-3501}\gdef\@continuouspages{yes}}
\DeclareOption{applsci}{\gdef\@journal{applsci}\gdef\@journalfull{Applied Sciences}\gdef\@journalshort{Appl. Sci.}\gdef\@doiabbr{app}\gdef\@ISSN{2076-3417}}
\DeclareOption{aquacj}{\gdef\@journal{aquacj}\gdef\@journalfull{Aquaculture Journal}\gdef\@journalshort{Aquac. J.}\gdef\@doiabbr{aj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{architecture}{\gdef\@journal{architecture}\gdef\@journalfull{Architecture}\gdef\@journalshort{Architecture}\gdef\@doiabbr{architecture}\gdef\@ISSN{2673-8945}\gdef\@continuouspages{yes}}
\DeclareOption{arm}{\gdef\@journal{arm}\gdef\@journalfull{Advances in Respiratory Medicine}\gdef\@journalshort{Adv. Respir. Med.}\gdef\@doiabbr{arm}\gdef\@ISSN{2543-6031}\gdef\@continuouspages{yes}}
\DeclareOption{arthropoda}{\gdef\@journal{arthropoda}\gdef\@journalfull{Arthropoda}\gdef\@journalshort{Arthropoda}\gdef\@doiabbr{arthropoda}\gdef\@ISSN{2813-3323}\gdef\@continuouspages{yes}}
\DeclareOption{arts}{\gdef\@journal{arts}\gdef\@journalfull{Arts}\gdef\@journalshort{Arts}\gdef\@doiabbr{arts}\gdef\@ISSN{2076-0752}}
\DeclareOption{asc}{\gdef\@journal{asc}\gdef\@journalfull{Automatic Systems and Control}\gdef\@journalshort{Autom. Syst. Control}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{asi}{\gdef\@journal{asi}\gdef\@journalfull{Applied System Innovation}\gdef\@journalshort{Appl. Syst. Innov.}\gdef\@doiabbr{asi}\gdef\@ISSN{2571-5577}}
\DeclareOption{astronomy}{\gdef\@journal{astronomy}\gdef\@journalfull{Astronomy}\gdef\@journalshort{Astronomy}\gdef\@doiabbr{astronomy}\gdef\@ISSN{2674-0346}\gdef\@continuouspages{yes}}
\DeclareOption{atmosphere}{\gdef\@journal{atmosphere}\gdef\@journalfull{Atmosphere}\gdef\@journalshort{Atmosphere}\gdef\@doiabbr{atmos}\gdef\@ISSN{2073-4433}}
\DeclareOption{atoms}{\gdef\@journal{atoms}\gdef\@journalfull{Atoms}\gdef\@journalshort{Atoms}\gdef\@doiabbr{atoms}\gdef\@ISSN{2218-2004}}
\DeclareOption{audiolres}{\gdef\@journal{audiolres}\gdef\@journalfull{Audiology Research}\gdef\@journalshort{Audiol. Res.}\gdef\@doiabbr{audiolres}\gdef\@ISSN{2039-4349}\gdef\@continuouspages{yes}}
\DeclareOption{automation}{\gdef\@journal{automation}\gdef\@journalfull{Automation}\gdef\@journalshort{Automation}\gdef\@doiabbr{automation}\gdef\@ISSN{2673-4052}\gdef\@continuouspages{yes}}
\DeclareOption{axioms}{\gdef\@journal{axioms}\gdef\@journalfull{Axioms}\gdef\@journalshort{Axioms}\gdef\@doiabbr{axioms}\gdef\@ISSN{2075-1680}}
\DeclareOption{bacteria}{\gdef\@journal{bacteria}\gdef\@journalfull{Bacteria}\gdef\@journalshort{Bacteria}\gdef\@doiabbr{bacteria}\gdef\@ISSN{2674-1334}\gdef\@continuouspages{yes}}
\DeclareOption{batteries}{\gdef\@journal{batteries}\gdef\@journalfull{Batteries}\gdef\@journalshort{Batteries}\gdef\@doiabbr{batteries}\gdef\@ISSN{2313-0105}}
\DeclareOption{bdcc}{\gdef\@journal{bdcc}\gdef\@journalfull{Big Data and Cognitive Computing}\gdef\@journalshort{Big Data Cogn. Comput.}\gdef\@doiabbr{bdcc}\gdef\@ISSN{2504-2289}}
\DeclareOption{behavsci}{\gdef\@journal{behavsci}\gdef\@journalfull{Behavioral Sciences}\gdef\@journalshort{Behav. Sci.}\gdef\@doiabbr{bs}\gdef\@ISSN{2076-328X}}
\DeclareOption{beverages}{\gdef\@journal{beverages}\gdef\@journalfull{Beverages}\gdef\@journalshort{Beverages}\gdef\@doiabbr{beverages}\gdef\@ISSN{2306-5710}}
\DeclareOption{biochem}{\gdef\@journal{biochem}\gdef\@journalfull{BioChem}\gdef\@journalshort{BioChem}\gdef\@doiabbr{biochem}\gdef\@ISSN{2673-6411}\gdef\@continuouspages{yes}}
\DeclareOption{bioengineering}{\gdef\@journal{bioengineering}\gdef\@journalfull{Bioengineering}\gdef\@journalshort{Bioengineering}\gdef\@doiabbr{bioengineering}\gdef\@ISSN{2306-5354}}
\DeclareOption{biologics}{\gdef\@journal{biologics}\gdef\@journalfull{Biologics}\gdef\@journalshort{Biologics}\gdef\@doiabbr{biologics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biology}{\gdef\@journal{biology}\gdef\@journalfull{Biology}\gdef\@journalshort{Biology}\gdef\@doiabbr{biology}\gdef\@ISSN{2079-7737}}
\DeclareOption{biomass}{\gdef\@journal{biomass}\gdef\@journalfull{Biomass}\gdef\@journalshort{Biomass}\gdef\@doiabbr{biomass}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomechanics}{\gdef\@journal{biomechanics}\gdef\@journalfull{Biomechanics}\gdef\@journalshort{Biomechanics}\gdef\@doiabbr{biomechanics}\gdef\@ISSN{2673-7078}\gdef\@continuouspages{yes}}
\DeclareOption{biomed}{\gdef\@journal{biomed}\gdef\@journalfull{BioMed}\gdef\@journalshort{BioMed}\gdef\@doiabbr{biomed}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomedicines}{\gdef\@journal{biomedicines}\gdef\@journalfull{Biomedicines}\gdef\@journalshort{Biomedicines}\gdef\@doiabbr{biomedicines}\gdef\@ISSN{2227-9059}}
\DeclareOption{biomedinformatics}{\gdef\@journal{biomedinformatics}\gdef\@journalfull{Biomedinformatics}\gdef\@journalshort{Biomedinformatics}\gdef\@doiabbr{biomedinformatics}\gdef\@ISSN{2673-7426}\gdef\@continuouspages{yes}}
\DeclareOption{biomimetics}{\gdef\@journal{biomimetics}\gdef\@journalfull{Biomimetics}\gdef\@journalshort{Biomimetics}\gdef\@doiabbr{biomimetics}\gdef\@ISSN{2313-7673}}
\DeclareOption{biomolecules}{\gdef\@journal{biomolecules}\gdef\@journalfull{Biomolecules}\gdef\@journalshort{Biomolecules}\gdef\@doiabbr{biom}\gdef\@ISSN{2218-273X}}
\DeclareOption{biophysica}{\gdef\@journal{biophysica}\gdef\@journalfull{Biophysica}\gdef\@journalshort{Biophysica}\gdef\@doiabbr{biophysica}\gdef\@ISSN{2673-4125}\gdef\@continuouspages{yes}}
\DeclareOption{biosensors}{\gdef\@journal{biosensors}\gdef\@journalfull{Biosensors}\gdef\@journalshort{Biosensors}\gdef\@doiabbr{bios}\gdef\@ISSN{2079-6374}}
\DeclareOption{biotech}{\gdef\@journal{biotech}\gdef\@journalfull{BioTech}\gdef\@journalshort{BioTech}\gdef\@doiabbr{biotech}\gdef\@ISSN{2673-6284}}
\DeclareOption{birds}{\gdef\@journal{birds}\gdef\@journalfull{Birds}\gdef\@journalshort{Birds}\gdef\@doiabbr{birds}\gdef\@ISSN{2673-6004}\gdef\@continuouspages{yes}}
\DeclareOption{bloods}{\gdef\@journal{bloods}\gdef\@journalfull{Bloods}\gdef\@journalshort{Bloods}\gdef\@doiabbr{bloods}\gdef\@ISSN{2673-415X}}
\DeclareOption{blsf}{\gdef\@journal{blsf}\gdef\@journalfull{Biology and Life Sciences Forum}\gdef\@journalshort{Biol. Life Sci. Forum}\gdef\@doiabbr{blsf	}\gdef\@ISSN{2673-9976}}
\DeclareOption{brainsci}{\gdef\@journal{brainsci}\gdef\@journalfull{Brain Sciences}\gdef\@journalshort{Brain Sci.}\gdef\@doiabbr{brainsci}\gdef\@ISSN{2076-3425}}
\DeclareOption{breath}{\gdef\@journal{breath}\gdef\@journalfull{Breath}\gdef\@journalshort{Breath}\gdef\@doiabbr{breath}\gdef\@ISSN{}}
\DeclareOption{buildings}{\gdef\@journal{buildings}\gdef\@journalfull{Buildings}\gdef\@journalshort{Buildings}\gdef\@doiabbr{buildings}\gdef\@ISSN{2075-5309}}
\DeclareOption{businesses}{\gdef\@journal{businesses}\gdef\@journalfull{Businesses}\gdef\@journalshort{Businesses}\gdef\@doiabbr{businesses}\gdef\@ISSN{2673-7116}\gdef\@continuouspages{yes}}
\DeclareOption{cancers}{\gdef\@journal{cancers}\gdef\@journalfull{Cancers}\gdef\@journalshort{Cancers}\gdef\@doiabbr{cancers}\gdef\@ISSN{2072-6694}}
\DeclareOption{carbon}{\gdef\@journal{carbon}\gdef\@journalfull{C}\gdef\@journalshort{C}\gdef\@doiabbr{c}\gdef\@ISSN{2311-5629}}
\DeclareOption{cardiogenetics}{\gdef\@journal{cardiogenetics}\gdef\@journalfull{Cardiogenetics}\gdef\@journalshort{Cardiogenetics}\gdef\@doiabbr{cardiogenetics}\gdef\@ISSN{2035-8148}\gdef\@continuouspages{yes}}
\DeclareOption{catalysts}{\gdef\@journal{catalysts}\gdef\@journalfull{Catalysts}\gdef\@journalshort{Catalysts}\gdef\@doiabbr{catal}\gdef\@ISSN{2073-4344}}
\DeclareOption{cells}{\gdef\@journal{cells}\gdef\@journalfull{Cells}\gdef\@journalshort{Cells}\gdef\@doiabbr{cells}\gdef\@ISSN{2073-4409}}
\DeclareOption{ceramics}{\gdef\@journal{ceramics}\gdef\@journalfull{Ceramics}\gdef\@journalshort{Ceramics}\gdef\@doiabbr{ceramics}\gdef\@ISSN{2571-6131}\gdef\@continuouspages{yes}}
\DeclareOption{challenges}{\gdef\@journal{challenges}\gdef\@journalfull{Challenges}\gdef\@journalshort{Challenges}\gdef\@doiabbr{challe}\gdef\@ISSN{2078-1547}}
\DeclareOption{chemengineering}{\gdef\@journal{chemengineering}\gdef\@journalfull{ChemEngineering}\gdef\@journalshort{ChemEngineering}\gdef\@doiabbr{chemengineering}\gdef\@ISSN{2305-7084}}
\DeclareOption{chemistry}{\gdef\@journal{chemistry}\gdef\@journalfull{Chemistry}\gdef\@journalshort{Chemistry}\gdef\@doiabbr{chemistry}\gdef\@ISSN{2624-8549}\gdef\@continuouspages{yes}}
\DeclareOption{chemosensors}{\gdef\@journal{chemosensors}\gdef\@journalfull{Chemosensors}\gdef\@journalshort{Chemosensors}\gdef\@doiabbr{chemosensors}\gdef\@ISSN{2227-9040}}
\DeclareOption{chemproc}{\gdef\@journal{chemproc}\gdef\@journalfull{Chemistry Proceedings}\gdef\@journalshort{Chem. Proc.}\gdef\@doiabbr{chemproc}\gdef\@ISSN{2673-4583}}
\DeclareOption{children}{\gdef\@journal{children}\gdef\@journalfull{Children}\gdef\@journalshort{Children}\gdef\@doiabbr{children}\gdef\@ISSN{2227-9067}}
\DeclareOption{chips}{\gdef\@journal{chips}\gdef\@journalfull{Chips}\gdef\@journalshort{Chips}\gdef\@doiabbr{chips}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{cimb}{\gdef\@journal{cimb}\gdef\@journalfull{Current Issues in Molecular Biology}\gdef\@journalshort{Curr. Issues Mol. Biol.}\gdef\@doiabbr{cimb}\gdef\@ISSN{1467-3045}\gdef\@continuouspages{yes}}
\DeclareOption{civileng}{\gdef\@journal{civileng}\gdef\@journalfull{CivilEng}\gdef\@journalshort{CivilEng}\gdef\@doiabbr{civileng}\gdef\@ISSN{2673-4109}\gdef\@continuouspages{yes}}
\DeclareOption{cleantechnol}{\gdef\@journal{cleantechnol}\gdef\@journalfull{Clean Technologies}\gdef\@journalshort{Clean Technol.}\gdef\@doiabbr{cleantechnol}\gdef\@ISSN{2571-8797}\gdef\@continuouspages{yes}}
\DeclareOption{climate}{\gdef\@journal{climate}\gdef\@journalfull{Climate}\gdef\@journalshort{Climate}\gdef\@doiabbr{cli}\gdef\@ISSN{2225-1154}}
\DeclareOption{clinpract}{\gdef\@journal{clinpract}\gdef\@journalfull{Clinics and Practice}\gdef\@journalshort{Clin. Pract.}\gdef\@doiabbr{clinpract}\gdef\@ISSN{2039-7283}\gdef\@continuouspages{yes}}
\DeclareOption{clockssleep}{\gdef\@journal{clockssleep}\gdef\@journalfull{Clocks \& Sleep}\gdef\@journalshort{Clocks\&Sleep}\gdef\@doiabbr{clockssleep}\gdef\@ISSN{2624-5175}\gdef\@continuouspages{yes}}
\DeclareOption{cmd}{\gdef\@journal{cmd}\gdef\@journalfull{Corrosion and Materials Degradation}\gdef\@journalshort{Corros. Mater. Degrad.}\gdef\@doiabbr{cmd}\gdef\@ISSN{2624-5558}\gdef\@continuouspages{yes}}
\DeclareOption{coasts}{\gdef\@journal{coasts}\gdef\@journalfull{Coasts}\gdef\@journalshort{Coasts}\gdef\@doiabbr{coasts}\gdef\@ISSN{2673-964X}\gdef\@continuouspages{yes}}
\DeclareOption{coatings}{\gdef\@journal{coatings}\gdef\@journalfull{Coatings}\gdef\@journalshort{Coatings}\gdef\@doiabbr{coatings}\gdef\@ISSN{2079-6412}}
\DeclareOption{colloids}{\gdef\@journal{colloids}\gdef\@journalfull{Colloids Interfaces}\gdef\@journalshort{Colloids Interfaces}\gdef\@doiabbr{colloids}\gdef\@ISSN{2504-5377}}
\DeclareOption{colorants}{\gdef\@journal{colorants}\gdef\@journalfull{Colorants}\gdef\@journalshort{Colorants}\gdef\@doiabbr{colorants}\gdef\@ISSN{2079-6447}\gdef\@continuouspages{yes}}
\DeclareOption{commodities}{\gdef\@journal{commodities}\gdef\@journalfull{Commodities}\gdef\@journalshort{Commodities}\gdef\@doiabbr{commodities}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{compounds}{\gdef\@journal{compounds}\gdef\@journalfull{Compounds}\gdef\@journalshort{Compounds}\gdef\@doiabbr{compounds}\gdef\@ISSN{2673-6918}\gdef\@continuouspages{yes}}
\DeclareOption{computation}{\gdef\@journal{computation}\gdef\@journalfull{Computation}\gdef\@journalshort{Computation}\gdef\@doiabbr{computation}\gdef\@ISSN{2079-3197}}
\DeclareOption{computers}{\gdef\@journal{computers}\gdef\@journalfull{Computers}\gdef\@journalshort{Computers}\gdef\@doiabbr{computers}\gdef\@ISSN{2073-431X}}
\DeclareOption{condensedmatter}{\gdef\@journal{condensedmatter}\gdef\@journalfull{Condensed Matter}\gdef\@journalshort{Condens. Matter}\gdef\@doiabbr{condmat}\gdef\@ISSN{2410-3896}}
\DeclareOption{conservation}{\gdef\@journal{conservation}\gdef\@journalfull{Conservation}\gdef\@journalshort{Conservation}\gdef\@doiabbr{conservation}\gdef\@ISSN{2673-7159}\gdef\@continuouspages{yes}}
\DeclareOption{constrmater}{\gdef\@journal{constrmater}\gdef\@journalfull{Construction Materials}\gdef\@journalshort{Constr. Mater.}\gdef\@doiabbr{constrmater}\gdef\@ISSN{2673-7108}\gdef\@continuouspages{yes}}
\DeclareOption{cosmetics}{\gdef\@journal{cosmetics}\gdef\@journalfull{Cosmetics}\gdef\@journalshort{Cosmetics}\gdef\@doiabbr{cosmetics}\gdef\@ISSN{2079-9284}}
\DeclareOption{covid}{\gdef\@journal{covid}\gdef\@journalfull{COVID}\gdef\@journalshort{COVID}\gdef\@doiabbr{covid}\gdef\@ISSN{2673-8112}\gdef\@continuouspages{yes}}
\DeclareOption{crops}{\gdef\@journal{crops}\gdef\@journalfull{Crops}\gdef\@journalshort{Crops}\gdef\@doiabbr{crops}\gdef\@ISSN{2673-7655}\gdef\@continuouspages{yes}}
\DeclareOption{cryptography}{\gdef\@journal{cryptography}\gdef\@journalfull{Cryptography}\gdef\@journalshort{Cryptography}\gdef\@doiabbr{cryptography}\gdef\@ISSN{2410-387X}}
\DeclareOption{crystals}{\gdef\@journal{crystals}\gdef\@journalfull{Crystals}\gdef\@journalshort{Crystals}\gdef\@doiabbr{cryst}\gdef\@ISSN{2073-4352}}
\DeclareOption{csmf}{\gdef\@journal{csmf}\gdef\@journalfull{Computer Sciences \& Mathematics Forum}\gdef\@journalshort{Comput. Sci. Math. Forum}\gdef\@doiabbr{csmf}\gdef\@ISSN{2813-0324}}
\DeclareOption{ctn}{\gdef\@journal{ctn}\gdef\@journalfull{Clinical and Translational Neuroscience}\gdef\@journalshort{Clin. Transl. Neurosci.}\gdef\@doiabbr{ctn}\gdef\@ISSN{2514-183X}}
\DeclareOption{curroncol}{\gdef\@journal{curroncol}\gdef\@journalfull{Current Oncology}\gdef\@journalshort{Curr. Oncol.}\gdef\@doiabbr{curroncol}\gdef\@ISSN{1718-7729}\gdef\@continuouspages{yes}}
\DeclareOption{cyber}{\gdef\@journal{cyber}\gdef\@journalfull{Cyber}\gdef\@journalshort{Cyber}\gdef\@doiabbr{cyber}\gdef\@ISSN{2624-800X}}
\DeclareOption{dairy}{\gdef\@journal{dairy}\gdef\@journalfull{Dairy}\gdef\@journalshort{Dairy}\gdef\@doiabbr{dairy}\gdef\@ISSN{2624-862X}\gdef\@continuouspages{yes}}
\DeclareOption{data}{\gdef\@journal{data}\gdef\@journalfull{Data}\gdef\@journalshort{Data}\gdef\@doiabbr{data}\gdef\@ISSN{2306-5729}}
\DeclareOption{ddc}{\gdef\@journal{ddc}\gdef\@journalfull{Drugs and Drug Candidates}\gdef\@journalshort{Drugs Drug Candidates}\gdef\@doiabbr{ddc}\gdef\@ISSN{2813-2998}\gdef\@continuouspages{yes}}
\DeclareOption{dentistry}{\gdef\@journal{dentistry}\gdef\@journalfull{Dentistry Journal}\gdef\@journalshort{Dent. J.}\gdef\@doiabbr{dj}\gdef\@ISSN{2304-6767}}
\DeclareOption{dermato}{\gdef\@journal{dermato}\gdef\@journalfull{Dermato}\gdef\@journalshort{Dermato}\gdef\@doiabbr{dermato}\gdef\@ISSN{2673-6179}\gdef\@continuouspages{yes}}
\DeclareOption{dermatopathology}{\gdef\@journal{dermatopathology}\gdef\@journalfull{Dermatopathology}\gdef\@journalshort{Dermatopathology}\gdef\@doiabbr{dermatopathology}\gdef\@ISSN{2296-3529}\gdef\@continuouspages{yes}}
\DeclareOption{designs}{\gdef\@journal{designs}\gdef\@journalfull{Designs}\gdef\@journalshort{Designs}\gdef\@doiabbr{designs}\gdef\@ISSN{2411-9660}}
\DeclareOption{devices}{\gdef\@journal{devices}\gdef\@journalfull{Devices}\gdef\@journalshort{Devices}\gdef\@doiabbr{devices}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{diabetology}{\gdef\@journal{diabetology}\gdef\@journalfull{Diabetology}\gdef\@journalshort{Diabetology}\gdef\@doiabbr{diabetology}\gdef\@ISSN{2673-4540}\gdef\@continuouspages{yes}}
\DeclareOption{diagnostics}{\gdef\@journal{diagnostics}\gdef\@journalfull{Diagnostics}\gdef\@journalshort{Diagnostics}\gdef\@doiabbr{diagnostics}\gdef\@ISSN{2075-4418}}
\DeclareOption{dietetics}{\gdef\@journal{dietetics}\gdef\@journalfull{Dietetics}\gdef\@journalshort{Dietetics}\gdef\@doiabbr{dietetics}\gdef\@ISSN{2674-0311}\gdef\@continuouspages{yes}}
\DeclareOption{digital}{\gdef\@journal{digital}\gdef\@journalfull{Digital}\gdef\@journalshort{Digital}\gdef\@doiabbr{digital}\gdef\@ISSN{2673-6470}\gdef\@continuouspages{yes}}
\DeclareOption{disabilities}{\gdef\@journal{disabilities}\gdef\@journalfull{Disabilities}\gdef\@journalshort{Disabilities}\gdef\@doiabbr{disabilities}\gdef\@ISSN{2673-7272}\gdef\@continuouspages{yes}}
\DeclareOption{diseases}{\gdef\@journal{diseases}\gdef\@journalfull{Diseases}\gdef\@journalshort{Diseases}\gdef\@doiabbr{diseases}\gdef\@ISSN{2079-9721}}
\DeclareOption{diversity}{\gdef\@journal{diversity}\gdef\@journalfull{Diversity}\gdef\@journalshort{Diversity}\gdef\@doiabbr{d}\gdef\@ISSN{1424-2818}}
\DeclareOption{dna}{\gdef\@journal{dna}\gdef\@journalfull{DNA}\gdef\@journalshort{DNA}\gdef\@doiabbr{dna}\gdef\@ISSN{2673-8856}\gdef\@continuouspages{yes}}
\DeclareOption{drones}{\gdef\@journal{drones}\gdef\@journalfull{Drones}\gdef\@journalshort{Drones}\gdef\@doiabbr{drones}\gdef\@ISSN{2504-446X}}
\DeclareOption{dynamics}{\gdef\@journal{dynamics}\gdef\@journalfull{Dynamics}\gdef\@journalshort{Dynamics}\gdef\@doiabbr{dynamics}\gdef\@ISSN{2673-8716}\gdef\@continuouspages{yes}}
\DeclareOption{earth}{\gdef\@journal{earth}\gdef\@journalfull{Earth}\gdef\@journalshort{Earth}\gdef\@doiabbr{earth}\gdef\@ISSN{2673-4834}\gdef\@continuouspages{yes}}
\DeclareOption{ebj}{\gdef\@journal{ebj}\gdef\@journalfull{European Burn Journal}\gdef\@journalshort{Eur. Burn J.}\gdef\@doiabbr{ebj}\gdef\@ISSN{2673-1991}\gdef\@continuouspages{yes}}
\DeclareOption{ecologies}{\gdef\@journal{ecologies}\gdef\@journalfull{Ecologies}\gdef\@journalshort{Ecologies}\gdef\@doiabbr{ecologies}\gdef\@ISSN{2673-4133}\gdef\@continuouspages{yes}}
\DeclareOption{econometrics}{\gdef\@journal{econometrics}\gdef\@journalfull{Econometrics}\gdef\@journalshort{Econometrics}\gdef\@doiabbr{econometrics}\gdef\@ISSN{2225-1146}}
\DeclareOption{economies}{\gdef\@journal{economies}\gdef\@journalfull{Economies}\gdef\@journalshort{Economies}\gdef\@doiabbr{economies}\gdef\@ISSN{2227-7099}}
\DeclareOption{education}{\gdef\@journal{education}\gdef\@journalfull{Education Sciences}\gdef\@journalshort{Educ. Sci.}\gdef\@doiabbr{educsci}\gdef\@ISSN{2227-7102}}
\DeclareOption{ejihpe}{\gdef\@journal{ejihpe}\gdef\@journalfull{European Journal of Investigation in Health Psychology and Education}\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}\gdef\@doiabbr{ejihpe}\gdef\@ISSN{2254-9625}\gdef\@continuouspages{yes}}
\DeclareOption{electricity}{\gdef\@journal{electricity}\gdef\@journalfull{Electricity}\gdef\@journalshort{Electricity}\gdef\@doiabbr{electricity}\gdef\@ISSN{2673-4826}\gdef\@continuouspages{yes}}
\DeclareOption{electrochem}{\gdef\@journal{electrochem}\gdef\@journalfull{Electrochem}\gdef\@journalshort{Electrochem}\gdef\@doiabbr{electrochem}\gdef\@ISSN{2673-3293}\gdef\@continuouspages{yes}}
\DeclareOption{electronicmat}{\gdef\@journal{electronicmat}\gdef\@journalfull{Electronic Materials}\gdef\@journalshort{Electron. Mater.}\gdef\@doiabbr{electronicmat}\gdef\@ISSN{2673-3978}\gdef\@continuouspages{yes}}
\DeclareOption{electronics}{\gdef\@journal{electronics}\gdef\@journalfull{Electronics}\gdef\@journalshort{Electronics}\gdef\@doiabbr{electronics}\gdef\@ISSN{2079-9292}}
\DeclareOption{encyclopedia}{\gdef\@journal{encyclopedia}\gdef\@journalfull{Encyclopedia}\gdef\@journalshort{Encyclopedia}\gdef\@doiabbr{encyclopedia}\gdef\@ISSN{2673-8392}\gdef\@continuouspages{yes}}
\DeclareOption{endocrines}{\gdef\@journal{endocrines}\gdef\@journalfull{Endocrines}\gdef\@journalshort{Endocrines}\gdef\@doiabbr{endocrines}\gdef\@ISSN{2673-396X}\gdef\@continuouspages{yes}}
\DeclareOption{energies}{\gdef\@journal{energies}\gdef\@journalfull{Energies}\gdef\@journalshort{Energies}\gdef\@doiabbr{en}\gdef\@ISSN{1996-1073}}
\DeclareOption{eng}{\gdef\@journal{eng}\gdef\@journalfull{Eng-Advances in Engineering}\gdef\@journalshort{Eng}\gdef\@doiabbr{eng}\gdef\@ISSN{2673-4117}\gdef\@continuouspages{yes}}
\DeclareOption{engproc}{\gdef\@journal{engproc}\gdef\@journalfull{Engineering Proceedings}\gdef\@journalshort{Eng. Proc.}\gdef\@doiabbr{engproc}\gdef\@ISSN{2673-4591}}
%\DeclareOption{ent}{\gdef\@journal{ent}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{entomology}{\gdef\@journal{entomology}\gdef\@journalfull{Entomology}\gdef\@journalshort{Entomology}\gdef\@doiabbr{entomology}\gdef\@ISSN{2813-0502}\gdef\@continuouspages{yes}}	
\DeclareOption{entropy}{\gdef\@journal{entropy}\gdef\@journalfull{Entropy}\gdef\@journalshort{Entropy}\gdef\@doiabbr{e}\gdef\@ISSN{1099-4300}}
\DeclareOption{environments}{\gdef\@journal{environments}\gdef\@journalfull{Environments}\gdef\@journalshort{Environments}\gdef\@doiabbr{environments}\gdef\@ISSN{2076-3298}}
\DeclareOption{environsciproc}{\gdef\@journal{environsciproc}\gdef\@journalfull{Environmental Sciences Proceedings}\gdef\@journalshort{Environ. Sci. Proc.}\gdef\@doiabbr{environsciproc}\gdef\@ISSN{2673-4931}}
\DeclareOption{epidemiologia}{\gdef\@journal{epidemiologia}\gdef\@journalfull{Epidemiologia}\gdef\@journalshort{Epidemiologia}\gdef\@doiabbr{epidemiologia}\gdef\@ISSN{2673-3986}\gdef\@continuouspages{yes}}
\DeclareOption{epigenomes}{\gdef\@journal{epigenomes}\gdef\@journalfull{Epigenomes}\gdef\@journalshort{Epigenomes}\gdef\@doiabbr{epigenomes}\gdef\@ISSN{2075-4655}}
\DeclareOption{est}{\gdef\@journal{est}\gdef\@journalfull{Electrochemical Science and Technology}\gdef\@journalshort{Electrochem. Sci. Technol.}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{fermentation}{\gdef\@journal{fermentation}\gdef\@journalfull{Fermentation}\gdef\@journalshort{Fermentation}\gdef\@doiabbr{fermentation}\gdef\@ISSN{2311-5637}}
\DeclareOption{fibers}{\gdef\@journal{fibers}\gdef\@journalfull{Fibers}\gdef\@journalshort{Fibers}\gdef\@doiabbr{fib}\gdef\@ISSN{2079-6439}}
\DeclareOption{fintech}{\gdef\@journal{fintech}\gdef\@journalfull{FinTech}\gdef\@journalshort{FinTech}\gdef\@doiabbr{fintech}\gdef\@ISSN{2674-1032}\gdef\@continuouspages{yes}}
\DeclareOption{fire}{\gdef\@journal{fire}\gdef\@journalfull{Fire}\gdef\@journalshort{Fire}\gdef\@doiabbr{fire}\gdef\@ISSN{2571-6255}}
\DeclareOption{fishes}{\gdef\@journal{fishes}\gdef\@journalfull{Fishes}\gdef\@journalshort{Fishes}\gdef\@doiabbr{fishes}\gdef\@ISSN{2410-3888}}
\DeclareOption{fluids}{\gdef\@journal{fluids}\gdef\@journalfull{Fluids}\gdef\@journalshort{Fluids}\gdef\@doiabbr{fluids}\gdef\@ISSN{2311-5521}}
\DeclareOption{foods}{\gdef\@journal{foods}\gdef\@journalfull{Foods}\gdef\@journalshort{Foods}\gdef\@doiabbr{foods}\gdef\@ISSN{2304-8158}}
\DeclareOption{forecasting}{\gdef\@journal{forecasting}\gdef\@journalfull{Forecasting}\gdef\@journalshort{Forecasting}\gdef\@doiabbr{forecast}\gdef\@ISSN{2571-9394}\gdef\@continuouspages{yes}}
\DeclareOption{forensicsci}{\gdef\@journal{forensicsci}\gdef\@journalfull{Forensic Sciences}\gdef\@journalshort{Forensic Sci.}\gdef\@doiabbr{forensicsci}\gdef\@ISSN{2673-6756}\gdef\@continuouspages{yes}}
\DeclareOption{forests}{\gdef\@journal{forests}\gdef\@journalfull{Forests}\gdef\@journalshort{Forests}\gdef\@doiabbr{f}\gdef\@ISSN{1999-4907}}
\DeclareOption{foundations}{\gdef\@journal{foundations}\gdef\@journalfull{Foundations}\gdef\@journalshort{Foundations}\gdef\@doiabbr{foundations}\gdef\@ISSN{2673-9321}\gdef\@continuouspages{yes}}
\DeclareOption{fractalfract}{\gdef\@journal{fractalfract}\gdef\@journalfull{Fractal and Fractional}\gdef\@journalshort{Fractal Fract.}\gdef\@doiabbr{fractalfract}\gdef\@ISSN{2504-3110}}
\DeclareOption{fuels}{\gdef\@journal{fuels}\gdef\@journalfull{Fuels}\gdef\@journalshort{Fuels}\gdef\@doiabbr{fuels}\gdef\@ISSN{2673-3994}\gdef\@continuouspages{yes}}
\DeclareOption{future}{\gdef\@journal{future}\gdef\@journalfull{Future}\gdef\@journalshort{Future}\gdef\@doiabbr{future}\gdef\@ISSN{2813-2882}\gdef\@continuouspages{yes}}
\DeclareOption{futureinternet}{\gdef\@journal{futureinternet}\gdef\@journalfull{Future Internet}\gdef\@journalshort{Future Internet}\gdef\@doiabbr{fi}\gdef\@ISSN{1999-5903}}
%\DeclareOption{futureparasites}{\gdef\@journal{futureparasites}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{futurepharmacol}{\gdef\@journal{futurepharmacol}\gdef\@journalfull{Future Pharmacology}\gdef\@journalshort{Future Pharmacol.}\gdef\@doiabbr{futurepharmacol}\gdef\@ISSN{2673-9879}\gdef\@continuouspages{yes}}
\DeclareOption{futurephys}{\gdef\@journal{futurephys}\gdef\@journalfull{Future Physics}\gdef\@journalshort{Future Phys.}\gdef\@doiabbr{futurephys}\gdef\@ISSN{2624-6503}}
\DeclareOption{futuretransp}{\gdef\@journal{futuretransp}\gdef\@journalfull{Future Transportation}\gdef\@journalshort{Future Transp.}\gdef\@doiabbr{futuretransp}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{galaxies}{\gdef\@journal{galaxies}\gdef\@journalfull{Galaxies}\gdef\@journalshort{Galaxies}\gdef\@doiabbr{galaxies}\gdef\@ISSN{2075-4434}}
\DeclareOption{games}{\gdef\@journal{games}\gdef\@journalfull{Games}\gdef\@journalshort{Games}\gdef\@doiabbr{g}\gdef\@ISSN{2073-4336}}
\DeclareOption{gases}{\gdef\@journal{gases}\gdef\@journalfull{Gases}\gdef\@journalshort{Gases}\gdef\@doiabbr{gases}\gdef\@ISSN{2673-5628}\gdef\@continuouspages{yes}}
\DeclareOption{gastroent}{\gdef\@journal{gastroent}\gdef\@journalfull{Gastroenterology Insights}\gdef\@journalshort{Gastroenterol. Insights}\gdef\@doiabbr{gastroent}\gdef\@ISSN{2036-7422}\gdef\@continuouspages{yes}}
\DeclareOption{gastrointestdisord}{\gdef\@journal{gastrointestdisord}\gdef\@journalfull{Gastrointestinal Disorders}\gdef\@journalshort{Gastrointest. Disord.}\gdef\@doiabbr{gidisord}\gdef\@ISSN{2624-5647}\gdef\@continuouspages{yes}}
\DeclareOption{gels}{\gdef\@journal{gels}\gdef\@journalfull{Gels}\gdef\@journalshort{Gels}\gdef\@doiabbr{gels}\gdef\@ISSN{2310-2861}}
\DeclareOption{genealogy}{\gdef\@journal{genealogy}\gdef\@journalfull{Genealogy}\gdef\@journalshort{Genealogy}\gdef\@doiabbr{genealogy}\gdef\@ISSN{2313-5778}}
\DeclareOption{genes}{\gdef\@journal{genes}\gdef\@journalfull{Genes}\gdef\@journalshort{Genes}\gdef\@doiabbr{genes}\gdef\@ISSN{2073-4425}}
\DeclareOption{geographies}{\gdef\@journal{geographies}\gdef\@journalfull{Geographies}\gdef\@journalshort{Geographies}\gdef\@doiabbr{geographies}\gdef\@ISSN{2673-7086}\gdef\@continuouspages{yes}}
\DeclareOption{geohazards}{\gdef\@journal{geohazards}\gdef\@journalfull{GeoHazards}\gdef\@journalshort{GeoHazards}\gdef\@doiabbr{geohazards}\gdef\@ISSN{2624-795X}\gdef\@continuouspages{yes}}
\DeclareOption{geomatics}{\gdef\@journal{geomatics}\gdef\@journalfull{Geomatics}\gdef\@journalshort{Geomatics}\gdef\@doiabbr{geomatics}\gdef\@ISSN{2673-7418}\gdef\@continuouspages{yes}}
\DeclareOption{geosciences}{\gdef\@journal{geosciences}\gdef\@journalfull{Geosciences}\gdef\@journalshort{Geosciences}\gdef\@doiabbr{geosciences}\gdef\@ISSN{2076-3263}}
\DeclareOption{geotechnics}{\gdef\@journal{geotechnics}\gdef\@journalfull{Geotechnics}\gdef\@journalshort{Geotechnics}\gdef\@doiabbr{geotechnics}\gdef\@ISSN{2673-7094}\gdef\@continuouspages{yes}}
\DeclareOption{geriatrics}{\gdef\@journal{geriatrics}\gdef\@journalfull{Geriatrics}\gdef\@journalshort{Geriatrics}\gdef\@doiabbr{geriatrics}\gdef\@ISSN{2308-3417}}
\DeclareOption{grasses}{\gdef\@journal{grasses}\gdef\@journalfull{Grasses}\gdef\@journalshort{Grasses}\gdef\@doiabbr{grasses}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{gucdd}{\gdef\@journal{gucdd}\gdef\@journalfull{Gout, Urate, and Crystal Deposition Disease}\gdef\@journalshort{Gout Urate Cryst. Depos. Dis.}\gdef\@doiabbr{gucdd}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hazardousmatters}{\gdef\@journal{hazardousmatters}\gdef\@journalfull{Hazardous Matters}\gdef\@journalshort{Hazard. Matters}\gdef\@doiabbr{}\gdef\@ISSN{0014-0014}}
\DeclareOption{healthcare}{\gdef\@journal{healthcare}\gdef\@journalfull{Healthcare}\gdef\@journalshort{Healthcare}\gdef\@doiabbr{healthcare}\gdef\@ISSN{2227-9032}}
\DeclareOption{hearts}{\gdef\@journal{hearts}\gdef\@journalfull{Hearts}\gdef\@journalshort{Hearts}\gdef\@doiabbr{hearts}\gdef\@ISSN{2673-3846}\gdef\@continuouspages{yes}}
\DeclareOption{hemato}{\gdef\@journal{hemato}\gdef\@journalfull{Hemato}\gdef\@journalshort{Hemato}\gdef\@doiabbr{hemato}\gdef\@ISSN{2673-6357}\gdef\@continuouspages{yes}}
\DeclareOption{hematolrep}{\gdef\@journal{hematolrep}\gdef\@journalfull{Hematology Reports}\gdef\@journalshort{Hematol. Rep.}\gdef\@doiabbr{hematolrep}\gdef\@ISSN{2038-8330}\gdef\@continuouspages{yes}}
\DeclareOption{heritage}{\gdef\@journal{heritage}\gdef\@journalfull{Heritage}\gdef\@journalshort{Heritage}\gdef\@doiabbr{heritage}\gdef\@ISSN{2571-9408}\gdef\@continuouspages{yes}}
\DeclareOption{higheredu}{\gdef\@journal{higheredu}\gdef\@journalfull{Trends in Higher Education}\gdef\@journalshort{Trends High. Educ.}\gdef\@doiabbr{higheredu}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{highthroughput}{\gdef\@journal{highthroughput}\gdef\@journalfull{High-Throughput}\gdef\@journalshort{High-Throughput}\gdef\@doiabbr{ht}\gdef\@ISSN{2571-5135}}
\DeclareOption{histories}{\gdef\@journal{histories}\gdef\@journalfull{Histories}\gdef\@journalshort{Histories}\gdef\@doiabbr{histories}\gdef\@ISSN{2409-9252}\gdef\@continuouspages{yes}}
\DeclareOption{horticulturae}{\gdef\@journal{horticulturae}\gdef\@journalfull{Horticulturae}\gdef\@journalshort{Horticulturae}\gdef\@doiabbr{horticulturae}\gdef\@ISSN{2311-7524}}
\DeclareOption{hospitals}{\gdef\@journal{hospitals}\gdef\@journalfull{Hospitals}\gdef\@journalshort{Hospitals}\gdef\@doiabbr{hospitals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{humanities}{\gdef\@journal{humanities}\gdef\@journalfull{Humanities}\gdef\@journalshort{Humanities}\gdef\@doiabbr{h}\gdef\@ISSN{2076-0787}}
\DeclareOption{humans}{\gdef\@journal{humans}\gdef\@journalfull{Humans}\gdef\@journalshort{Humans}\gdef\@doiabbr{humans}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hydrobiology}{\gdef\@journal{hydrobiology}\gdef\@journalfull{Hydrobiology}\gdef\@journalshort{Hydrobiology	}\gdef\@doiabbr{hydrobiology}\gdef\@ISSN{2673-9917}\gdef\@continuouspages{yes}}
\DeclareOption{hydrogen}{\gdef\@journal{hydrogen}\gdef\@journalfull{Hydrogen}\gdef\@journalshort{Hydrogen}\gdef\@doiabbr{hydrogen}\gdef\@ISSN{2673-4141}\gdef\@continuouspages{yes}}
\DeclareOption{hydrology}{\gdef\@journal{hydrology}\gdef\@journalfull{Hydrology}\gdef\@journalshort{Hydrology}\gdef\@doiabbr{hydrology}\gdef\@ISSN{2306-5338}}
\DeclareOption{hygiene}{\gdef\@journal{hygiene}\gdef\@journalfull{Hygiene}\gdef\@journalshort{Hygiene}\gdef\@doiabbr{hygiene}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{idr}{\gdef\@journal{idr}\gdef\@journalfull{Infectious Disease Reports}\gdef\@journalshort{Infect. Dis. Rep.}\gdef\@doiabbr{idr}\gdef\@ISSN{2036-7449}\gdef\@continuouspages{yes}}
\DeclareOption{ijerph}{\gdef\@journal{ijerph}\gdef\@journalfull{International Journal of Environmental Research and Public Health}\gdef\@journalshort{Int. J. Environ. Res. Public Health}\gdef\@doiabbr{ijerph}\gdef\@ISSN{1660-4601}}
\DeclareOption{ijfs}{\gdef\@journal{ijfs}\gdef\@journalfull{International Journal of Financial Studies}\gdef\@journalshort{Int. J. Financial Stud.}\gdef\@doiabbr{ijfs}\gdef\@ISSN{2227-7072}}
\DeclareOption{ijgi}{\gdef\@journal{ijgi}\gdef\@journalfull{ISPRS International Journal of Geo-Information}\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}\gdef\@doiabbr{ijgi}\gdef\@ISSN{2220-9964}}
\DeclareOption{ijms}{\gdef\@journal{ijms}\gdef\@journalfull{International Journal of Molecular Sciences}\gdef\@journalshort{Int. J. Mol. Sci.}\gdef\@doiabbr{ijms}\gdef\@ISSN{1422-0067}}
\DeclareOption{ijns}{\gdef\@journal{ijns}\gdef\@journalfull{International Journal of Neonatal Screening}\gdef\@journalshort{Int. J. Neonatal Screen.}\gdef\@doiabbr{ijns}\gdef\@ISSN{2409-515X}}
\DeclareOption{ijpb}{\gdef\@journal{ijpb}\gdef\@journalfull{International Journal of Plant Biology}\gdef\@journalshort{Int. J. Plant Biol.}\gdef\@doiabbr{ijpb}\gdef\@ISSN{2037-0164}\gdef\@continuouspages{yes}}
\DeclareOption{ijtm}{\gdef\@journal{ijtm}\gdef\@journalfull{International Journal of Translational Medicine}\gdef\@journalshort{Int. J. Transl. Med.}\gdef\@doiabbr{ijtm}\gdef\@ISSN{2673-8937}\gdef\@continuouspages{yes}}
\DeclareOption{ijtpp}{\gdef\@journal{ijtpp}\gdef\@journalfull{International Journal of Turbomachinery Propulsion and Power}\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}\gdef\@doiabbr{ijtpp}\gdef\@ISSN{2504-186X}}
\DeclareOption{ime}{\gdef\@journal{ime}\gdef\@journalfull{International Medical Education}\gdef\@journalshort{Int. Med. Educ.}\gdef\@doiabbr{ime}\gdef\@ISSN{2813-141X}\gdef\@continuouspages{yes}}
\DeclareOption{immuno}{\gdef\@journal{immuno}\gdef\@journalfull{Immuno}\gdef\@journalshort{Immuno}\gdef\@doiabbr{immuno}\gdef\@ISSN{2673-5601}\gdef\@continuouspages{yes}}
\DeclareOption{informatics}{\gdef\@journal{informatics}\gdef\@journalfull{Informatics}\gdef\@journalshort{Informatics}\gdef\@doiabbr{informatics}\gdef\@ISSN{2227-9709}}
\DeclareOption{information}{\gdef\@journal{information}\gdef\@journalfull{Information}\gdef\@journalshort{Information}\gdef\@doiabbr{info}\gdef\@ISSN{2078-2489}}
\DeclareOption{infrastructures}{\gdef\@journal{infrastructures}\gdef\@journalfull{Infrastructures}\gdef\@journalshort{Infrastructures}\gdef\@doiabbr{infrastructures}\gdef\@ISSN{2412-3811}}
\DeclareOption{inorganics}{\gdef\@journal{inorganics}\gdef\@journalfull{Inorganics}\gdef\@journalshort{Inorganics}\gdef\@doiabbr{inorganics}\gdef\@ISSN{2304-6740}}
\DeclareOption{insects}{\gdef\@journal{insects}\gdef\@journalfull{Insects}\gdef\@journalshort{Insects}\gdef\@doiabbr{insects}\gdef\@ISSN{2075-4450}}
\DeclareOption{instruments}{\gdef\@journal{instruments}\gdef\@journalfull{Instruments}\gdef\@journalshort{Instruments}\gdef\@doiabbr{instruments}\gdef\@ISSN{2410-390X}}
\DeclareOption{inventions}{\gdef\@journal{inventions}\gdef\@journalfull{Inventions}\gdef\@journalshort{Inventions}\gdef\@doiabbr{inventions}\gdef\@ISSN{2411-5134}}
\DeclareOption{iot}{\gdef\@journal{iot}\gdef\@journalfull{IoT}\gdef\@journalshort{IoT}\gdef\@doiabbr{iot}\gdef\@ISSN{2624-831X}\gdef\@continuouspages{yes}}
\DeclareOption{j}{\gdef\@journal{j}\gdef\@journalfull{J}\gdef\@journalshort{J}\gdef\@doiabbr{j}\gdef\@ISSN{2571-8800}\gdef\@continuouspages{yes}}
\DeclareOption{jal}{\gdef\@journal{jal}\gdef\@journalfull{Journal of Ageing and Longevity}\gdef\@journalshort{J. Ageing Longev.}\gdef\@doiabbr{jal}\gdef\@ISSN{2673-9259}\gdef\@continuouspages{yes}}
\DeclareOption{jcdd}{\gdef\@journal{jcdd}\gdef\@journalfull{Journal of Cardiovascular Development and Disease}\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}\gdef\@doiabbr{jcdd}\gdef\@ISSN{2308-3425}}
\DeclareOption{jcm}{\gdef\@journal{jcm}\gdef\@journalfull{Journal of Clinical Medicine}\gdef\@journalshort{J. Clin. Med.}\gdef\@doiabbr{jcm}\gdef\@ISSN{2077-0383}}
\DeclareOption{jcp}{\gdef\@journal{jcp}\gdef\@journalfull{Journal of Cybersecurity and Privacy}\gdef\@journalshort{J. Cybersecur. Priv.}\gdef\@doiabbr{jcp}\gdef\@ISSN{2624-800X}\gdef\@continuouspages{yes}}
\DeclareOption{jcs}{\gdef\@journal{jcs}\gdef\@journalfull{Journal of Composites Science}\gdef\@journalshort{J. Compos. Sci.}\gdef\@doiabbr{jcs}\gdef\@ISSN{2504-477X}}
\DeclareOption{jcto}{\gdef\@journal{jcto}\gdef\@journalfull{Journal of Clinical \& Translational Ophthalmology}\gdef\@journalshort{J. Clin. Transl. Ophthalmol.}\gdef\@doiabbr{jcto}\gdef\@ISSN{2813-1053}\gdef\@continuouspages{yes}}
\DeclareOption{jdb}{\gdef\@journal{jdb}\gdef\@journalfull{Journal of Developmental Biology}\gdef\@journalshort{J. Dev. Biol.}\gdef\@doiabbr{jdb}\gdef\@ISSN{2221-3759}}
\DeclareOption{jeta}{\gdef\@journal{jeta}\gdef\@journalfull{Journal of Experimental and Theoretical Analyses}\gdef\@journalshort{J. Exp. Theor. Anal.}\gdef\@doiabbr{jeta}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jfb}{\gdef\@journal{jfb}\gdef\@journalfull{Journal of Functional Biomaterials}\gdef\@journalshort{J. Funct. Biomater.}\gdef\@doiabbr{jfb}\gdef\@ISSN{2079-4983}}
\DeclareOption{jfmk}{\gdef\@journal{jfmk}\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}\gdef\@doiabbr{jfmk}\gdef\@ISSN{2411-5142}}
\DeclareOption{jimaging}{\gdef\@journal{jimaging}\gdef\@journalfull{Journal of Imaging}\gdef\@journalshort{J. Imaging}\gdef\@doiabbr{jimaging}\gdef\@ISSN{2313-433X}}
\DeclareOption{jintelligence}{\gdef\@journal{jintelligence}\gdef\@journalfull{Journal of Intelligence}\gdef\@journalshort{J. Intell.}\gdef\@doiabbr{jintelligence}\gdef\@ISSN{2079-3200}}
\DeclareOption{jlpea}{\gdef\@journal{jlpea}\gdef\@journalfull{Journal of Low Power Electronics and Applications}\gdef\@journalshort{J. Low Power Electron. Appl.}\gdef\@doiabbr{jlpea}\gdef\@ISSN{2079-9268}}
\DeclareOption{jmmp}{\gdef\@journal{jmmp}\gdef\@journalfull{Journal of Manufacturing and Materials Processing}\gdef\@journalshort{J. Manuf. Mater. Process.}\gdef\@doiabbr{jmmp}\gdef\@ISSN{2504-4494}}
\DeclareOption{jmp}{\gdef\@journal{jmp}\gdef\@journalfull{Journal of Molecular Pathology}\gdef\@journalshort{J. Mol. Pathol.}\gdef\@doiabbr{jmp}\gdef\@ISSN{2673-5261}\gdef\@continuouspages{yes}}
\DeclareOption{jmse}{\gdef\@journal{jmse}\gdef\@journalfull{Journal of Marine Science and Engineering}\gdef\@journalshort{J. Mar. Sci. Eng.}\gdef\@doiabbr{jmse}\gdef\@ISSN{2077-1312}}
\DeclareOption{jne}{\gdef\@journal{jne}\gdef\@journalfull{Journal of Nuclear Engineering}\gdef\@journalshort{J. Nucl. Eng.}\gdef\@doiabbr{jne}\gdef\@ISSN{2673-4362}\gdef\@continuouspages{yes}}
\DeclareOption{jnt}{\gdef\@journal{jnt}\gdef\@journalfull{Journal of Nanotheranostics}\gdef\@journalshort{J. Nanotheranostics}\gdef\@doiabbr{jnt}\gdef\@ISSN{2624-845X}\gdef\@continuouspages{yes}}
\DeclareOption{jof}{\gdef\@journal{jof}\gdef\@journalfull{Journal of Fungi}\gdef\@journalshort{J. Fungi}\gdef\@doiabbr{jof}\gdef\@ISSN{2309-608X}}
\DeclareOption{joitmc}{\gdef\@journal{joitmc}\gdef\@journalfull{Journal of Open Innovation: Technology Market and Complexity}\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}\gdef\@doiabbr{joitmc}\gdef\@ISSN{2199-8531}}
\DeclareOption{jor}{\gdef\@journal{jor}\gdef\@journalfull{Journal of Respiration}\gdef\@journalshort{J. Respir.}\gdef\@doiabbr{jor}\gdef\@ISSN{2673-527X}\gdef\@continuouspages{yes}}
\DeclareOption{journalmedia}{\gdef\@journal{journalmedia}\gdef\@journalfull{Journalism and Media}\gdef\@journalshort{Journal. Media}\gdef\@doiabbr{journalmedia}\gdef\@ISSN{2673-5172}\gdef\@continuouspages{yes}}
\DeclareOption{jox}{\gdef\@journal{jox}\gdef\@journalfull{Journal of Xenobiotics}\gdef\@journalshort{J. Xenobiot.}\gdef\@doiabbr{jox}\gdef\@ISSN{2039-4713}\gdef\@continuouspages{yes}}
\DeclareOption{jpm}{\gdef\@journal{jpm}\gdef\@journalfull{Journal of Personalized Medicine}\gdef\@journalshort{J. Pers. Med.}\gdef\@doiabbr{jpm}\gdef\@ISSN{2075-4426}}
\DeclareOption{jrfm}{\gdef\@journal{jrfm}\gdef\@journalfull{Journal of Risk and Financial Management}\gdef\@journalshort{J. Risk Financial Manag.}\gdef\@doiabbr{jrfm}\gdef\@ISSN{1911-8074}}
\DeclareOption{jsan}{\gdef\@journal{jsan}\gdef\@journalfull{Journal of Sensor and Actuator Networks}\gdef\@journalshort{J. Sens. Actuator Netw.}\gdef\@doiabbr{jsan}\gdef\@ISSN{2224-2708}}
\DeclareOption{jtaer}{\gdef\@journal{jtaer}\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}\gdef\@doiabbr{jtaer}\gdef\@ISSN{0718-1876}\gdef\@continuouspages{yes}}
\DeclareOption{jvd}{\gdef\@journal{jvd}\gdef\@journalfull{Journal of Vascular Diseases}\gdef\@journalshort{JVD}\gdef\@doiabbr{jvd}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jzbg}{\gdef\@journal{jzbg}\gdef\@journalfull{Journal of Zoological and Botanical Gardens}\gdef\@journalshort{J. Zool. Bot. Gard.}\gdef\@doiabbr{jzbg}\gdef\@ISSN{2673-5636}\gdef\@continuouspages{yes}}
%\DeclareOption{kidney}{\gdef\@journal{kidney}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kidneydial}{\gdef\@journal{kidneydial}\gdef\@journalfull{Kidney and Dialysis}\gdef\@journalshort{Kidney Dial.}\gdef\@doiabbr{kinasesphosphatases}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kinasesphosphatases}{\gdef\@journal{kinasesphosphatases}\gdef\@journalfull{Kinases and Phosphatases}\gdef\@journalshort{Kinases Phosphatases}\gdef\@doiabbr{kinasesphosphatases}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{knowledge}{\gdef\@journal{knowledge}\gdef\@journalfull{Knowledge}\gdef\@journalshort{Knowledge}\gdef\@doiabbr{knowledge}\gdef\@ISSN{2673-9585}\gdef\@continuouspages{yes}}
\DeclareOption{land}{\gdef\@journal{land}\gdef\@journalfull{Land}\gdef\@journalshort{Land}\gdef\@doiabbr{land}\gdef\@ISSN{2073-445X}}
\DeclareOption{languages}{\gdef\@journal{languages}\gdef\@journalfull{Languages}\gdef\@journalshort{Languages}\gdef\@doiabbr{languages}\gdef\@ISSN{2226-471X}}
\DeclareOption{laws}{\gdef\@journal{laws}\gdef\@journalfull{Laws}\gdef\@journalshort{Laws}\gdef\@doiabbr{laws}\gdef\@ISSN{2075-471X}}
\DeclareOption{life}{\gdef\@journal{life}\gdef\@journalfull{Life}\gdef\@journalshort{Life}\gdef\@doiabbr{life}\gdef\@ISSN{2075-1729}}
\DeclareOption{liquids}{\gdef\@journal{liquids}\gdef\@journalfull{Liquids}\gdef\@journalshort{Liquids}\gdef\@doiabbr{liquids}\gdef\@ISSN{2673-8015}\gdef\@continuouspages{yes}}
\DeclareOption{literature}{\gdef\@journal{literature}\gdef\@journalfull{Literature}\gdef\@journalshort{Literature}\gdef\@doiabbr{literature}\gdef\@ISSN{2410-9789}\gdef\@continuouspages{yes}}
\DeclareOption{livers}{\gdef\@journal{livers}\gdef\@journalfull{Livers}\gdef\@journalshort{Livers}\gdef\@doiabbr{livers}\gdef\@ISSN{2673-4389}\gdef\@continuouspages{yes}}
\DeclareOption{logics}{\gdef\@journal{logics}\gdef\@journalfull{Logics}\gdef\@journalshort{Logics}\gdef\@doiabbr{logics}\gdef\@ISSN{2813-0405}\gdef\@continuouspages{yes}}
\DeclareOption{logistics}{\gdef\@journal{logistics}\gdef\@journalfull{Logistics}\gdef\@journalshort{Logistics}\gdef\@doiabbr{logistics}\gdef\@ISSN{2305-6290}}
\DeclareOption{lubricants}{\gdef\@journal{lubricants}\gdef\@journalfull{Lubricants}\gdef\@journalshort{Lubricants}\gdef\@doiabbr{lubricants}\gdef\@ISSN{2075-4442}}
\DeclareOption{lymphatics}{\gdef\@journal{lymphatics}\gdef\@journalfull{Lymphatics}\gdef\@journalshort{Lymphatics}\gdef\@doiabbr{lymphatics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}	
\DeclareOption{machines}{\gdef\@journal{machines}\gdef\@journalfull{Machines}\gdef\@journalshort{Machines}\gdef\@doiabbr{machines}\gdef\@ISSN{2075-1702}}
\DeclareOption{macromol}{\gdef\@journal{macromol}\gdef\@journalfull{Macromol}\gdef\@journalshort{Macromol}\gdef\@doiabbr{macromol}\gdef\@ISSN{2673-6209}\gdef\@continuouspages{yes}}
\DeclareOption{magnetism}{\gdef\@journal{magnetism}\gdef\@journalfull{Magnetism}\gdef\@journalshort{Magnetism}\gdef\@doiabbr{magnetism}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{magnetochemistry}{\gdef\@journal{magnetochemistry}\gdef\@journalfull{Magnetochemistry}\gdef\@journalshort{Magnetochemistry}\gdef\@doiabbr{magnetochemistry}\gdef\@ISSN{2312-7481}}
\DeclareOption{make}{\gdef\@journal{make}\gdef\@journalfull{Machine Learning and Knowledge Extraction}\gdef\@journalshort{Mach. Learn. Knowl. Extr.}\gdef\@doiabbr{make}\gdef\@ISSN{2504-4990}\gdef\@continuouspages{yes}}
\DeclareOption{marinedrugs}{\gdef\@journal{marinedrugs}\gdef\@journalfull{Marine Drugs}\gdef\@journalshort{Mar. Drugs}\gdef\@doiabbr{md}\gdef\@ISSN{1660-3397}}
\DeclareOption{materials}{\gdef\@journal{materials}\gdef\@journalfull{Materials}\gdef\@journalshort{Materials}\gdef\@doiabbr{ma}\gdef\@ISSN{1996-1944}}
\DeclareOption{materproc}{\gdef\@journal{materproc}\gdef\@journalfull{Materials Proceedings}\gdef\@journalshort{Mater. Proc.}\gdef\@doiabbr{materproc}\gdef\@ISSN{2673-4605}}
\DeclareOption{mathematics}{\gdef\@journal{mathematics}\gdef\@journalfull{Mathematics}\gdef\@journalshort{Mathematics}\gdef\@doiabbr{math}\gdef\@ISSN{2227-7390}}
\DeclareOption{mca}{\gdef\@journal{mca}\gdef\@journalfull{Mathematical and Computational Applications}\gdef\@journalshort{Math. Comput. Appl.}\gdef\@doiabbr{mca}\gdef\@ISSN{2297-8747}}
\DeclareOption{measurements}{\gdef\@journal{measurements}\gdef\@journalfull{Measurements}\gdef\@journalshort{Measurements}\gdef\@doiabbr{measurements}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{medicina}{\gdef\@journal{medicina}\gdef\@journalfull{Medicina}\gdef\@journalshort{Medicina}\gdef\@doiabbr{medicina}\gdef\@ISSN{1648-9144}}
\DeclareOption{medicines}{\gdef\@journal{medicines}\gdef\@journalfull{Medicines}\gdef\@journalshort{Medicines}\gdef\@doiabbr{medicines}\gdef\@ISSN{2305-6320}}
\DeclareOption{medsci}{\gdef\@journal{medsci}\gdef\@journalfull{Medical Sciences}\gdef\@journalshort{Med. Sci.}\gdef\@doiabbr{medsci}\gdef\@ISSN{2076-3271}}
\DeclareOption{membranes}{\gdef\@journal{membranes}\gdef\@journalfull{Membranes}\gdef\@journalshort{Membranes}\gdef\@doiabbr{membranes}\gdef\@ISSN{2077-0375}}
\DeclareOption{merits}{\gdef\@journal{merits}\gdef\@journalfull{Merits}\gdef\@journalshort{Merits}\gdef\@doiabbr{merits}\gdef\@ISSN{2673-8104}\gdef\@continuouspages{yes}}
\DeclareOption{metabolites}{\gdef\@journal{metabolites}\gdef\@journalfull{Metabolites}\gdef\@journalshort{Metabolites}\gdef\@doiabbr{metabo}\gdef\@ISSN{2218-1989}}
\DeclareOption{metals}{\gdef\@journal{metals}\gdef\@journalfull{Metals}\gdef\@journalshort{Metals}\gdef\@doiabbr{met}\gdef\@ISSN{2075-4701}}
\DeclareOption{meteorology}{\gdef\@journal{meteorology}\gdef\@journalfull{Meteorology}\gdef\@journalshort{Meteorology}\gdef\@doiabbr{meteorology}\gdef\@ISSN{2674-0494}\gdef\@continuouspages{yes}}
\DeclareOption{methane}{\gdef\@journal{methane}\gdef\@journalfull{Methane}\gdef\@journalshort{Methane}\gdef\@doiabbr{methane}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{metrology}{\gdef\@journal{metrology}\gdef\@journalfull{Metrology}\gdef\@journalshort{Metrology}\gdef\@doiabbr{metrology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{micro}{\gdef\@journal{micro}\gdef\@journalfull{Micro}\gdef\@journalshort{Micro}\gdef\@doiabbr{micro}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{microarrays}{\gdef\@journal{microarrays}\gdef\@journalfull{Microarrays}\gdef\@journalshort{Microarrays}\gdef\@doiabbr{microarrays}\gdef\@ISSN{2076-3905}}
\DeclareOption{microbiolres}{\gdef\@journal{microbiolres}\gdef\@journalfull{Microbiology Research}\gdef\@journalshort{Microbiol. Res.}\gdef\@doiabbr{microbiolres}\gdef\@ISSN{2036-7481}\gdef\@continuouspages{yes}}
\DeclareOption{micromachines}{\gdef\@journal{micromachines}\gdef\@journalfull{Micromachines}\gdef\@journalshort{Micromachines}\gdef\@doiabbr{mi}\gdef\@ISSN{2072-666X}}
\DeclareOption{microorganisms}{\gdef\@journal{microorganisms}\gdef\@journalfull{Microorganisms}\gdef\@journalshort{Microorganisms}\gdef\@doiabbr{microorganisms}\gdef\@ISSN{2076-2607}}
\DeclareOption{microplastics}{\gdef\@journal{microplastics}\gdef\@journalfull{Microplastics}\gdef\@journalshort{Microplastics}\gdef\@doiabbr{microplastics}\gdef\@ISSN{2673-8929}\gdef\@continuouspages{yes}}
\DeclareOption{minerals}{\gdef\@journal{minerals}\gdef\@journalfull{Minerals}\gdef\@journalshort{Minerals}\gdef\@doiabbr{min}\gdef\@ISSN{2075-163X}}
\DeclareOption{mining}{\gdef\@journal{mining}\gdef\@journalfull{Mining}\gdef\@journalshort{Mining}\gdef\@doiabbr{mining}\gdef\@ISSN{2673-6489}\gdef\@continuouspages{yes}}
\DeclareOption{modelling}{\gdef\@journal{modelling}\gdef\@journalfull{Modelling}\gdef\@journalshort{Modelling}\gdef\@doiabbr{modelling}\gdef\@ISSN{2673-3951}\gdef\@continuouspages{yes}}
\DeclareOption{molbank}{\gdef\@journal{molbank}\gdef\@journalfull{Molbank}\gdef\@journalshort{Molbank}\gdef\@doiabbr{M}\gdef\@ISSN{1422-8599}}
\DeclareOption{molecules}{\gdef\@journal{molecules}\gdef\@journalfull{Molecules}\gdef\@journalshort{Molecules}\gdef\@doiabbr{molecules}\gdef\@ISSN{1420-3049}}
\DeclareOption{mps}{\gdef\@journal{mps}\gdef\@journalfull{Methods and Protocols}\gdef\@journalshort{Methods Protoc.}\gdef\@doiabbr{mps}\gdef\@ISSN{2409-9279}}
\DeclareOption{msf}{\gdef\@journal{msf}\gdef\@journalfull{Medical Sciences Forum}\gdef\@journalshort{Med. Sci. Forum}\gdef\@doiabbr{msf}\gdef\@ISSN{2673-9992}}
\DeclareOption{mti}{\gdef\@journal{mti}\gdef\@journalfull{Multimodal Technologies and Interaction}\gdef\@journalshort{Multimodal Technol. Interact.}\gdef\@doiabbr{mti}\gdef\@ISSN{2414-4088}}
\DeclareOption{muscles}{\gdef\@journal{muscles}\gdef\@journalfull{Muscles}\gdef\@journalshort{Muscles}\gdef\@doiabbr{muscles}\gdef\@ISSN{2813-0413}\gdef\@continuouspages{yes}}
\DeclareOption{nanoenergyadv}{\gdef\@journal{nanoenergyadv}\gdef\@journalfull{Nanoenergy Advances}\gdef\@journalshort{Nanoenergy Adv.}\gdef\@doiabbr{nanoenergyadv}\gdef\@ISSN{2673-706X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomanufacturing}{\gdef\@journal{nanomanufacturing}\gdef\@journalfull{Nanomanufacturing}\gdef\@journalshort{Nanomanufacturing}\gdef\@doiabbr{nanomanufacturing}\gdef\@ISSN{2673-687X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomaterials}{\gdef\@journal{nanomaterials}\gdef\@journalfull{Nanomaterials}\gdef\@journalshort{Nanomaterials}\gdef\@doiabbr{nano}\gdef\@ISSN{2079-4991}}
\DeclareOption{ncrna}{\gdef\@journal{ncrna}\gdef\@journalfull{Non-Coding RNA}\gdef\@journalshort{Non-Coding RNA}\gdef\@doiabbr{ncrna}\gdef\@ISSN{2311-553X}}
\DeclareOption{ndt}{\gdef\@journal{ndt}\gdef\@journalfull{NDT}\gdef\@journalshort{NDT}\gdef\@doiabbr{ndt}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{network}{\gdef\@journal{network}\gdef\@journalfull{Network}\gdef\@journalshort{Network}\gdef\@doiabbr{network}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{neuroglia}{\gdef\@journal{neuroglia}\gdef\@journalfull{Neuroglia}\gdef\@journalshort{Neuroglia}\gdef\@doiabbr{neuroglia}\gdef\@ISSN{2571-6980}\gdef\@continuouspages{yes}}
\DeclareOption{neurolint}{\gdef\@journal{neurolint}\gdef\@journalfull{Neurology International}\gdef\@journalshort{Neurol. Int.}\gdef\@doiabbr{neurolint}\gdef\@ISSN{2035-8377}\gdef\@continuouspages{yes}}
\DeclareOption{neurosci}{\gdef\@journal{neurosci}\gdef\@journalfull{NeuroSci}\gdef\@journalshort{NeuroSci}\gdef\@doiabbr{neurosci}\gdef\@ISSN{2673-4087}\gdef\@continuouspages{yes}}
\DeclareOption{nitrogen}{\gdef\@journal{nitrogen}\gdef\@journalfull{Nitrogen}\gdef\@journalshort{Nitrogen}\gdef\@doiabbr{nitrogen}\gdef\@ISSN{2504-3129}\gdef\@continuouspages{yes}}
\DeclareOption{notspecified}{\gdef\@journal{notspecified}\gdef\@journalfull{Journal Not Specified}\gdef\@journalshort{Journal Not Specified}\gdef\@doiabbr{}\gdef\@ISSN{}}
%%\DeclareOption{nri}{\gdef\@journal{nri}\gdef\@journalfull{Natural Resources Informatics}\gdef\@journalshort{Nat. Resour. Inform.}\gdef\@doiabbr{nri}\gdef\@ISSN{2673-981X}\gdef\@continuouspages{yes}}
\DeclareOption{nursrep}{\gdef\@journal{nursrep}\gdef\@journalfull{Nursing Reports}\gdef\@journalshort{Nurs. Rep.}\gdef\@doiabbr{nursrep}\gdef\@ISSN{2039-4403}\gdef\@continuouspages{yes}}
\DeclareOption{nutraceuticals}{\gdef\@journal{nutraceuticals}\gdef\@journalfull{Nutraceuticals}\gdef\@journalshort{Nutraceuticals}\gdef\@doiabbr{nutraceuticals}\gdef\@ISSN{1661-3821}\gdef\@continuouspages{yes}}
\DeclareOption{nutrients}{\gdef\@journal{nutrients}\gdef\@journalfull{Nutrients}\gdef\@journalshort{Nutrients}\gdef\@doiabbr{nu}\gdef\@ISSN{2072-6643}}
\DeclareOption{obesities}{\gdef\@journal{obesities}\gdef\@journalfull{Obesities}\gdef\@journalshort{Obesities}\gdef\@doiabbr{obesities}\gdef\@ISSN{2673-4168}\gdef\@continuouspages{yes}}
\DeclareOption{oceans}{\gdef\@journal{oceans}\gdef\@journalfull{Oceans}\gdef\@journalshort{Oceans}\gdef\@doiabbr{oceans}\gdef\@ISSN{2673-1924}\gdef\@continuouspages{yes}}
\DeclareOption{ohbm}{\gdef\@journal{ohbm}\gdef\@journalfull{Journal of Otorhinolaryngology Hearing and Balance Medicine}\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}\gdef\@doiabbr{ohbm}\gdef\@ISSN{2504-463X}}
\DeclareOption{onco}{\gdef\@journal{onco}\gdef\@journalfull{Onco}\gdef\@journalshort{Onco}\gdef\@doiabbr{onco}\gdef\@ISSN{2673-7523}\gdef\@continuouspages{yes}}
%\DeclareOption{oncopathology}{\gdef\@journal{oncopathology}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{optics}{\gdef\@journal{optics}\gdef\@journalfull{Optics}\gdef\@journalshort{Optics}\gdef\@doiabbr{opt}\gdef\@ISSN{2673-3269}\gdef\@continuouspages{yes}}
\DeclareOption{oral}{\gdef\@journal{oral}\gdef\@journalfull{Oral}\gdef\@journalshort{Oral}\gdef\@doiabbr{oral}\gdef\@ISSN{2673-6373}\gdef\@continuouspages{yes}}
\DeclareOption{organics}{\gdef\@journal{organics}\gdef\@journalfull{Organics}\gdef\@journalshort{Organics}\gdef\@doiabbr{org}\gdef\@ISSN{2673-401X}\gdef\@continuouspages{yes}}
\DeclareOption{organoids}{\gdef\@journal{organoids}\gdef\@journalfull{Organoids}\gdef\@journalshort{Organoids}\gdef\@doiabbr{organoids}\gdef\@ISSN{2674-1172}\gdef\@continuouspages{yes}}
\DeclareOption{osteology}{\gdef\@journal{osteology}\gdef\@journalfull{Osteology}\gdef\@journalshort{Osteology}\gdef\@doiabbr{osteology}\gdef\@ISSN{2673-4036}\gdef\@continuouspages{yes}}
\DeclareOption{oxygen}{\gdef\@journal{oxygen}\gdef\@journalfull{Oxygen}\gdef\@journalshort{Oxygen}\gdef\@doiabbr{oxygen}\gdef\@ISSN{2673-9801}\gdef\@continuouspages{yes}}
\DeclareOption{parasites}{\gdef\@journal{parasites}\gdef\@journalfull{Parasites}\gdef\@journalshort{Parasites}\gdef\@doiabbr{parasites}\gdef\@ISSN{2673-5946}}
\DeclareOption{parasitologia}{\gdef\@journal{parasitologia}\gdef\@journalfull{Parasitologia}\gdef\@journalshort{Parasitologia}\gdef\@doiabbr{parasitologia}\gdef\@ISSN{2673-6772}\gdef\@continuouspages{yes}}
\DeclareOption{particles}{\gdef\@journal{particles}\gdef\@journalfull{Particles}\gdef\@journalshort{Particles}\gdef\@doiabbr{particles}\gdef\@ISSN{2571-712X}\gdef\@continuouspages{yes}}
\DeclareOption{pathogens}{\gdef\@journal{pathogens}\gdef\@journalfull{Pathogens}\gdef\@journalshort{Pathogens}\gdef\@doiabbr{pathogens}\gdef\@ISSN{2076-0817}}
\DeclareOption{pathophysiology}{\gdef\@journal{pathophysiology}\gdef\@journalfull{Pathophysiology}\gdef\@journalshort{Pathophysiology}\gdef\@doiabbr{pathophysiology}\gdef\@ISSN{0928-4680}\gdef\@continuouspages{yes}}
\DeclareOption{pediatrrep}{\gdef\@journal{pediatrrep}\gdef\@journalfull{Pediatric Reports}\gdef\@journalshort{Pediatr. Rep.}\gdef\@doiabbr{pediatric}\gdef\@ISSN{2036-7503}\gdef\@continuouspages{yes}}
\DeclareOption{pharmaceuticals}{\gdef\@journal{pharmaceuticals}\gdef\@journalfull{Pharmaceuticals}\gdef\@journalshort{Pharmaceuticals}\gdef\@doiabbr{ph}\gdef\@ISSN{1424-8247}}
\DeclareOption{pharmaceutics}{\gdef\@journal{pharmaceutics}\gdef\@journalfull{Pharmaceutics}\gdef\@journalshort{Pharmaceutics}\gdef\@doiabbr{pharmaceutics}\gdef\@ISSN{1999-4923}}
\DeclareOption{pharmacoepidemiology}{\gdef\@journal{pharmacoepidemiology}\gdef\@journalfull{Pharmacoepidemiology}\gdef\@journalshort{Pharmacoepidemiology}\gdef\@doiabbr{pharma}\gdef\@ISSN{2813-0618}\gdef\@continuouspages{yes}}
\DeclareOption{pharmacy}{\gdef\@journal{pharmacy}\gdef\@journalfull{Pharmacy}\gdef\@journalshort{Pharmacy}\gdef\@doiabbr{pharmacy}\gdef\@ISSN{2226-4787}}
\DeclareOption{philosophies}{\gdef\@journal{philosophies}\gdef\@journalfull{Philosophies}\gdef\@journalshort{Philosophies}\gdef\@doiabbr{philosophies}\gdef\@ISSN{2409-9287}}
\DeclareOption{photochem}{\gdef\@journal{photochem}\gdef\@journalfull{Photochem}\gdef\@journalshort{Photochem}\gdef\@doiabbr{photochem}\gdef\@ISSN{2673-7256}\gdef\@continuouspages{yes}}
\DeclareOption{photonics}{\gdef\@journal{photonics}\gdef\@journalfull{Photonics}\gdef\@journalshort{Photonics}\gdef\@doiabbr{photonics}\gdef\@ISSN{2304-6732}}
\DeclareOption{phycology}{\gdef\@journal{phycology}\gdef\@journalfull{Phycology}\gdef\@journalshort{Phycology}\gdef\@doiabbr{phycology}\gdef\@ISSN{2673-9410}\gdef\@continuouspages{yes}}
\DeclareOption{physchem}{\gdef\@journal{physchem}\gdef\@journalfull{Physchem}\gdef\@journalshort{Physchem}\gdef\@doiabbr{physchem}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{physics}{\gdef\@journal{physics}\gdef\@journalfull{Physics}\gdef\@journalshort{Physics}\gdef\@doiabbr{physics}\gdef\@ISSN{2624-8174}\gdef\@continuouspages{yes}}
\DeclareOption{physiologia}{\gdef\@journal{physiologia}\gdef\@journalfull{Physiologia}\gdef\@journalshort{Physiologia}\gdef\@doiabbr{physiologia}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{plants}{\gdef\@journal{plants}\gdef\@journalfull{Plants}\gdef\@journalshort{Plants}\gdef\@doiabbr{plants}\gdef\@ISSN{2223-7747}}
\DeclareOption{plasma}{\gdef\@journal{plasma}\gdef\@journalfull{Plasma}\gdef\@journalshort{Plasma}\gdef\@doiabbr{plasma}\gdef\@ISSN{2571-6182}\gdef\@continuouspages{yes}}
\DeclareOption{platforms}{\gdef\@journal{platforms}\gdef\@journalfull{Platforms}\gdef\@journalshort{Platforms}\gdef\@doiabbr{platforms}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{pollutants}{\gdef\@journal{pollutants}\gdef\@journalfull{Pollutants}\gdef\@journalshort{Pollutants}\gdef\@doiabbr{pollutants}\gdef\@ISSN{2673-4672}\gdef\@continuouspages{yes}}
\DeclareOption{polymers}{\gdef\@journal{polymers}\gdef\@journalfull{Polymers}\gdef\@journalshort{Polymers}\gdef\@doiabbr{polym}\gdef\@ISSN{2073-4360}}
\DeclareOption{polysaccharides}{\gdef\@journal{polysaccharides}\gdef\@journalfull{Polysaccharides}\gdef\@journalshort{Polysaccharides}\gdef\@doiabbr{polysaccharides}\gdef\@ISSN{2673-4176}\gdef\@continuouspages{yes}}
\DeclareOption{poultry}{\gdef\@journal{poultry}\gdef\@journalfull{Poultry}\gdef\@journalshort{Poultry}\gdef\@doiabbr{poultry}\gdef\@ISSN{2674-1164}\gdef\@continuouspages{yes}}
\DeclareOption{powders}{\gdef\@journal{powders}\gdef\@journalfull{Powders}\gdef\@journalshort{Powders}\gdef\@doiabbr{powders}\gdef\@ISSN{2674-0516}\gdef\@continuouspages{yes}}
\DeclareOption{preprints}{\gdef\@journal{preprints}\gdef\@journalfull{Preprints}\gdef\@journalshort{Preprints}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{proceedings}{\gdef\@journal{proceedings}\gdef\@journalfull{Proceedings}\gdef\@journalshort{Proceedings}\gdef\@doiabbr{proceedings}\gdef\@ISSN{2504-3900}}
\DeclareOption{processes}{\gdef\@journal{processes}\gdef\@journalfull{Processes}\gdef\@journalshort{Processes}\gdef\@doiabbr{pr}\gdef\@ISSN{2227-9717}}
\DeclareOption{prosthesis}{\gdef\@journal{prosthesis}\gdef\@journalfull{Prosthesis}\gdef\@journalshort{Prosthesis}\gdef\@doiabbr{prosthesis}\gdef\@ISSN{2673-1592}\gdef\@continuouspages{yes}}
\DeclareOption{proteomes}{\gdef\@journal{proteomes}\gdef\@journalfull{Proteomes}\gdef\@journalshort{Proteomes}\gdef\@doiabbr{proteomes}\gdef\@ISSN{2227-7382}}
\DeclareOption{psf}{\gdef\@journal{psf}\gdef\@journalfull{Physical Sciences Forum}\gdef\@journalshort{Phys. Sci. Forum}\gdef\@doiabbr{psf}\gdef\@ISSN{2673-9984}}
\DeclareOption{psych}{\gdef\@journal{psych}\gdef\@journalfull{Psych}\gdef\@journalshort{Psych}\gdef\@doiabbr{psych}\gdef\@ISSN{2624-8611}\gdef\@continuouspages{yes}}
\DeclareOption{psychiatryint}{\gdef\@journal{psychiatryint}\gdef\@journalfull{Psychiatry International}\gdef\@journalshort{Psychiatry Int.}\gdef\@doiabbr{psychiatryint}\gdef\@ISSN{2673-5318}\gdef\@continuouspages{yes}}
\DeclareOption{psychoactives}{\gdef\@journal{psychoactives}\gdef\@journalfull{Psychoactives}\gdef\@journalshort{Psychoactives}\gdef\@doiabbr{psychoactives}\gdef\@ISSN{2813-1851}\gdef\@continuouspages{yes}}
\DeclareOption{publications}{\gdef\@journal{publications}\gdef\@journalfull{Publications}\gdef\@journalshort{Publications}\gdef\@doiabbr{publications}\gdef\@ISSN{2304-6775}}
\DeclareOption{quantumrep}{\gdef\@journal{quantumrep}\gdef\@journalfull{Quantum Reports}\gdef\@journalshort{Quantum Rep.}\gdef\@doiabbr{quantum}\gdef\@ISSN{2624-960X}\gdef\@continuouspages{yes}}
\DeclareOption{quaternary}{\gdef\@journal{quaternary}\gdef\@journalfull{Quaternary}\gdef\@journalshort{Quaternary}\gdef\@doiabbr{quat}\gdef\@ISSN{2571-550X}}
\DeclareOption{qubs}{\gdef\@journal{qubs}\gdef\@journalfull{Quantum Beam Science}\gdef\@journalshort{Quantum Beam Sci.}\gdef\@doiabbr{qubs}\gdef\@ISSN{2412-382X}}
\DeclareOption{radiation}{\gdef\@journal{radiation}\gdef\@journalfull{Radiation}\gdef\@journalshort{Radiation}\gdef\@doiabbr{radiation}\gdef\@ISSN{2673-592X}\gdef\@continuouspages{yes}}
\DeclareOption{reactions}{\gdef\@journal{reactions}\gdef\@journalfull{Reactions}\gdef\@journalshort{Reactions}\gdef\@doiabbr{reactions}\gdef\@ISSN{2624-781X}\gdef\@continuouspages{yes}}
\DeclareOption{receptors}{\gdef\@journal{receptors}\gdef\@journalfull{Receptors}\gdef\@journalshort{Receptors}\gdef\@doiabbr{receptors}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{recycling}{\gdef\@journal{recycling}\gdef\@journalfull{Recycling}\gdef\@journalshort{Recycling}\gdef\@doiabbr{recycling}\gdef\@ISSN{2313-4321}}
\DeclareOption{regeneration}{\gdef\@journal{regeneration}\gdef\@journalfull{Regeneration}\gdef\@journalshort{Regeneration}\gdef\@doiabbr{regeneration}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{religions}{\gdef\@journal{religions}\gdef\@journalfull{Religions}\gdef\@journalshort{Religions}\gdef\@doiabbr{rel}\gdef\@ISSN{2077-1444}}
\DeclareOption{remotesensing}{\gdef\@journal{remotesensing}\gdef\@journalfull{Remote Sensing}\gdef\@journalshort{Remote Sens.}\gdef\@doiabbr{rs}\gdef\@ISSN{2072-4292}}
\DeclareOption{reports}{\gdef\@journal{reports}\gdef\@journalfull{Reports}\gdef\@journalshort{Reports}\gdef\@doiabbr{reports}\gdef\@ISSN{2571-841X}}
\DeclareOption{reprodmed}{\gdef\@journal{reprodmed}\gdef\@journalfull{Reproductive Medicine}\gdef\@journalshort{Reprod. Med.}\gdef\@doiabbr{reprodmed}\gdef\@ISSN{2673-3897}\gdef\@continuouspages{yes}}
\DeclareOption{resources}{\gdef\@journal{resources}\gdef\@journalfull{Resources}\gdef\@journalshort{Resources}\gdef\@doiabbr{resources}\gdef\@ISSN{2079-9276}}
\DeclareOption{rheumato}{\gdef\@journal{rheumato}\gdef\@journalfull{Rheumato}\gdef\@journalshort{Rheumato}\gdef\@doiabbr{rheumato}\gdef\@ISSN{2674-0621}\gdef\@continuouspages{yes}}
\DeclareOption{risks}{\gdef\@journal{risks}\gdef\@journalfull{Risks}\gdef\@journalshort{Risks}\gdef\@doiabbr{risks}\gdef\@ISSN{2227-9091}}
\DeclareOption{robotics}{\gdef\@journal{robotics}\gdef\@journalfull{Robotics}\gdef\@journalshort{Robotics}\gdef\@doiabbr{robotics}\gdef\@ISSN{2218-6581}}
\DeclareOption{ruminants}{\gdef\@journal{ruminants}\gdef\@journalfull{Ruminants}\gdef\@journalshort{Ruminants}\gdef\@doiabbr{ruminants}\gdef\@ISSN{2673-933X}\gdef\@continuouspages{yes}}
\DeclareOption{safety}{\gdef\@journal{safety}\gdef\@journalfull{Safety}\gdef\@journalshort{Safety}\gdef\@doiabbr{safety}\gdef\@ISSN{2313-576X}}
\DeclareOption{sci}{\gdef\@journal{sci}\gdef\@journalfull{Sci}\gdef\@journalshort{Sci}\gdef\@doiabbr{sci}\gdef\@ISSN{2413-4155}}
\DeclareOption{scipharm}{\gdef\@journal{scipharm}\gdef\@journalfull{Scientia Pharmaceutica}\gdef\@journalshort{Sci. Pharm.}\gdef\@doiabbr{scipharm}\gdef\@ISSN{2218-0532}}
\DeclareOption{sclerosis}{\gdef\@journal{sclerosis}\gdef\@journalfull{Sclerosis}\gdef\@journalshort{Sclerosis}\gdef\@doiabbr{sclerosis}\gdef\@ISSN{2813-3064}\gdef\@continuouspages{yes}}
\DeclareOption{seeds}{\gdef\@journal{seeds}\gdef\@journalfull{Seeds}\gdef\@journalshort{Seeds}\gdef\@doiabbr{seeds}\gdef\@ISSN{2674-1024}\gdef\@continuouspages{yes}}
\DeclareOption{sensors}{\gdef\@journal{sensors}\gdef\@journalfull{Sensors}\gdef\@journalshort{Sensors}\gdef\@doiabbr{s}\gdef\@ISSN{1424-8220}}
\DeclareOption{separations}{\gdef\@journal{separations}\gdef\@journalfull{Separations}\gdef\@journalshort{Separations}\gdef\@doiabbr{separations}\gdef\@ISSN{2297-8739}}
\DeclareOption{sexes}{\gdef\@journal{sexes}\gdef\@journalfull{Sexes}\gdef\@journalshort{Sexes}\gdef\@doiabbr{sexes}\gdef\@ISSN{2411-5118}\gdef\@continuouspages{yes}}
\DeclareOption{signals}{\gdef\@journal{signals}\gdef\@journalfull{Signals}\gdef\@journalshort{Signals}\gdef\@doiabbr{signals}\gdef\@ISSN{2624-6120}\gdef\@continuouspages{yes}}
\DeclareOption{sinusitis}{\gdef\@journal{sinusitis}\gdef\@journalfull{Sinusitis}\gdef\@journalshort{Sinusitis}\gdef\@doiabbr{sinusitis}\gdef\@ISSN{2309-107X}\gdef\@continuouspages{yes}}
\DeclareOption{skins}{\gdef\@journal{skins}\gdef\@journalfull{Skins}\gdef\@journalshort{Skins}\gdef\@doiabbr{skins}\gdef\@ISSN{}}
\DeclareOption{smartcities}{\gdef\@journal{smartcities}\gdef\@journalfull{Smart Cities}\gdef\@journalshort{Smart Cities}\gdef\@doiabbr{smartcities}\gdef\@ISSN{2624-6511}\gdef\@continuouspages{yes}}
\DeclareOption{sna}{\gdef\@journal{sna}\gdef\@journalfull{Sinusitis and Asthma}\gdef\@journalshort{Sinusitis Asthma}\gdef\@doiabbr{sna}\gdef\@ISSN{2624-7003}}
\DeclareOption{societies}{\gdef\@journal{societies}\gdef\@journalfull{Societies}\gdef\@journalshort{Societies}\gdef\@doiabbr{soc}\gdef\@ISSN{2075-4698}}
\DeclareOption{socsci}{\gdef\@journal{socsci}\gdef\@journalfull{Social Sciences}\gdef\@journalshort{Soc. Sci.}\gdef\@doiabbr{socsci}\gdef\@ISSN{2076-0760}}
\DeclareOption{software}{\gdef\@journal{software}\gdef\@journalfull{Software}\gdef\@journalshort{Software}\gdef\@doiabbr{software}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{soilsystems}{\gdef\@journal{soilsystems}\gdef\@journalfull{Soil Systems}\gdef\@journalshort{Soil Syst.}\gdef\@doiabbr{soilsystems}\gdef\@ISSN{2571-8789}}
\DeclareOption{solar}{\gdef\@journal{solar}\gdef\@journalfull{Solar}\gdef\@journalshort{Solar}\gdef\@doiabbr{solar}\gdef\@ISSN{2673-9941}\gdef\@continuouspages{yes}}
\DeclareOption{solids}{\gdef\@journal{solids}\gdef\@journalfull{Solids}\gdef\@journalshort{Solids}\gdef\@doiabbr{solids}\gdef\@ISSN{2673-6497}\gdef\@continuouspages{yes}}
\DeclareOption{spectroscj}{\gdef\@journal{spectroscj}\gdef\@journalfull{Spectroscopy Journal}\gdef\@journalshort{Spectrosc. J.}\gdef\@doiabbr{spectroscj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{sports}{\gdef\@journal{sports}\gdef\@journalfull{Sports}\gdef\@journalshort{Sports}\gdef\@doiabbr{sports}\gdef\@ISSN{2075-4663}}
\DeclareOption{standards}{\gdef\@journal{standards}\gdef\@journalfull{Standards}\gdef\@journalshort{Standards}\gdef\@doiabbr{standards}\gdef\@ISSN{2305-6703}\gdef\@continuouspages{yes}}
\DeclareOption{stats}{\gdef\@journal{stats}\gdef\@journalfull{Stats}\gdef\@journalshort{Stats}\gdef\@doiabbr{stats}\gdef\@ISSN{2571-905X}\gdef\@continuouspages{yes}}
\DeclareOption{std}{\gdef\@journal{std}\gdef\@journalfull{Surgical Techniques Development}\gdef\@journalshort{Surg. Tech. Dev.}\gdef\@doiabbr{std}\gdef\@ISSN{2038-9582}\gdef\@continuouspages{yes}}
\DeclareOption{stresses}{\gdef\@journal{stresses}\gdef\@journalfull{Stresses}\gdef\@journalshort{Stresses}\gdef\@doiabbr{stresses}\gdef\@ISSN{2673-7140}\gdef\@continuouspages{yes}}
\DeclareOption{surfaces}{\gdef\@journal{surfaces}\gdef\@journalfull{Surfaces}\gdef\@journalshort{Surfaces}\gdef\@doiabbr{surfaces}\gdef\@ISSN{2571-9637}\gdef\@continuouspages{yes}}
\DeclareOption{surgeries}{\gdef\@journal{surgeries}\gdef\@journalfull{Surgeries}\gdef\@journalshort{Surgeries}\gdef\@doiabbr{surgeries}\gdef\@ISSN{2017-2017}\gdef\@continuouspages{yes}}
\DeclareOption{suschem}{\gdef\@journal{suschem}\gdef\@journalfull{Sustainable Chemistry}\gdef\@journalshort{Sustain. Chem.}\gdef\@doiabbr{suschem}\gdef\@ISSN{2673-4079}\gdef\@continuouspages{yes}}
\DeclareOption{sustainability}{\gdef\@journal{sustainability}\gdef\@journalfull{Sustainability}\gdef\@journalshort{Sustainability}\gdef\@doiabbr{su}\gdef\@ISSN{2071-1050}}
\DeclareOption{symmetry}{\gdef\@journal{symmetry}\gdef\@journalfull{Symmetry}\gdef\@journalshort{Symmetry}\gdef\@doiabbr{sym}\gdef\@ISSN{2073-8994}}
\DeclareOption{synbio}{\gdef\@journal{synbio}\gdef\@journalfull{Synbio}\gdef\@journalshort{Synbio}\gdef\@doiabbr{synbio}\gdef\@ISSN{2674-0583}\gdef\@continuouspages{yes}}
\DeclareOption{systems}{\gdef\@journal{systems}\gdef\@journalfull{Systems}\gdef\@journalshort{Systems}\gdef\@doiabbr{systems}\gdef\@ISSN{2079-8954}}
\DeclareOption{targets}{\gdef\@journal{targets}\gdef\@journalfull{Targets}\gdef\@journalshort{Targets}\gdef\@doiabbr{targets}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{taxonomy}{\gdef\@journal{taxonomy}\gdef\@journalfull{Taxonomy}\gdef\@journalshort{Taxonomy}\gdef\@doiabbr{taxonomy}\gdef\@ISSN{2673-6500}\gdef\@continuouspages{yes}}
\DeclareOption{technologies}{\gdef\@journal{technologies}\gdef\@journalfull{Technologies}\gdef\@journalshort{Technologies}\gdef\@doiabbr{technologies}\gdef\@ISSN{2227-7080}}
\DeclareOption{telecom}{\gdef\@journal{telecom}\gdef\@journalfull{Telecom}\gdef\@journalshort{Telecom}\gdef\@doiabbr{telecom}\gdef\@ISSN{2673-4001}\gdef\@continuouspages{yes}}
\DeclareOption{test}{\gdef\@journal{test}\gdef\@journalfull{Test}\gdef\@journalshort{Test}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{textiles}{\gdef\@journal{textiles}\gdef\@journalfull{Textiles}\gdef\@journalshort{Textiles}\gdef\@doiabbr{textiles}\gdef\@ISSN{2673-7248}\gdef\@continuouspages{yes}}
\DeclareOption{thalassrep}{\gdef\@journal{thalassrep}\gdef\@journalfull{Thalassemia Reports}\gdef\@journalshort{Thalass. Rep.}\gdef\@doiabbr{thalassrep}\gdef\@ISSN{2039-4365}\gdef\@continuouspages{yes}}
\DeclareOption{thermo}{\gdef\@journal{thermo}\gdef\@journalfull{Thermo}\gdef\@journalshort{Thermo}\gdef\@doiabbr{thermo}\gdef\@ISSN{2673-7264}\gdef\@continuouspages{yes}}
\DeclareOption{tomography}{\gdef\@journal{tomography}\gdef\@journalfull{Tomography}\gdef\@journalshort{Tomography}\gdef\@doiabbr{tomography}\gdef\@ISSN{2379-139X}\gdef\@continuouspages{yes}}
\DeclareOption{tourismhosp}{\gdef\@journal{tourismhosp}\gdef\@journalfull{Tourism and Hospitality}\gdef\@journalshort{Tour. Hosp.}\gdef\@doiabbr{tourhosp}\gdef\@ISSN{2673-5768}\gdef\@continuouspages{yes}}
\DeclareOption{toxics}{\gdef\@journal{toxics}\gdef\@journalfull{Toxics}\gdef\@journalshort{Toxics}\gdef\@doiabbr{toxics}\gdef\@ISSN{2305-6304}}
\DeclareOption{toxins}{\gdef\@journal{toxins}\gdef\@journalfull{Toxins}\gdef\@journalshort{Toxins}\gdef\@doiabbr{toxins}\gdef\@ISSN{2072-6651}}
\DeclareOption{transplantology}{\gdef\@journal{transplantology}\gdef\@journalfull{Transplantology}\gdef\@journalshort{Transplantology}\gdef\@doiabbr{transplantology}\gdef\@ISSN{2673-3943}\gdef\@continuouspages{yes}}
\DeclareOption{transportation}{\gdef\@journal{transportation}\gdef\@journalfull{Transportation}\gdef\@journalshort{Transportation}\gdef\@doiabbr{transportation}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{traumacare}{\gdef\@journal{traumacare}\gdef\@journalfull{Trauma Care}\gdef\@journalshort{Trauma Care}\gdef\@doiabbr{traumacare}\gdef\@ISSN{2673-866X}\gdef\@continuouspages{yes}}
\DeclareOption{traumas}{\gdef\@journal{traumas}\gdef\@journalfull{Traumas}\gdef\@journalshort{Traumas}\gdef\@doiabbr{traumas}\gdef\@ISSN{2673-7477}\gdef\@continuouspages{yes}}
\DeclareOption{tropicalmed}{\gdef\@journal{tropicalmed}\gdef\@journalfull{Tropical Medicine and Infectious Disease}\gdef\@journalshort{Trop. Med. Infect. Dis.}\gdef\@doiabbr{tropicalmed}\gdef\@ISSN{2414-6366}}
\DeclareOption{universe}{\gdef\@journal{universe}\gdef\@journalfull{Universe}\gdef\@journalshort{Universe}\gdef\@doiabbr{universe}\gdef\@ISSN{2218-1997}}
\DeclareOption{urbansci}{\gdef\@journal{urbansci}\gdef\@journalfull{Urban Science}\gdef\@journalshort{Urban Sci.}\gdef\@doiabbr{urbansci}\gdef\@ISSN{2413-8851}}
\DeclareOption{uro}{\gdef\@journal{uro}\gdef\@journalfull{Uro}\gdef\@journalshort{Uro}\gdef\@doiabbr{uro}\gdef\@ISSN{2673-4397}\gdef\@continuouspages{yes}}
\DeclareOption{vaccines}{\gdef\@journal{vaccines}\gdef\@journalfull{Vaccines}\gdef\@journalshort{Vaccines}\gdef\@doiabbr{vaccines}\gdef\@ISSN{2076-393X}}
\DeclareOption{vehicles}{\gdef\@journal{vehicles}\gdef\@journalfull{Vehicles}\gdef\@journalshort{Vehicles}\gdef\@doiabbr{vehicles}\gdef\@ISSN{2624-8921}\gdef\@continuouspages{yes}}
\DeclareOption{venereology}{\gdef\@journal{venereology}\gdef\@journalfull{Venereology}\gdef\@journalshort{Venereology}\gdef\@doiabbr{venereology}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{vetsci}{\gdef\@journal{vetsci}\gdef\@journalfull{Veterinary Sciences}\gdef\@journalshort{Vet. Sci.}\gdef\@doiabbr{vetsci}\gdef\@ISSN{2306-7381}}
\DeclareOption{vibration}{\gdef\@journal{vibration}\gdef\@journalfull{Vibration}\gdef\@journalshort{Vibration}\gdef\@doiabbr{vibration}\gdef\@ISSN{2571-631X}\gdef\@continuouspages{yes}}
\DeclareOption{virtualworlds}{\gdef\@journal{virtualworlds}\gdef\@journalfull{Virtual Worlds}\gdef\@journalshort{Virtual Worlds}\gdef\@doiabbr{virtualworlds}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{viruses}{\gdef\@journal{viruses}\gdef\@journalfull{Viruses}\gdef\@journalshort{Viruses}\gdef\@doiabbr{v}\gdef\@ISSN{1999-4915}}
\DeclareOption{vision}{\gdef\@journal{vision}\gdef\@journalfull{Vision}\gdef\@journalshort{Vision}\gdef\@doiabbr{vision}\gdef\@ISSN{2411-5150}}
\DeclareOption{waste}{\gdef\@journal{waste}\gdef\@journalfull{Waste}\gdef\@journalshort{Waste}\gdef\@doiabbr{waste}\gdef\@ISSN{2813-0391}\gdef\@continuouspages{yes}}
\DeclareOption{water}{\gdef\@journal{water}\gdef\@journalfull{Water}\gdef\@journalshort{Water}\gdef\@doiabbr{w}\gdef\@ISSN{2073-4441}}
\DeclareOption{wem}{\gdef\@journal{wem}\gdef\@journalfull{Wildlife Ecology and Management}\gdef\@journalshort{Wildl. Ecol. Manag.}\gdef\@doiabbr{}\gdef\@ISSN{1234-4321}}
\DeclareOption{wevj}{\gdef\@journal{wevj}\gdef\@journalfull{World Electric Vehicle Journal}\gdef\@journalshort{World Electr. Veh. J.}\gdef\@doiabbr{wevj}\gdef\@ISSN{2032-6653}}
\DeclareOption{wind}{\gdef\@journal{wind}\gdef\@journalfull{Wind}\gdef\@journalshort{Wind}\gdef\@doiabbr{wind}\gdef\@ISSN{2674-032X}\gdef\@continuouspages{yes}}
\DeclareOption{women}{\gdef\@journal{women}\gdef\@journalfull{Women}\gdef\@journalshort{Women}\gdef\@doiabbr{women}\gdef\@ISSN{2673-4184}\gdef\@continuouspages{yes}}
\DeclareOption{world}{\gdef\@journal{world}\gdef\@journalfull{World}\gdef\@journalshort{World}\gdef\@doiabbr{world}\gdef\@ISSN{2673-4060}\gdef\@continuouspages{yes}}
\DeclareOption{youth}{\gdef\@journal{youth}\gdef\@journalfull{Youth}\gdef\@journalshort{Youth}\gdef\@doiabbr{youth}\gdef\@ISSN{2673-995X}\gdef\@continuouspages{yes}}
\DeclareOption{zoonoticdis}{\gdef\@journal{zoonoticdis}\gdef\@journalfull{Zoonotic Diseases}\gdef\@journalshort{Zoonotic Dis.}\gdef\@doiabbr{zoonoticdis}\gdef\@ISSN{2813-0227}\gdef\@continuouspages{yes}}


==> algoritems/3_main_algorithm.tex <==
\begin{algorithm}[t]
	\caption{Skew Class-balanced Effective Number}
	\label{al:effective} 
	\begin{algorithmic}[1]
		\Require Dataset $\mathcal{D}$, SGG Model $f_{\theta}$
		\For {$t=0,1,2,\ldots,T$}
		\State $\mathcal{B} \leftarrow$ Minibatch($\mathcal{D}$)
		\State $\hat{\bs{R}}_{skew} \leftarrow Skew\_Logits(\hat{\bs{R}}_{freq}, \hat{\bs{R}}_{emb};\mathcal{B}, f_\theta)$~~~~~~~~~~~ (Eq. \ref{eq:skewness})
		\State $\mathcal{M} \leftarrow Sample\_Estimates(\hat{\bs{R}}_{skew})$ ~~~~~~~~~~~~~~~~~~~~~~~~ (Eq. \ref{eq:predicate_effective})
		\State $\bs{S}_{skew} \leftarrow Skew(\hat{\bs{R}}_{skew},\bs{R})$ ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\;\;(Eq. \ref{eq:skew})
		\State $\bs{H}_{skew} \leftarrow Entropy(\hat{\bs{R}}_{skew})$ ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~(Eq. \ref{eq:entropy})
		\If {$\bs{S}_{skew} > S_{th}$}
		\State $\bs{\beta} = \bs{1.0} - \bs{H}_{skew}$
		\Else
		\State $\bs{\beta} = \bs{0.0}$
		\EndIf
		\State $E^i_{m_y} = \frac{1-\beta_i^{m_y}}{1-\beta_i} \text{ ; } m_y \in \mathcal{M}, i \in \left[0, \mathcal{N}(\mathcal{N}-1) \right)$ ~~~~~~~~(Eq. \ref{eq:effec})
		\EndFor
	\end{algorithmic} 
\end{algorithm}

==> figures/1_main_intro.tex <==
\begin{figure}[t]
	\centering
    %\begin{subfigmatrix}
	\begin{subfigure}{.98\textwidth}
		%\centering
		\includegraphics[width=\textwidth]{./img/predicates}
		\caption{The Long-tailed Predicate Distribution.}
		\label{fig:imbalance}
	\end{subfigure}
    \par\bigskip
	\begin{subfigure}{.98\textwidth}
		%\centering
		\includegraphics[width=\linewidth]{img/man-board}
		\caption{The Predicate Distribution of the \textcolor{orange}{\textit{Subject - Object}} Pair.}
		\label{fig:subj_obj}
	\end{subfigure}
    %\end{subfigmatrix}
	\caption{The Long-tailed Predicate Distribution: (a) The predicate proportion of the Visual Genome~\cite{xu2017scene}, where backgrounds are possibly far more than others and (b) The possible predicates of a \textcolor{orange}{\textit{man - board}} pair.}
	% The majority predicates are more frequently observed than the minority ones. Given a \textcolor{orange}{\textit{man - board}} pair, the possible predicates- \textcolor{cyan}{\textit{backgrounds, on, holding, riding, etc.}} represents a long-tail distribution.}
	\label{fig:three_graphs}
\end{figure}
%\vspace{-0.1cm}

==> figures/3_main_model.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth, trim=1. 1. 1. 2., clip]{img/model}
	%\includegraphics[width=1.0\linewidth]{img/model}
	\caption{Skew Class-balanced Re-weighting (SCR) For Unbiased SGG models. Based on (a) object detection, the SGG model predicts \textcolor{red}{(d) predicates} of \textcolor{red}{(b) FREQ} and \textcolor{red}{(c) visual predictions}; Unbiased SGG is trained by \textcolor{cyan}{(g) target sample weight}, which is estimated by \textcolor{cyan}{(f) skew measures} of \textcolor{cyan}{(e) possible sample estimates}.}
	%\caption{Skew Class-balanced Re-weighting (SCR) For Unbiased SGG models. The traditional SGG model and \textcolor{red}{(d) predicate prediction} ($\hat{\bm{R}}$): (a) object detector outputs its predictions: \textcolor{orange}{\textit{man}} and \textcolor{orange}{\textit{hourse}}, (b) FREQ embeds prior predicates and (c) predicate model outputs predicate predictions ($\hat{\bm{R}}_{vis}$); Given \textcolor{orange}{\textit{man - horse}} label predictions, our SCR estimates (e) a sample size of the possible predicate candidates through FREQ ($\bm{R}_{freq}$ or $\bm{R}_{emb}$ ) and measures (f) the target label skew score and then calculates (g) the training target sample weight for the adaptive re-weighted loss, and in (f) and (g), \textcolor{red}{red lines} around the target label indicate \textcolor{red}{predicate skew} ($S^i_{skew}$) and \textcolor{red}{re-weight scores} ($\bm{W}^i$), respectively, where they have an approximately inverse relationship.}
	\label{fig:model}
\end{figure*}

==> figures/3_main_skew_balance.tex <==
\begin{figure}[tp]
	\centering
	\begin{subfigure}{.98\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./img/weights/softmax}
		\caption{The Predicate Biased Logits, $softmax(\hat{\bs{R}}_{skew})$.}
		\label{fig:skew_softmax}
	\end{subfigure}
	\par\bigskip
	\begin{subfigure}{.98\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./img/weights/weight}
		\caption{The Predicate Weights, $\bs{W}=\bs{1}/\bs{E}_{m_y}$.}
		\label{fig:skew_weight}
	\end{subfigure}
	\par\bigskip
	\begin{subfigure}{.98\textwidth}
		\centering
		\includegraphics[width=\linewidth]{img/weights/skew}
		\caption{The Predicate Target Label-Wise Skew, $\bs{S}_{skew}$}
		\label{fig:skew_entropy}	
	\end{subfigure}
	\caption{The Biased Predicate Weights: (a) the predicate biased logits $\hat{\bm{R}}_{skew}$ of label frequency $\mathcal{M}^{1/5}$, depending on entropy $H_{skew}$, (b) the sensitivity of sample weights $\bm{W}$, according to entropy $H_{skew}$, and (c) the skew measures $\bm{S}_{skew}$ of a target label $r_y$.}
	%\caption{The Biased Predicate Weights: (a) an assumption that the predicate biased logits are represented by its frequency $\mathcal{M}^{1/5}$ and that the degree of biased predictions is also modeled by its entropy $H_{skew}$, (b) the discrete sample weights are assigned to the minority predicates according to the entropy $H_{skew}$ and (c) the skew in Eq. \ref{eq:skew} measures not only the degree of true/false prediction but also biased predictions; the true prediction has the negative skew $S_{skew} < 0$ while others do not.}
	\label{fig:skew_weight_entropy}
\end{figure}

==> figures/4_main_qaul_weight.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.98\textwidth]{./img/experiments/transform_predcls}
	\caption{The Recall@100 on PredCls: we compare the SCR of FREQ+EMB with CogTree using the SG-Transformer \cite{yu2020cogtree}. }
	%\caption{The Recall@100 on PredCls: we compare the Skew Class-balanced Re-weight (SCR) of FREQ+EMB with the Re-weighting method (CogTree), based on the SG-Transformer \cite{yu2020cogtree}. }
	\label{fig:qual_weight}
\end{figure}

==> figures/4_main_skew_prods.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.98\textwidth, trim=4.0 3.0 2.0 3.0, clip]{./img/experiments/skew_preds}
	\caption{The Predicate Predictions and Sample Estimates: when the \textit{woman-coat} pair (upper) have possible predicates such as \textit{has, wearing, in}, etc., we show predicate predictions $\hat{\bs{R}}_i$ with its target skew $S^i_{skew}$ deduced by its sample estimates $\hat{\bs{R}}^i_{skew}$. The larger $\hat{R}^i_{skew} \in \hat{\bs{R}}^i_{skew}$ tends to be a smaller $S^i_{skew}$, when compared to the \textit{hill-snow} pair (lower). }
	\label{fig:qual_skew_preds}
\end{figure}

==> figures/5_main_pred_weight.tex <==
\begin{figure}[t]
	\centering
	\begin{subfigure}{.97\textwidth}
		\centering
		\includegraphics[width=\textwidth]{experiments/woman-coat/1294_1_woman-coat_freqs.pdf}
	\end{subfigure}
	%\par\bigskip
	\begin{subfigure}{.98\textwidth}
		\centering
		\includegraphics[width=\textwidth]{experiments/woman-coat/1294_1_woman-coat_preds.pdf}
		%\caption{The Predicate Weights, $\bs{W}=\bs{1}/\bs{E}_{m_y}$.}
		%\label{fig:skew_weight}
	\end{subfigure}
    \begin{subfigure}{.97\textwidth}
		\centering
		\includegraphics[width=\textwidth]{experiments/covered_in/hill-snow/1097_20_hill-snow_freqs.pdf}
	\end{subfigure}
	%\par\bigskip
	\begin{subfigure}{.98\textwidth}
		\centering
		\includegraphics[width=\textwidth]{experiments/covered_in/hill-snow/1097_20_hill-snow_preds.pdf}
		%\caption{The Predicate Weights, $\bs{W}=\bs{1}/\bs{E}_{m_y}$.}
		%\label{fig:skew_weight}
	\end{subfigure}
	
	\caption{The Predicate Predictions and Sample Estimates: in a SCR-trained SGG model, the larger $\hat{R}^i_{skew}$ tends to be a smaller $S^i_{skew}$, i.e., \textcolor{orange}{\textit{woman} -} \textcolor{green}{$S^{\text{wearing}}_{skew}$}  \textcolor{orange}{- coat} (upper) < \textcolor{orange}{\textit{hill -}} \textcolor{green}{$S^{\text{covered in}}_{skew}$} \textcolor{orange}{- snow} (lower). }

	%\caption{The Predicate Predictions and Sample Estimates: when one \textcolor{orange}{\textit{woman} -} \textcolor{green}{wearing}  \textcolor{orange}{- coat} pair (upper) have possible predicates such as \textcolor{cyan}{\textit{backgrounds, has, wearing, in}, etc.}, we show \textcolor{violet}{predicate predictions $\hat{\bs{R}}_i$} with its \textcolor{green}{target skew $S^i_{skew}$} deduced by its \textcolor{red}{sample estimates $\hat{\bs{R}}^i_{skew}$}. The larger $\hat{R}^i_{skew} \in \hat{\bs{R}}^i_{skew}$ tends to be a smaller $S^i_{skew}$, when compared to another \textcolor{orange}{\textit{hill -}} \textcolor{green}{covered in}  \textcolor{orange}{- snow} pair (lower) in a finetuned-SGG model. }
	\label{fig:qual_skew_preds}
\end{figure}

==> materials/0_abstract.tex <==
\abstract{
An unbiased scene graph generation (SGG) algorithm referred to as Skew Class-balanced Re-weighting (SCR) is proposed for considering the unbiased predicate prediction caused by the long-tailed distribution. The prior works focus mainly on alleviating the deteriorating performances of the minority predicate predictions, showing drastic dropping recall scores, i.e., losing the majority predicate performances. It has not yet correctly analyzed the trade-off between majority and minority predicate performances in the limited SGG datasets. In this paper, to alleviate the issue, the \textit{Skew Class-balanced Re-weighting} (SCR) loss function is considered for the unbiased SGG models. Leveraged by the skewness of biased predicate predictions, the SCR estimates the target predicate weight coefficient and then re-weights more to the biased predicates for better trading-off between the majority predicates and the minority ones. Extensive experiments conducted on the standard Visual Genome dataset and Open Image V4 \& V6 show the performances and generality of the SCR with the traditional SGG models. The source code is available at \url{https://github.com/ihaeyong/Unbiased-SGG}.
}

==> materials/1_introduction.tex <==
\section{Introduction}

Currently, computer vision~\cite{jarvis1983perspective, forsyth2002computer, voulodimos2018deep, s23031713, hoye2021deep, guo2022attention} has been prevalent in various fields: material ~\cite{sethian1999level}, chemical~\cite{scheuerman2021datasets, verma2022varscene}, and medical science~\cite{esteva2021deep}. Of great interest are tasks related to classifying and detecting objects by classical neural networks~\cite{Andriyanov2022DetectionOO, pmlr-v108-dutordoir20a, PAPAKOSTAS201790, joseph2021towards, wang2022yolov7}. With the development of computer vision, graph neural networks~\cite{Zhang2021biased, zhang2022greaselm, wu2022discovering, pmlr-v162-gao22e, minji2022, math10214021, ZHOU202057} and multimodal text and image models~\cite{Chen_2022_CVPR, Ding_2022_CVPR, Lou_2022_CVPR, Walmer_2022_CVPR, Koh2023, s21041270} have also been intensely investigated. However, there is less information on Scene Graph Generation (SGG) models in the literature. For this reason, SGG has recently been receiving increased attention for improving image comprehension, divided into two approaches: one-stage \cite{liu2021fully, cong2022} and two-stage~\cite{xu2017scene,dai2017detecting,li2017scene,li2017vip,jae2018tensorize,li2018factorizable,yang2018graph,yin2018zoom,woo2018linknet,wang2019exploring,tang2019learning,chen2019counterfactual,tang2020unbiased,desai2021learning,suhail2021energy}. The core building blocks of SGG are the objects in the image. There can be diverse relationships among the objects~\cite{chen2019knowledge,lin2020gps}. All relationships can be represented as triplets \textit{subject}, \textit{relation}, \textit{object}, which can be used for generating the scene graph. The precise interpretation of an image depends on the core relations between the \textit{subject-object} pairs. For example, given an image of \textit{dog, woman, kite} objects, the image can be interpreted in multiple ways such as $\left<\textit{dog}, \textit{has}, \textit{leg} \right>$,  $\left<\textit{dog}, \textit{near}, \textit{woman} \right>$, and $\left<\textit{woman}, \textit{holding}, \textit{kite} \right>$. 

%\noindent
In general, however, the real-world large data sets often have shown long-tailed predicate distributions as depicted in Fig.~\ref{fig:imbalance} - the predicate proportion of the Visual Genome~\cite{xu2017scene}, containing $51$ predicates. One cause of long-tail distribution is the background predicates. The background predicates account for more than $80\%$ in total predicates since it is not trivial to annotate all possible relationships, leading to possibly far more \textit{subject}-\textit{object} pairs without annotating ground truth than ones with ground truth labels. Another reason is the visual event frequency, as shown in Fig.~\ref{fig:subj_obj}. The majority predicates more frequently occur than the minority ones given a visual \textit{subject-object} pair in the real-world scene. For example, given a $\textit{man-board}$ pair, the possible predicates - \textcolor{cyan}{\textit{backgrounds, on, holding, riding, etc.}} represents a long-tail distribution. The predicate $\textit{on}$ is more frequently observed than $\textit{holding}$ and $\textit{riding}$. 

\input{figures/1_main_intro}

%\noindent
This long-tailed label distribution causes the trained model to tend to be biased toward the majority predicates. The SGG models~\cite{tang2020unbiased, yu2020cogtree, Li_2021_CVPR, yan2020pcpl, chiou2021recovering, guo2021general} focus on increasing the minority predicate performances for the unbiased scene graph generation, i.e., increasing mean recall scores. However, these methods lead to deteriorating performances of the majority predicates, drastically dropping recall scores, i.e., losing the majority predicate performances. Recently, the issue has been alleviated through resampling images and object instances~\cite{li2021bipartite}. However, this method needs more computing power and time to train the model on the resampled samples. The current state-of-the-art models focus on re-balancing biased loss~\cite{li2022ppdl} or correcting noisy labels~\cite{li2022devil} to acquire an unbiased SGG model. Nevertheless, the prior works have not yet adequately described and analyzed the trade-off performances between majority and minority predicates for learning SGG models based on the given imbalanced datasets. 

%\noindent
In this paper, the \textit{Skew Class-balanced Re-weighting} (SCR) loss function is considered for alleviating the issues and acquiring the best trade-off performances in the multiple SGG tasks. Leveraged by the skewness of predicate predictions, the SCR estimates its weight coefficients and then reweights more to biased predicate samples to adaptively be unbiased SGG models. The extensive experimental results show that the SCR loss function gives more generalized performances than priors in the multiple SGG tasks on the Visual Genome dataset~\cite{krishna2017visual} and the Open Images datasets~\cite{kuznetsova2020open}. \\ 

\noindent
\textbf{Contributions of our SCR} learning scheme to unbiased SGG models:

\begin{itemize}
	\item Leveraged by the skewness of biased predicate predictions, the \textit{Skew Class-balanced Re-weighting} (SCR) loss function is firstly proposed for the unbiased scene graph generation (SGG) models.
	\item The SCR is applied to the current state-of-the-art SGG models to show its effectiveness, leading to more generalized performances: the SCR outperforms the prior reweighted methods on both mean recall and recall measurements in the multiple SGG tasks.
\end{itemize}

%\noindent 
This paper is organized as follows. The Related Work section provides discussions on unbiased scene graph generation. The unbiased SGG section presents scene graph generation. In the Skew Class-balanced Re-weighting (SCR) section, the SCR loss function is depicted in detail. In the experimental section, the results of scene graph generation on the Visual Genome and Open Image V4 \& V6 dataset are examined, along with an analysis and ablation study on the SCR with the current state-of-the-art SGG models. Finally, we conclude.


==> materials/2_related_works.tex <==
\section{Related Works.}\label{sec2:related_work}

% Imbalanced Relational Distributions
\noindent
\textbf{Unbiased Scene Graph Generation (SGG)}. Predicate distribution is much more long-tailed than object distribution. For $N$ objects and $R$ predicates, the model has to address the fundamental challenge of learning $O(N^2R)$ relations with few~\cite{zhan2019exploring,sadeghi2011recognition}. To overcome the limited training dataset, the linguistic external knowledge ~\cite{zhan2019exploring,yin2018zoom,gu2019scene} was used by~\citet{yu2017visual}, regularizing the deep neural network; using linguistic knowledge, the probabilistic model has also alleviated the semantical ambiguity of visual relationships~\cite{yang2021probabilistic}. Furthermore, to alleviate the imbalanced relationship distribution, \citet{yin2018zoom} reformulated the conventional one-hot classification as a $n$-hot multiclass hierarchical recognition via a novel Intra-Hierarchical trees (IH-trees) for each label set in the triplet $\left<subject, predicate, object\right>$. Recently, unbiased SGG~\cite{lin2020gps, yu2020cogtree, tang2020unbiased, Li_2021_CVPR, li2022ppdl, li2022devil, yan2020pcpl, chiou2021recovering, guo2021general, lyu2022fine, dong2022stacked, goel2022not, li2022dynamic, teng2022structured, zhang2022fine, lin2022ru, yang2022panoptic, deng2022hierarchical, he2022towards} has drawn unprecedented interest for more generalized SGG models. Occurrence-based Node Priority Sensitive (NPS)-loss~\cite{lin2020gps} was used for balancing predictions; the Total Direct Effect (TDE) method has proposed firstly for unbiased learning by~\citet{tang2020unbiased}, which directly separates the bias from biased predictions through the counterfactual methodologies on causal graphs; CogTree~\cite{yu2020cogtree} addressed the debiasing issue based on the coarse-to-fine structure of the relationships from the cognition viewpoint; \citet{Li_2021_CVPR} improved the context modeling for tail categories by designing the bipartite graph network and message propagation on resampled objects and images. Lastly, the Predicate Probability Distribution based Loss (PPDL)~\cite{li2022ppdl} has proposed to train the biased SGG models, which measure the semantic predicate representation to re-balance the biased training loss. In this work, the \textit{Skew Class-balanced Re-weighting} (SCR) loss function is proposed for alleviating biased predicate predictions, leading to the most generalized SGG models through the novel adaptive re-weighting learning scheme. \\

\noindent
\textbf{Re-Weighting based Unbiased SGG.} 
Overall unbiased SGG models can be categorized into re-balancing strategy of re-weighting~\cite{lin2020gps, yan2020pcpl, yu2020cogtree, li2022ppdl} and re-sampling~\cite{Li_2021_CVPR} and biased model-based strategy~\cite{tang2020unbiased, chiou2021recovering, guo2021general}. For unbiased SGG modes, \citet{tang2020unbiased} first investigated the re-weighting learning algorithm. However, they observed that the performances of the majority predicates were drastically dropped, resulting in low recall scores while with high mean recall scores. This shows the general tendency that there is a trade-off performance between majority predicates and minority ones. To alleviate the trade-off issue, \citet{yu2020cogtree} proposed CogTree based on the coarse-to-fine structure of the relationships from the cognition viewpoint. Recently, the Predicate Probability Distribution (PPD)~\cite{li2022ppdl} re-balances the biased training loss according to the similarity between the predicted probability distribution and the estimated one. However, it has not yet correctly analyzed the trade-off performances between the majority and minority classes in various SGG tasks. In this paper, we measure the sample skew score based on the sample estimates for bias toward the majority classes to assign the sample weight correctly. The sample skewness is computed as the Fisher-Pearson coefficient of skewness on its sample mean value~\cite{brown2011measures}. However, since the mean value tends to be biased toward the majority predicates, we measure the sample skew score fairly on its target logit instead of its mean value. Based on the sample skew score, the SCR assigns the sample weights adaptively - if there is no bias,  we assign fewer weights to the sample (majority). If it is biased to one side, we assign larger weights to the samples (minority). Such that the SGG models with SCR show superior performances and generality on the multiple SGG tasks.

%\noindent
%We set more current models to show our effectiveness as follows as:
%\begin{itemize}

% cvpr2022-trade-off, re-balancing the biased training
%\item The Predicate Probability Distribution based Loss (PPDL)~\cite{li2022ppdl} has proposed to train the biased SGG models and obtain unbiased Scene Graphs ultimately. First, they considered PPD the semantic representation of a particular predicate class, then re-balance the biased training loss according to the similarity between the predicted probability distribution and the estimated one. 

% cvpr2022-trade-off, refined predicate labels
%\item \citet{li2022devil} propose a novel model agnostic NoIsy label CorrEction (NICE) strategy for SGG. NICE can not only detect noisy samples but also reassign more high-quality predicate labels to them. After the NICE training, a cleaner version of the SGG dataset could be obtained for model training. 



% acmm2020
%\item PCPL \cite{yan2020pcpl}: In this paper, we first discover that when predicate labels have strong correlation with each other, prevalent re-balancing strategies(e.g., re-sampling and re-weighting) will give rise to either over-fitting the tail data(e.g., bench sitting on sidewalk rather than on), or still suffering the adverse effect from the original uneven distribution(e.g., aggregating varied parked on/standing on/sitting on into on). We argue the principal reason is that re-balancing strategies are sensitive to the frequencies of predicates yet blind to their relatedness, which may play a more important role to promote the learning of predicate features. Therefore, we propose a novel Predicate-Correlation Perception Learning(PCPL for short) scheme to adaptively seek out appropriate loss weights by directly perceiving and utilizing the correlation among predicate classes. Moreover, our PCPL framework is further equipped with a graph encoder module to better extract context features. 

% acmm2021, 
%\item DLFE \cite{chiou2021recovering}: To obtain accurate label frequency estimates, we propose Dynamic Label Frequency Estimation (DLFE) to take advantage of training-time data augmentation and average over multiple training iterations to introduce more valid examples. 

% iccv2021, semantic adjustmetn and balanced learning
%\item To tackle semantic space level imbalance and training sample level imbalance, \citet{guo2021general} propose BA-SGG, a simple yet effective SGG framework based on balance adjustment but not the conventional distribution fitting. It integrates two components: Semantic Adjustment (SA) and Balanced Predicate Learning (BPL), respectively, for adjusting these imbalances. 

%Specifically, NICE consists of three components: negative Noisy Sample Detection (Neg-NSD), positive NSD (Pos-NSD), and Noisy Sample Correction (NSC). Firstly, in Neg-NSD, we formulate this task as an out-of-distribution detection problem and assign pseudo labels to all detected noisy negative samples. Then, in Pos-NSD, we use a clustering-based algorithm to divide all positive samples into multiple sets and treat the samples in the noisiest set as noisy positive samples. Lastly, in NSC, we use a simple but effective weighted KNN to reassign new predicate labels to noisy positive samples. 

% cvpr2022-fine-granined, no-tradeoff
%\item fine-grained \cite{lyu2022fine}: The performance of current Scene Graph Generation models is severely hampered by some hard-to-distinguish predicates, e.g., "woman-on/standing on/walking on-beach" or "woman-near/looking at/in front of-child". While general SGG models are prone to predict head predicates and existing re-balancing strategies prefer tail categories, none of them can appropriately handle these hard-to-distinguish predicates. 

%To tackle this issue, inspired by fine-grained image classification, which focuses on differentiating among hard-to-distinguish object classes, we propose a method named Fine-Grained Predicates Learning (FGPL) which aims at differentiating among hard-to-distinguish predicates for Scene Graph Generation task. Specifically, we first introduce a Predicate Lattice that helps SGG models to figure out fine-grained predicate pairs. Then, utilizing the Predicate Lattice, we propose a Category Discriminating Loss and an Entity Discriminating Loss, which both contribute to distinguishing fine-grained predicates while maintaining learned discriminatory power over recognizable ones. The proposed model-agnostic strategy significantly boosts the performances of three benchmark models (Transformer, VCTree, and Motif) by 22.8\%, 24.1\% and 21.7\% of Mean Recall (mR@100) on the Predicate Classification sub-task, respectively. Our model also outperforms state-of-the-art methods by a large margin (i.e., 6.1\%, 4.6\%, and 3.2\% of Mean Recall (mR@100)) on the Visual Genome dataset.

% cvpr2022- stacked, no-trade-off
%\item stacked \cite{dong2022stacked}: Scene Graph Generation, which generally follows a regular encoder-decoder pipeline, aims to first encode the visual contents within the given image and then parse them into a compact summary graph. Existing SGG generally approaches not only neglect the insufficient modality fusion between vision and language but also fail to provide informative predicates due to the biased relationship predictions, leading SGG far from practical. Towards this end, in this paper, we first present a novel Stacked Hybrid-Attention network, which facilitates the intra-modal refinement as well as the inter-modal interaction to serve as the encoder. We then devise an innovative Group Collaborative Learning strategy to optimize the decoder. Particularly, based upon the observation that the recognition capability of one classifier is limited towards an extremely unbalanced dataset, we first deploy a group of classifiers that are experts in distinguishing different subsets of classes and then cooperatively optimize them from two aspects to promote the unbiased SGG. Experiments conducted on VG and GQA datasets demonstrate that we not only establish a new state-of-the-art unbiased metric but also nearly double the performance compared with the two baselines. 



% cvpr2022-not all relations, no-trade-off
%\item, not all relations \cite{goel2022not} Scene graph generation (SGG) aims to capture a wide variety of interactions between pairs of objects, which is essential for full scene understanding. Existing SGG methods trained on the entire set of relations fail to acquire complex reasoning about visual and textual correlations due to various biases in training data. Learning on trivial relations that indicate generic spatial configuration like 'on' instead of informative relations such as 'parked on' does not enforce this complex reasoning, harming generalization. To address this problem, we propose a novel framework for SGG training that exploits relation labels based on their informativeness. Our model-agnostic training procedure imputes missing informative relations for less informative samples in the training data and trains an SGG model on the imputed labels along with existing annotations. We show that this approach can successfully be used in conjunction with state-of-the-art SGG methods and improves their performance significantly in multiple metrics on the standard Visual Genome benchmark. Furthermore, we obtain considerable improvements for unseen triplets in a more challenging zero-shot setting.

% cvpr2022-dynamic scene graph
%\item dynamic \cite{li2022dynamic} Humans can not only see the collection of objects in visual scenes but also identify the relationship between objects. The visual relationship in the scene can be abstracted into the semantic representation of a triple subject, predicate, and object and thus results in a scene graph, which can convey a lot of information for visual understanding. Due to the motion of objects, the visual relationship between two objects in videos may vary, which makes the task of dynamically generating scene graphs from videos more complicated and challenging than the conventional image-based static scene graph generation. Inspired by the ability of humans to infer the visual relationship, we propose a novel anticipatory pre-training paradigm based on Transformer to explicitly model the temporal correlation of visual relationships in different frames to improve dynamic scene graph generation. In the pre-training stage, the model predicts the visual relationships of the current frame based on the previous frames by extracting intra-frame spatial information with a spatial encoder and inter-frame temporal correlations with a progressive temporal encoder. In the fine-tuning stage, we reuse the spatial encoder and the progressive temporal encoder while the information of the current frame is combined for predicting the visual relationship. Extensive experiments demonstrate that our method achieves state-of-the-art performance on the Action Genome dataset.

% cvpr2022-new
%\item Structure Sparse \cite{teng2022structured}: Scene graph generation (SGG) is to detect object pairs with their relations in an image. Existing SGG approaches often use multi-stage pipelines to decompose this task into object detection, relation graph construction, and dense or dense-to-sparse relation prediction. Instead, from a perspective on SGG as a direct set prediction, this paper presents a simple, sparse, and unified framework termed Structured Sparse R-CNN. The key to our method is a set of learnable triplet queries and a structured triplet detector which could be jointly optimized from the training set in an end-to-end manner. Specifically, the triplet queries encode the general prior for object pairs with their relations and provide an initial guess of scene graphs for subsequent refinement. The triplet detector presents a cascaded architecture to refine the detected scene graphs with customized dynamic heads progressively. In addition, to relieve the training difficulty of our method, we propose a relaxed and enhanced training strategy based on knowledge distillation from a Siamese Sparse R-CNN. We perform experiments on several datasets: Visual Genome and Open Images V4/V6, and the results demonstrate that our method achieves state-of-the-art performance. In addition, we also perform in-depth ablation studies to provide insights into our structured modeling in triplet detector design and training strategies.

% eccv2022-data trans
%\item IETrans \cite{zhang2022fine}: Scene graph generation (SGG) is designed to extract (subject, predicate, object) triplets in images. Recent works have made steady progress on SGG and provide useful tools for high-level vision and language understanding. However, due to the data distribution problems, including long-tail distribution and semantic ambiguity, the predictions of current SGG models tend to collapse to several frequent but uninformative predicates (e.g., on, at), which limits the practical application of these models' downstream tasks. To deal with the problems above, we propose a novel Internal and External Data Transfer (IETrans) method, which can be applied plug-and-play and expanded to large SGG with 1,807 predicate classes. Our IETrans tries to relieve the data distribution problem by automatically creating an enhanced dataset that provides more sufficient and coherent annotations for all predicates. By training on the enhanced dataset, a Neural Motif model doubles the macro performance while maintaining competitive micro performance. 

% cvpr2022-new
%\item RU-Net \cite{lin2022ru}: Scene graph generation (SGG) aims to detect objects and predict the relationships between each pair of objects. Existing SGG methods usually suffer from several issues, including 1) ambiguous object representations, as graph neural network-based message passing (GMP) modules, are typically sensitive to spurious inter-node correlations, and 2) low diversity in relationship predictions due to severe class imbalance and a large number of missing annotations. To address both problems, in this paper, we propose a regularized unrolling network (RU-Net). We first study the relation between GMP and graph Laplacian denoising (GLD) from the perspective of the unrolling technique, determining that GMP can be formulated as a solver for GLD. Based on this observation, we propose an unrolled message-passing module and introduce an l$\_$p-based graph regularization to suppress spurious connections between nodes. Second, we propose a group diversity enhancement module that promotes the prediction diversity of relationships via rank maximization. Systematic experiments demonstrate that RU-Net is effective under various settings and metrics. Furthermore, RU-Net achieves new state-of-the-art on three popular databases: VG, VRD, and OI.


% eccv2022-segmentation
%\item Panoptic\cite{yang2022panoptic}: Existing research addresses scene graph generation (SGG) -- a critical technology for scene understanding in images -- from a detection perspective, i.e., objects are detected using bounding boxes followed by prediction of their pairwise relationships. We argue that such a paradigm causes several problems that impede the progress of the field. For instance, bounding box-based labels in current datasets usually contain redundant classes like hairs, and leave out background information that is crucial to the understanding of context. In this work, we introduce panoptic scene graph generation (PSG), a new problem task that requires the model to generate a more comprehensive scene graph representation based on panoptic segmentations rather than rigid bounding boxes. A high-quality PSG dataset, which contains 49k well-annotated overlapping images from COCO and Visual Genome, is created for the community to keep track of its progress. For benchmarking, we build four two-stage baselines, which are modified from classic methods in SGG, and two one-stage baselines called PSGTR and PSGFormer, which are based on the efficient Transformer-based detector, i.e., DETR. While PSGTR uses a set of queries to directly learn triplets, PSGFormer separately models the objects and relations in the form of queries from two Transformer decoders, followed by a prompting-like relation-object matching mechanism. In the end, we share insights on open challenges and future directions.


% eccv2022-memory
%\item Memory \cite{deng2022hierarchical}: As far as Scene Graph Generation (SGG), coarse and fine predicates mix in the dataset due to the crowd-sourced labeling, and the long-tail problem is also pronounced. Given this tricky situation, many existing SGG methods treat the predicates equally and learn the model under the supervision of mixed-granularity predicates in one stage, leading to relatively coarse predictions. In order to alleviate the negative impact of the suboptimum mixed-granularity annotation and long-tail effect problems, this paper proposes a novel Hierarchical Memory Learning (HML) framework to learn the model from simple to complex, which is similar to the human beings' hierarchical memory learning process. After the autonomous partition of coarse and fine predicates, the model is first trained on the coarse predicates and then learns the fine predicates. In order to realize this hierarchical learning pattern, this paper, for the first time, formulates the HML framework using the new Concept Reconstruction (CR) and Model Reconstruction (MR) constraints. It is worth noticing that the HML framework can be taken as one general optimization strategy to improve various SGG models, and significant improvement can be achieved on the SGG benchmark (i.e., Visual Genome).


% eccv2022-open-vocabulary
%\item  vocabulary~\cite{he2022towards}: Scene graph generation (SGG) is a fundamental task aimed at detecting visual relations between objects in an image. The prevailing SGG methods require all object classes to be given in the training set. Such a closed setting limits the practical application of SGG. In this paper, we introduce open-vocabulary scene graph generation, a novel, realistic and challenging setting in which a model is trained on a set of base object classes but is required to infer relations for unseen target object classes. To this end, we propose a two-step method that firstly pre-trains on large amounts of coarse-grained region-caption data and then leverages two prompt-based techniques to finetune the pre-trained model without updating its parameters. Moreover, our method can support inference over completely unseen object classes, which existing methods are incapable of handling. On extensive experiments on three benchmark datasets, Visual Genome, GQA, and Open-Image, our method significantly outperforms recent, strong SGG methods on the setting of Ov-SGG, as well as on the conventional closed SGG.

%\end{itemize}

==> materials/3_unbiased_sgg.tex <==
\section{Unbiased Scene Graph Generation} \label{sec3:sgg}
In this section, we discuss the general scene graph generation model of the object and predicate predictions and depict the predicate sample estimates for measuring its skewness of biased predictions.

\subsection{Scene Graph Generations.} \label{sec3:task}
Given an image $I$, a scene graph model generates a graph $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, where $\mathcal{V}$ and $\mathcal{E}$ are the sets of nodes and edges, respectively. Each node $\bs{o}_i \in \mathcal{V}$ is represented by a bounding box $\bs{v}^{bbox} \in \mathbb{R}^4$ and a corresponding class label $o_y \in \mathcal{C}_{obj}$. Each edge $\bs{r}_{i,j} \in \mathcal{E}$ represents the predicate between the subject node $\bs{v}_i$ and the object node $\bs{v}_j$. The corresponding predicate label is $r_y \in \mathcal{C}_{rel}$.

We depict the proposed unbiased SGG framework as shown in Fig. \ref{fig:model}. Object detector outputs its predictions (a): \textcolor{orange}{\textit{man}} and \textcolor{orange}{\textit{hourse}}. Given \textcolor{orange}{\textit{man - horse}} label prediction pair, the traditional SGG model predicts (d) predicate predictions ($\hat{\bm{R}}$ see Eq. \ref{eq:rel_dist}) through a fusion of (b) non-visual FREQ prior predicates and (c) visual predicate predictions ($\hat{\bm{R}}_{vis}$). For unbiased SGG model training, our SCR estimates (e) a sample size of the possible predicate candidates through FREQ ($\bm{R}_{freq}$ or $\bm{R}_{emb}$ ) and measures (f) the target label skew score and then calculates (g) the training target sample weight for the adaptive re-weighted loss. In (f) and (g), \textcolor{red}{red lines} around the target label indicate \textcolor{red}{predicate skew} ($S^i_{skew}$ see Eq. \ref{eq:skew}) and \textcolor{red}{re-weight scores} ($\bm{W}^i$ see Eq. \ref{eq:effec}), respectively, where they have an approximately inverse relationship.

\input{figures/3_main_model}

\subsubsection{Object Predictions.} \label{sec3_2_2:SOE}
Following \cite{tang2020unbiased}, the node features are derived from the object detector. In particular, for each bounding box $v_i^{bbox}$, the detector returns an RoI-Align feature $\bs{x}_i^{RoI}$ and an object label embedding $\bs{l}_i$. In general SGG model, the $\mathcal{N}$ number of node features are constructed by vector concatenation $\bs{X} = \{[\bs{x}^{RoI}_i; \bs{l}_i; \bs{b}_i]\}_{i=1}^{\mathcal{N}}$, where $\bs{b}_i$ is the embedded box feature from the box coordinate $\bs{v}_i^{bbox}$. 
\begin{equation}
	\tilde{\bs{X}} = fc_{obj}(\bs{X}) \in \mathbb{R}^{\mathcal{N} \times \mathcal{D}_{obj}},
\end{equation}
where all $fc_{*}$ denote a fully connected layer for linear transformations or logits, and the object feature dimension $\mathcal{D}_{obj}$ depends on the SGG model. As depicted in Fig. \ref{fig:model}(a), the predicted object label of $\hat{\bs{O}} \in \mathbb{R}^{\mathcal{N}\times|\mathcal{C}_{obj}|}$ is estimated by object logits $fc(\tilde{\bs{X}})$ as follows:
\begin{equation}
	\hat{\bs{O}} = fc(\tilde{\bs{X}}).
	\label{eq:p_obj}
\end{equation}

\subsubsection{Predicate Predictions.}
Inspired by \citet{tang2020unbiased}, \citet{zhu2023brain}, predicate predictions can be made by employing multiple logits from visual and non-visual features. We follow the sum over all outputs to generate the final predicate prediction.  As illustrated in Fig. \ref{fig:model}(d), the combined predicate logit $\hat{\bs{R}}$ is estimated based on the summation of the visual logits and the non-visual logits as follows:
\begin{equation}
	\hat{\bs{R}} = \hat{\bs{R}}_{vis} \oplus \hat{\bs{R}}_{freq} \oplus \hat{\bs{R}}_{emb},
	\label{eq:rel_dist}
\end{equation}
\noindent
where $\hat{\bs{R}} \in \mathbb{R}^{\mathcal{N}(\mathcal{N}-1)\times |\mathcal{C}_{rel}|}$; $\oplus$ is an element-wise sum; as shown in Fig. \ref{fig:model}(c), $\hat{\bs{R}}_{vis}$ is the predicate logits from visual feature $\bs{F}_{vis}$ such as a $\mathcal{D}_{vis}$ dimensional union feature and a \textit{subject-object} pair feature, which also depends on the SGG model, \\

\begin{equation}
	\begin{aligned}
		&\hat{\bs{R}}_{vis} = fc_{vis}(\bs{F}_{vis}),~~ \bs{F}_{vis}  \in \mathbb{R}^{\mathcal{N}(\mathcal{N}-1) \times \mathcal{D}_{vis} }, \\
		%&\hat{\bs{R}}_u = fc_{u}(\tilde{\bs{G}}_{u}), \tilde{\bs{G}}_{u} \in \mathbb{R}^{N(N-1) \times 4096}, \\
		&\hat{\bs{R}}_{freq} = \text{Sigmoid}( \bs{R}_{freq})\in \mathbb{R}^{\mathcal{N}(\mathcal{N}-1) \times |\mathcal{C}_{rel}|}, \\
		&\hat{\bs{R}}_{emb} = fc_{emb}(\bs{L}_{emb} ), ~~\bs{L}_{emb}  \in \mathbb{R}^{\mathcal{N}(\mathcal{N}-1) \times 400}.  \\
		%&\hat{\bs{R}}_{geo} = fc_{geo}(\bs{B}_{u} ), \bs{B}_{u} \in \mathbb{R}^{N(N-1) \times 128}.
	\end{aligned}
\end{equation}

\noindent
The FREQ~\cite{zellers2018neural} as a non-visual feature, $\bs{R}_{freq}$ (Fig. \ref{fig:model}(b)) looks up the empirical distribution over relationships between subject $\hat{o}_i$ and object $\hat{o}_j$ as computed in the training set where $\hat{o}_i, \hat{o}_j \in \hat{\bs{O}}$. However, since FREQ does not consider any image representations when predicting predicates, it tends to lead to biased predicate predictions due to its imbalanced predicate distribution. To minimize the biased effects, we use the Sigmoid-activated FREQ predicate logits. In addition, for acquiring the more smoothness of the empirical distribution, the concatenated \textit{subject-object} embedding $\hat{\bs{R}}_{emb}$ is added to the predicate predictions where  $\bs{L}_{emb} = \{[\bs{l}_i; \bs{l}_j] \}_{i,j}^{\mathcal{N}}$. \\

\noindent
\subsection{Sample Estimates} 
Non-visual predicate features tend to be more biased than visual features due to an imbalanced training set. If the degree of biased predictions can be measured, we can leverage its value to learn the SGG models without bias. According to \citet{brown2011measures}, the degree of bias prediction can generally be measured in a skew score. In general, if there is no bias, the skew score is close to $0$, and if it is biased to one side, the skew score is over either $-1$ or $+1$. 

In SCR, we need to estimate how many predicate samples are biased to measure the predicate skew scores. To approximate the biased sample numbers, we use two non-visual prior predicate distributions of FREQ, $\hat{\bs{R}}_{freq}$ and \textit{subject-object} label embedding $\hat{\bs{R}}_{emb}$ as described in Fig. \ref{fig:model}(e). Based on the two predicate distributions, at first, we define the skew logit $\hat{\bs{R}}_{skew}$ with the Sigmoid activation function as follows:
\begin{equation}
	\hat{\bs{R}}_{skew} = \text{Sigmoid}(\bs{R}_{freq} \oplus \hat{\bs{R}}_{emb}).
	\label{eq:skewness}
\end{equation} 
To estimate the predicate sample weights properly, the SCR approximates skewness through the predicate sample estimates $\hat{\bs{R}}_{skew}$ in Eq. \ref{eq:skewness}. We investigate the best predicate sample estimates through several experiments with a combination of non-visual predictions as follows:
\begin{itemize}
	\item SCR of EMB: $\hat{\bs{R}}_{skew}= \text{Sigmoid}(\hat{\bs{R}}_{emb})$,
	\item SCR of FREQ: $ \hat{\bs{R}}_{skew}=\text{Sigmoid}(\bs{R}_{freq})$,
	\item SCR of FREQ+EMB: $\hat{\bs{R}}_{skew}=\text{Sigmoid}(\bs{R}_{freq} \oplus \hat{\bs{R}}_{emb})$.
\end{itemize}


\noindent
Then, the predicate sample estimates are acquired as follows:  
\begin{equation}
	\mathcal{M} = \sum_i^{\mathcal{N} (\mathcal{N}-1)} \hat{\bs{r}}_i,
	\label{eq:predicate_effective}
\end{equation} 
where $\hat{\bs{r}}_i \in \hat{\bs{R}}_{skew}$; the estimated $m_y \in \mathcal{M}$ is the number of $y$th predicate sample size and $m_y \in [0, \mathcal{N}(\mathcal{N}-1))$.

Moreover, the skew predicate $\hat{\bs{R}}_{skew}$ serves to estimate the predicate candidates that a \textit{subject-object} pair can have fairly since the Sigmoid activation function suppresses the more extensive biased predictions. For example, a \textit{Man-Horse} pair may have predicates such as \textit{riding, on, with}, etc. The Sigmoid activation function amplifies the frequency of the minority predicates while squeezing that of the majority ones, as shown in Fig.~\ref{fig:model} (b) and (e), which is used to calculate Skew Class-Balanced Effective Number that we depict in the following section. \\

\noindent 
Note in Eq. \ref{eq:skewness}, the Sigmoid activation function was applied to estimate the predicate sample sizes (Eq. \ref{eq:predicate_effective}) and measure skewness (Eq. \ref{eq:skew}), given a subject-object pair. The main reason was that it provides smoothly activated outputs from 0 to 1. We assumed that an output value of 1 is regarded as one predicate.


\section{Skew Class-balanced Re-weighting (SCR)} \label{sec4:scr}
In this section, leveraged by the biased predictions deduced by the predicate sample estimates, the \textit{Skew Class-balanced Re-weighting} (SCR) performs sample weight estimates for learning unbiased SGG models.

\subsection{Skew Class-balanced Effective Number} \label{sec4:effective_number}
The \textit{Skew Class-balanced Effective Number} approximates the mini-batch class-balanced re-weighting coefficients $\bs{E}_{m_y}$ based on the predicate skew logit $\hat{\bs{R}}_{skew}$ in Eq.~\ref{eq:skewness}. The $i$th predicate sample $E^{i}_{m_y}$ is defined as follows as \cite{cui2019class, mm2021kang}: 
\begin{equation}
	E^{i}_{m_y} = \frac{1-\beta^{m_y}_i}{(1-\beta_i)}, 
	\label{eq:effec}
\end{equation}
where $\beta_i = (m_y - 1) / m_y$; the effective number satisfies the following properties that $E^{i}_{m_y} = 1$ if $\beta_i=0 \; (m_y=1)$; $E^i_{m_y} \rightarrow m_y$ as $\beta_i \rightarrow 1 \; (m_y \rightarrow \infty)$ such that $\beta_i$ controls how fast $E^i_{m_y}$ grows as the target predicate sample size $m_y$ increases. 

To estimate the $i$th predicate effective number $E^{i}_{m_y}$, we adaptively estimate the $\beta_i \in [0, 1)$ by using the entropy $H^i_{skew}$ and skew score function $S^i_{skew}$ of the $\hat{\bs{R}}_{skew}$ as shown in Alg.~\ref{al:effective}: if $S^i_{skew} > S_{th}$ then the $\beta_i \in [0, 1)$ that assigns more weights to the minority predicate samples than the majority ones; otherwise, $S^i_{skew} \leq S_{th}$ then $\beta_i=0$ that re-weights uniformly over the entire class sample loss, i.e., conventional cross-entropy loss. The threshold $S_{th}$ is determined as follows: 
\begin{equation}
	S_{th} = \bar{S}_{skew}-\delta, 
	\label{eq:skew_th}
\end{equation}
where $\bar{S}_{skew}$ and $\delta=0.7$ are the mean value of $\bs{S}_{skew}$ and the hyper-parameter used respectively in all experiments.  

\input{figures/3_main_skew_balance}

\subsection{Skew Measures}
In training, the predicate sample skewness depends on the predicate label. In other words, according to~\citet{brown2011measures}, some majority predicate skew values tend to be greater than zero while others tend to be zero or negative. This is an unfair skew measure, leading the SCR Alg.~\ref{al:effective} to more weights either in the majority predicates or in the minority ones. In this paper, as portrayed in Fig. \ref{fig:model}(f), to measure the skew value of all target labels fairly, we use the target skew logit instead of the mean value. Therefore, the $i$th predicate sample skew $S^{i}_{skew}$ is firstly measured by the following equation given the target label index $y$ as follows:
\begin{equation}
	S^{i}_{skew} = \frac{\frac{1}{|\mathcal{C}_{rel}|} \sum_{\hat{r}_{i,j} \in \hat{\bs{R}}^i_{skew}} (\hat{r}_{i,j} - \hat{r}_{i,y})^3}{\left(\frac{1}{|\mathcal{C}_{rel}|} \sum_{\hat{r}_{i,j} \in \hat{\bs{R}}^i_{skew}}(\hat{r}_{i,j} - \hat{r}_{i,y})^2 \right)^{3/2}}.
	\label{eq:skew}
\end{equation} 

\noindent
Then, we use the uniformness to determine the $\beta$. The uniformness provides confidence in the predicate sample estimates. To calculate the uniformness of the $i$th predicate sample, we estimate the entropy $H^{i}_{skew}$ as follows:
\begin{equation}
	H^{i}_{skew} = -\lambda_{skew} \sum_{\hat{r}_{i,j} \in \hat{\bs{R}}^i_{skew}} p(\hat{r}_{i,j}) \log_{|\mathcal{C}_{rel}|} p(\hat{r}_{i,j}),
	\label{eq:entropy}
\end{equation}
where the number of predicates $|\mathcal{C}_{rel}|$ is used as the base of the logarithm, which $H^{i}_{skew} \in [0, 1]$; the $\hat{\bs{r}}_i \in \hat{\bs{R}}_{skew}$ have uniform distributions when $H^{i}_{skew}$ is close to $1$; otherwise, the predicate sample may have either skew distributions or correct distributions and the $\lambda_{skew}=0.06$ is the coefficient of $S_{skew}$. The following section depicts the relationship between skew and entropy in detail. 

\input{algoritems/3_main_algorithm}


%\caption{The Biased Predicate Weights: (a) an assumption that the predicate biased logits are represented by its frequency $\mathcal{M}^{1/5}$ and that the degree of biased predictions is also modeled by its entropy $H_{skew}$, (b) the discrete sample weights are assigned to the minority predicates according to the entropy $H_{skew}$ and (c) the skew in Eq. \ref{eq:skew} measures not only the degree of true/false prediction but also biased predictions; the true prediction has the negative skew $S_{skew} < 0$ while others do not.}

\subsection{Target Sample Weights}
The interpretation of the relationship between skew and weight is depicted based on biased predicate prediction as shown in Fig.~\ref{fig:skew_weight_entropy}. In Fig.~\ref{fig:skew_softmax}, to understand the sample weight estimate from the predicate sample estimates, we assume that the predicate biased predictions $\hat{\bs{R}}_{skew}$ are given by the predicate sample frequency $\mathcal{M}^{1/5}$ (see Fig.~\ref{fig:imbalance}) and the predicate entropy $\bs{H}_{skew}$, i.e., the more frequent sample is the more biased prediction is; the more biased the prediction is the less entropy is. The skew $\bs{S}_{skew}$ measures not only the degree of true/false prediction but also biased predictions as shown in Fig.~\ref{fig:skew_entropy}. The following simple equation summarizes the degree of true/false predictions:
\begin{equation}
	\begin{cases}
		S^{i}_{skew} > 0 & \text{if} \arg\max_{j} \hat{\bs{r}}_{i,j} \neq r_y\\
		S^{i}_{skew} < 0 & \text{otherwise.}
	\end{cases}
\end{equation}
where $S^{i}_{skew} \approx -1$ for the true prediction; $S^{i}_{skew} = 0$ for the uniform prediction and $S^{i}_{skew} \gg 0$ for the false and biased prediction. Moreover, the predicate target label-wise skew has more discrete at high entropy. The final $i$th sample weight $w^i_y=1/E^{i}_{m_y}$ (Fig. \ref{fig:model}(g)) is acquired by the criteria of skew and entropy as shown in Fig.~\ref{fig:skew_weight}. The minority predicates have larger weights than the majority when $S^{i}_{skew} \gg 0$.

%where $w_y^{obj} \in \frac{1}{E_{n_y}^{obj}} = \frac{1-\beta^{obj}}{1-\beta^{n_y^{obj}}}$ and $|\mathcal{C}_{obj}| = \sum_i^{|\mathcal{C}_{obj}|} w^{obj}_j$.
\subsection{Learning with SCR} 
Except for object loss, all traditional SGG models are learned by the skew class-balanced re-weighting cross-entropy loss functions. The conventional cross-entropy loss for the objects is computed, given object predictions $\hat{\bs{O}}$ and the object ground-truth $o^i_y \in \bs{O}$ as follows:  
\begin{equation}
	\mathcal{L}_{obj}(\hat{\bs{O}}, \bs{O}) = \sum_i^\mathcal{N} -\gamma_{obj} \cdot w_{y}^{i} \log \left( \frac{\exp(\hat{o}_y)}{\sum_{\hat{o}_j \in \hat{\bs{O}}_i} \exp(\hat{o}_j)} \right),
	\label{eq:loss_obj}
\end{equation}
where, given $\mathcal{N}$ of objects, $i$th object sample weight is $w_y^{i}=1$ s.t. $|\mathcal{C}_{obj}| = \sum_j^{|\mathcal{C}_{obj}|} w^i_j$; here, the sample weight denominator $\gamma_{obj}=1/\sum_i^\mathcal{N} w^i_y$ is used for the mean object cross-entropy loss. The skew class-balanced cross-entropy loss computes the skew predicate-balanced cross-entropy, based on the predicate predictions $\hat{\bs{R}}$ and the predicate ground-truth $r^i_y \in \bs{R}$:
\begin{equation}
	\mathcal{L}_{rel}(\hat{\bs{R}}, \bs{R}) = \sum_{i}^{\mathcal{N}(\mathcal{N}-1)} - \gamma_{rel} \cdot w_{y}^{i} \log \left( \frac{\exp(\hat{r}_y)}{\sum_{\hat{r}_j \in \hat{\bs{R}}_i} \exp(\hat{r}_j)} \right),
	\label{eq:loss_rel}
\end{equation}
where, given $\mathcal{N}(\mathcal{N}-1)$ of object-subject pairs, the $i$th predicate sample weight is $w_y^{i} = \frac{1}{E^i_{m_y}} = \frac{1-\beta_i}{1-\beta^{m_y}_i}$ s.t. $|\mathcal{C}_{rel}| = \sum_j^{|\mathcal{C}_{rel}|} w^{i}_j$; here, we set the predicate sample normalizer as $\gamma_{rel}=1/\sum_i^{\mathcal{N}(\mathcal{N}-1)} w^i_y$ for mean predicate loss. In summary, the total objective loss function $\mathcal{L}_{total}$ for unbiased SGG learning can be formulated as follows:
\begin{equation}
	\mathcal{L}_{total} = \mathcal{L}_{obj} + \mathcal{L}_{rel}.
	\label{eq:loss_total}
\end{equation}

==> materials/4_experiments.tex <==
\section{Experiments}\label{sec5:exp}
The proposed SCR is evaluated with the traditional SGG models on the Visual Genome benchmark datasets~\cite{krishna2017visual}, and the performances of the SCR are compared with others in the multiple SGG tasks.

\input{figures/4_main_qaul_weight}

\subsection{Visual Genome}
We used Visual Genome (VG)~\cite{krishna2017visual} dataset to train and evaluate our models, which is composed of $108$k images across $75$k object categories and $37$k predicate categories. We followed the widely adopted VG split~\cite{xu2017scene,zellers2018neural,chen2019counterfactual} containing the most frequent $150$ object categories and $50$ predicate categories. The original split only has a training set ($70\%$) and a test set ($30\%$). We followed ~\citet{zellers2018neural} to sample a $5$k validation set from the training set for parameter tuning.

\subsection{Open Images}
The Open Images dataset~\cite{kuznetsova2020open} is a large-scale dataset proposed by Google recently. Compared with the Visual Genome dataset, it has a superior annotation quality for the scene graph generation. In this work, we conduct experiments on Open Images $V4\& V6$, following similar data processing and evaluation protocols in \cite{kuznetsova2020open, zhang2019graphical, lin2020gps}. The Open Images V4 is introduced as a benchmark for scene graph generation by~\citet{zhang2019graphical} and \citet{lin2020gps}, which has $53,953$ and $3,234$ images for the train and validation sets, $57$ objects categories, and $9$ predicate categories in total. The Open Images V6 has $126,368$ images used for training, $1813$, and $5322$ images for validation and testing, respectively, with $301$ object categories and $31$ predicate categories. This dataset has a comparable amount of semantics categories with the VG.

\subsection{Experiments Configurations}
\noindent
\textbf{State-of-the-Art Comparisons.} For fair comparisons, all the compared SGG models should use the FREQ~\cite{zellers2018neural}, which looks up the empirical distribution over relationships between subject prediction $\hat{o}_i$ and object ones $\hat{o}_j$. To evaluate the effectiveness of the SCR learning algorithm, we follow the same experimental settings as the CogTree~\cite{yu2020cogtree}. We also set the current state-of-the-art SGG models as the baseline: MOTIFS \cite{zellers2018neural}, VCTree~\cite{tang2019learning} and SG-Transformer~\cite{yu2020cogtree} which contains 3 $O2O$ blocks and 2 $R2O$ blocks with $12$ attention heads, and Bipartite-Graph~\cite{li2021bipartite} without resampling layers and compare the performance with the state-of-the-art debiasing approach TDE~\cite{tang2020unbiased}, CogTree~\cite{yu2020cogtree}, PCPL~\cite{yan2020pcpl}, DLFE~\cite{chiou2021recovering}, BPL-SA~\cite{guo2021general}, PPDL~\cite{li2022ppdl}, and NICE~\cite{li2022devil}. \\

\input{tables/4_main_sgg_performances}

\noindent
\textbf{Implementation.} Following the previous works~\cite{tang2020unbiased, yu2020cogtree, li2021bipartite}, the object detector is the pre-trained Faster R-CNN~\cite{ren2015faster} with ResNeXt-101-FPN~\cite{lin2017feature}. In bi-level resampling~\cite{li2021bipartite}, we also set the repeat factor $t=0.07$, instances drop rate $\gamma_d=0.7$, and weight of fusion the entities features $\rho=-5$. The $\alpha, \beta$ are initialized as 2.2 and 0.025, respectively. 

\subsection{Evaluations}
Our SCR has the following two evaluations: 

\noindent
\textbf{Relationship Retrieval (RR)} contains three sub-task: (1) Predicate Classification (PredCls): taking ground truth bounding boxes and labels as inputs, (2) Scene Graph Classification (SGCls): using ground truth bounding boxes without labels, (3) Scene Graph Detection (SGDet): detecting SGs from scratch. The conventional metric of RR is \textbf{Recall@K (R@K)}, included in this paper even though the biased prediction is reported by~\citet{misra2016seeing} for the performance of the SCR. Moreover, to evaluate the general performances, we adopted \textbf{mean Recall@ K (mR@K)} that retrieves each predicate separately and then averages R@K for all predicates.\\

\noindent
\textbf{Zero-Shot Relationship Retrieval (ZSRR)}. The \textbf{Zero-Shot Recall@K} was firstly evaluated on the VG dataset in~\cite{tang2020unbiased}, which reports the R@K of those subject-predicate-object triplets that have never been observed in the training set. ZSRR also has three sub-tasks as RR.

\input{tables/4_main_sgg_openimage}

\subsection{Quantitative Results}
\noindent
\textbf{Visual Genome.} The SCR is compared with others on the two evaluation tasks: RR and ZSRR, which are the same as shown in Table.~\ref{table:m_recall} and \ref{table:zero_shot}. The SCR achieves the best and second best performances over the previous methods: TDE, PCPL, Cogtree, DLFE, BPL-SA PPDL, and NICE, demonstrating its generality and effectiveness on the two measures of RR task. Moreover, the SCR shows the best trade-off performances on the ZSRR task as shown in Fig. \ref{table:zero_shot}. \\

\noindent
\textbf{The Best Trade-off performances.} To analyze the trade-off between majority and minority predicate performances, firstly, we need to understand the two measurements, mRR and RR. The mRR was introduced to calculate the recall on each predicate category independently and then to average the results by \citet{tang2019learning}. This is because of RR’s bias, which was reported by \citet{misra2016seeing}. The higher the recall scores (RR) are, the more biased the majority categories are. Therefore, a higher mRR is a more unbiased SGG model; a higher RR is a more biased SGG model. Traditional SGG models show the tendency that if mRR is higher than RR, RR performances are low, i.e., MOTIFS, VCTREE, and SG-Transformer show the best Recall but low mRR@100 in Table.~\ref{table:m_recall}. However, our SCR shows the best trade-off in terms of mRR and RR measurements; MOTIFS with SCR shows the best performances in mRR and the second-best performances in RR except for MOTIFS. So do the other models' results. Figure \ref{fig:qual_weight} supports our analysis of the best trade-off since overall predicate performances were better than the traditional SGG model (SG-Transformer). \\

\input{tables/4_main_sgg_zeroshot}

\noindent
\textbf{Open Image V4 \& V6.} 
To show the effectiveness of SCR, we set BGNN as the baseline, as shown in Table.~\ref{table:openimage}. On Open Images Dataset V4, SCR outperformed BGNN except for $score_{wtd}$ measurement. Mainly, SCR shows outstanding performance in terms of phrase evaluation. Moreover, on Open Images Dataset V6, SCR outperformed all baselines such as BGNN, GPS-Net, Etc., showing a good trade-off between mean recall@50 and recall@50. These results proved that we could have a good trade-off performance in long-tailed predicated distributions if properly assigning weights in training.

\subsection{Ablation Study}
We investigate the predicate-biased prediction and the best hyper-parameter settings of the SCR loss function for the better generalized SGG models. \\

\input{figures/5_main_pred_weight}

\noindent
\textbf{Predicate Bias.} To estimate the predicate bias and assign the proper sample weights, we define the predicate sample estimates $\hat{\bs{R}}_{skew}$ of $\hat{\bs{R}}_{freq}$ and $\hat{\bs{R}}_{emb}$ in Eq.~\ref{eq:skewness}. To investigate the proper predicate sample estimates, we examined the effectiveness of the predicate sample estimates-SCR of EMB, SCR of FREQ, and SCR of FREQ+EMB with the fixed predicate predictions (Eq.~\ref{eq:rel_dist}) as shown in Table.~\ref{table:skew_ablation}. In the experiments, the SCR of FREQ+EMB leads to more generalized performances over others. In summary, the previous Re-Weight methods worsen the recall performances, while the SCR does not. \\

\input{tables/4_main_sgg_ablation}

\noindent
\textbf{Hyper-parameters.} The hyper-parameters of SCR control the weight of the SGG loss. We investigate the best hyper-parameter settings as shown in Table. \ref{table:hyper_ablation}. The best hyper-parameter settings $\delta=0.7$ and $\lambda_{skew}=0.06$ show the generalized performances of the SGG tasks. The smaller $\lambda_{skew}$ is, the higher mean Recall scores are, while the higher $\lambda_{skew}$ is, the higher Recall scores are, i.e., the $\lambda_{skew}$ controls the trade-off between the majority predicates and the minority ones since the smaller $H_{skew}$ tend to assign more weights to the minority predicates in the SCR. The $\delta=0.7$ shows the best proportion of Re-weighting the predicate samples.  

\input{tables/4_main_sgg_hyper_ablation}
%\input{tables/4_main_head_tail}

\subsection{Qualitative Examples}
To demonstrate the effectiveness of the sample-wise SCR Re-weighting, we show the comparison of Recall @100 on PredCls of all predicates based on the SG-Transformer~\cite{yu2020cogtree} as shown in Fig.~\ref{fig:qual_weight}. The SCR of FREQ+EMB achieves a significant performance gain on the overall predicate categories. Moreover, the skew predicate $\hat{\bs{R}}_{skew}$ serves to estimate not only the predicate candidates that a \textit{subject-object} pair can have but also the target skew $S_{skew}$ which determines the sample weight. Figure~\ref{fig:qual_skew_preds} includes a \textit{subject-object} pair which have possible predicates, its predicate prediction $\hat{\bs{R}}_i$, and the target skew $S^i_{skew}$ deduced by the predicate sample estimate $\hat{\bs{R}}^i_{skew}$. The higher the sample estimate is, the lower the target skew is. To be specific, when one \textcolor{orange}{\textit{woman} -} \textcolor{green}{$S^{\text{wearing}}_{skew}$}  \textcolor{orange}{- coat} pair have possible predicates such as \textcolor{cyan}{\textit{backgrounds, has, wearing, in}, etc.}, we show \textcolor{violet}{predicate predictions $\hat{\bs{R}}_i$} with its \textcolor{green}{target skew $S^i_{skew}$} deduced by its \textcolor{red}{sample estimates $\hat{\bs{R}}^i_{skew}$}. The larger $\hat{R}^i_{skew} \in \hat{\bs{R}}^i_{skew}$ tends to be a smaller $S^i_{skew}$, when compared to another \textcolor{orange}{\textit{hill -}} \textcolor{green}{$S^{\text{covered in}}_{skew}$}  \textcolor{orange}{- snow} pair in a SCR-trained SGG model.


==> materials/5_conclusions.tex <==
\section{Conclusions}\label{sec6:conc}
In this paper, the unbiased Scene Graph Generation (SGG) algorithm, referred to as Skew Class-balanced Re-weighting (SCR), was proposed for considering the unbiased predicate prediction caused by the long-tailed distribution. The prior works focus mainly on alleviating the deteriorating performances of the minority predicate predictions, showing drastic dropping recall scores, i.e., forgetting the majority predicate class. It has not yet properly analyzed the trade-off performances between majority and minority predicates in the given SGG datasets. In this paper, to address the issues leveraged by the skewness of biased predicate predictions, firstly, the SCR estimated the predicate re-weighting coefficient and then re-weighted more to the biased predicates for the better trading-off performances between the majority and the minority predicates. Extensive experiments conducted on the standard Visual Genome dataset and Open Image V4 \& V6 showed the SCR's effectiveness and generality with the traditional SGG models.

==> tables/4_main_head_tail.tex <==
\begin{table}[h]
	\scriptsize
	\center
    \caption{The Ablation Study for the SCR + Resample. $\dagger$ denote results reproduced by \cite{li2021bipartite}.}
	\begin{adjustbox}{width=0.58\textwidth}
		\begin{tabular}{c cc ccc}
			%\hlinewd{1.4pt}
			%\hlinewd{1.0pt}
			%\multicolumn{3}{l|}{\textbf{Relationship Retrieval}} & 
			%\multicolumn{2}{l|}{\textbf{PredCls}} & \multicolumn{2}{l|}{\textbf{SGCls}} & \multicolumn{2}{l}{\textbf{SGDet}}  \\ \hline
			%Model  & $\lambda_{skew}$ & $\delta$                                       
			%& mRR & RR                                                     
			%& mRR & RR                                                   
			%& mRR & RR   \\ \hline
			
			%\multirow{4}{*}{ \begin{tabular}[c]{@{}l@{}} VCTree  \\ +SCR$\ssymbol{2}$ \end{tabular} } &
			%&\begin{tabular}[c]{@{}l@{}} 0.03         \\ 0.06 \\ 0.08    \end{tabular}   &
			%\begin{tabular}[c]{@{}l@{}} 0.7          \\ 0.7  \\ 0.7     \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 35.9\\ 33.7 \\ 32.8    \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 57.0         \\ 60.0 \\ 60.4    \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 20.1\\ 18.0 \\ 17.2    \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 31.9         \\ 33.3 \\ 34.2    \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 16.3\\ 14.4 \\ 13.5    \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 29.4         \\ 31.9 \\ 32.6    \end{tabular}   %\\ \cline{2-9}
			\toprule
			          & \multicolumn{5}{c}{\textbf{SGDet}} \\
			          \cline{2-6}
			          & mR@100 & R@100 & Head  & Body  & Tail \\ \midrule
			None $^\dagger$  & 9.7    & 36.1  & 34.2  & 9.9   & 2.6  \\
			RFS $^\dagger$ \cite{gupta2019lvis}    & 10.7   & 34.6  & 33.2  & 9.7   & 3.5  \\
			BLS $^\dagger$ \cite{li2021bipartite}   & 12.6   & 35.8  & 34.0  & 12.9  & 6.0  \\ \midrule
			\textbf{BLS+SCR}   &        &       &       &       &      \\
			\bottomrule
		
			%\begin{tabular}[c]{@{}l@{}} SCR+FREQ+EMB \end{tabular}            &
			%&
			%\begin{tabular}[c]{@{}l@{}} 0.06 \\ 0.06 \\ 0.06 \end{tabular}   &
			%\begin{tabular}[c]{@{}l@{}} 0.6  \\ 0.7  \\ 0.8  \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 33.5 \\ 33.7 \\ 33.3 \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 60.6 \\ 60.0 \\ 59.3 \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 17.8 \\ 18.0 \\ 17.6 \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 34.3 \\ 33.3 \\ 33.0 \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 14.2 \\ 14.4 \\ 14.0 \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 32.0 \\ 31.9 \\ 30.6 \end{tabular}   \\ \hline %\cline{2-8}  
			%\hlinewd{1.0pt}                                                    
		\end{tabular}
	\end{adjustbox}
	\label{table:head_tail}
\end{table}

==> tables/4_main_sgg_ablation.tex <==
\begin{table}[hptb]
	%\scriptsize
	\centering
    \caption{The Ablation Study for the Predicate Sample Estimates on Recall@100. The underbar represents the predicate sample estimates for better generality.}
	\begin{adjustbox}{width=0.88\textwidth}
		\begin{tabular}{cc ccc ccc ccc}
			%\hlinewd{1.0pt}
			%\hlinewd{1.0pt}
			\hline 
			\multicolumn{2}{l}{\textbf{Relationship Retrieval}} & 
			\multicolumn{3}{l}{\textbf{PredCls}} & \multicolumn{3}{l}{\textbf{SGCls}} & 
			\multicolumn{3}{l}{\textbf{SGDet}}  \\ \hline
			Model  & Method                                      
			& mRR & ZSRR & RR                                                    
			& mRR & ZSRR & RR                                                   
			& mRR & ZSRR & RR  \\ \midrule
			
			%\multirow{1}{*}{Bipartite-Graph  \cite{li2021bipartite}}    & 
			\begin{tabular}[c]{@{}l@{}} VCTree \end{tabular} &
			\begin{tabular}[c]{@{}l@{}}SCR of FREQ \\ SCR of EMB \\ \textbf{SCR of FREQ+EMB} \end{tabular} & 
			\begin{tabular}[c]{@{}l@{}} 31.6 \\ 33.3 \\ \underbar{33.7} \end{tabular}   &
			\begin{tabular}[c]{@{}l@{}} 22.2 \\ 21.1 \\ \underbar{20.1} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 60.0 \\ 60.1 \\ \underbar{60.0} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 16.9 \\ 17.9 \\ \underbar{18.0} \end{tabular}   &
			\begin{tabular}[c]{@{}l@{}}  6.2 \\ 5.9  \\ \underbar{6.1}  \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 35.4 \\ 35.2 \\ \underbar{33.3} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 13.3 \\ 15.4 \\ \underbar{14.4} \end{tabular}   &
			\begin{tabular}[c]{@{}l@{}}  3.5 \\ 3.5  \\ \underbar{3.5}  \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 31.6 \\ 30.0 \\ \underbar{31.9} \end{tabular}   \\ 
			\bottomrule
			%\cline{2-8}  
			%\hlinewd{1.0pt}                                                    
		\end{tabular}
	\end{adjustbox}
	\label{table:skew_ablation}
\end{table}

==> tables/4_main_sgg_hyper_ablation.tex <==
\begin{table}[hptb]
	\scriptsize
	\center
    \caption{The Ablation Study for the SCR Hyper-Parameters on Recall@100. The underbar represents the best trade-off performances between mRecall and Recall. SCR$\ssymbol{2}$ denotes SCR of FREQ+EMB.}
	\begin{adjustbox}{width=0.68\textwidth}
		\begin{tabular}{c cc cc cc cc}
			%\hlinewd{1.4pt}
			%\hlinewd{1.0pt}
			%\hline
			\toprule
			\multicolumn{3}{l}{\textbf{Relationship Retrieval}} & 
			\multicolumn{2}{l}{\textbf{PredCls}} & \multicolumn{2}{l}{\textbf{SGCls}} & \multicolumn{2}{l}{\textbf{SGDet}}  \\ \hline
			Model  & $\lambda_{skew}$ & $\delta$                                       
			& mRR & RR                                                     
			& mRR & RR                                                   
			& mRR & RR   \\ \midrule
			
			\multirow{4}{*}{ \begin{tabular}[c]{@{}l@{}} VCTree  \\ +\textbf{SCR}$\ssymbol{2}$ \end{tabular} } &
			\begin{tabular}[c]{@{}l@{}} 0.03         \\ \underbar{0.06} \\ 0.08    \end{tabular}   &
			\begin{tabular}[c]{@{}l@{}} 0.7          \\ 0.7  \\ 0.7     \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} \textbf{35.5}\\ \underbar{33.7} \\ 32.8    \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 58.3         \\ \underbar{60.0} \\ 60.4    \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} \textbf{20.1}\\ \underbar{18.0} \\ 17.2    \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 31.9         \\ \underbar{33.3} \\ 34.2    \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} \textbf{16.3}\\ \underbar{14.4} \\ 13.5    \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 29.4         \\ \underbar{31.9} \\ 32.6    \end{tabular}   \\ \cline{2-9}
			
			%\begin{tabular}[c]{@{}l@{}} SCR+FREQ+EMB \end{tabular}            &
			&
			\begin{tabular}[c]{@{}l@{}} 0.06 \\ 0.06 \\ 0.06 \end{tabular}   &
			\begin{tabular}[c]{@{}l@{}} 0.6  \\ \underbar{0.7}  \\ 0.8  \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 33.5 \\ \underbar{33.7} \\ 33.3 \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 60.6 \\ \underbar{60.0} \\ 59.3 \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 17.8 \\ \underbar{18.0} \\ 17.6 \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 34.3 \\ \underbar{33.3} \\ 33.0 \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 14.2 \\ \underbar{14.4} \\ 14.0 \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 32.0 \\ \underbar{31.9} \\ 30.6 \end{tabular}   \\ 
			\bottomrule
			%\cline{2-8}  
			%\hlinewd{1.0pt}                                                    
		\end{tabular}
	\end{adjustbox}
	\label{table:hyper_ablation}
\end{table}

==> tables/4_main_sgg_openimage.tex <==
\begin{table}[h]
    \centering
    %\caption{The Performances of Open Images Dataset. $\dagger$ denote results reproduced by \cite{li2021bipartite}. $\ast$ denotes the Bi-Level Resampling (BLS) \cite{li2021bipartite} is not applied for this model.}
    \caption{The Performances of Open Images Dataset. $\ast$ denote results reproduced by \citet{li2021bipartite}. SCR$\ssymbol{2}$ denotes SCR of FREQ+EMB.}
	\begin{adjustbox}{width=0.68\textwidth}
	\begin{tabular}{c c cc cc c}
		\toprule
		\multirow{2}{*}{\textbf{Dataset}}  & \multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{mR@50}} & \multirow{2}{*}{\textbf{R@50}} & \multicolumn{2}{c}{~~~\textbf{wmAP}} & \multirow{2}{*}{\textbf{score}$_\textbf{wtd}$}  \\ 
		\cline{5-6}
		& &  & & \textbf{rel} & \textbf{phr} & \\
		\midrule
		
		\multirow{5}{*}{V4} 
		& \multicolumn{1}{l}{RelDN \cite{zhang2019graphical}$^\ast$} & 70.40  & 75.66 & 36.13 & 39.91 & 45.21  \\
		& \multicolumn{1}{l}{GPS-Net \cite{lin2020gps}$^\ast$ }& 69.50  & 74.65 & 35.02 & 39.40 & 44.70  \\
		& \multicolumn{1}{l}{BGNN \cite{li2021bipartite}} & 72.11  & 75.46 & 37.76 & 41.70 & \textbf{46.87}  \\
		\cline{2-7}
		%& BGNN$^\ast$+SCR       &        &       &       &       &        \\
		& \multicolumn{1}{l}{\textbf{BGNN+SCR$\ssymbol{2}$ (ours)}}  & \textbf{72.20} &  \textbf{75.48}  &  \textbf{38.64}   &  \textbf{45.01} &  45.01       \\
		\midrule
		
		\multirow{8}{*}{V6} 
		& \multicolumn{1}{l}{RelDN \cite{zhang2019graphical}$^\ast$} & 33.98 & 73.08  & 32.16 & 33.39 & 40.84 \\
		& \multicolumn{1}{l}{VCTree \cite{tang2019learning}$^\ast$}  & 33.91 & 74.08  & 34.16 & 33.11 & 40.21 \\
		& \multicolumn{1}{l}{MOTIFS \cite{zellers2018neural}$^\ast$} & 32.68 & 71.63  & 29.91 & 31.59 & 38.93 \\
		& \multicolumn{1}{l}{TDE \cite{tang2020unbiased}$^\ast$}  & 35.47 & 69.30  & 30.74 & 32.80 & 39.27 \\
		& \multicolumn{1}{l}{GPS-Net \cite{lin2020gps}$^\ast$}  & 35.26 & 74.81  & 32.85 & 33.98 & 41.69 \\
		& \multicolumn{1}{l}{BGNN \cite{li2021bipartite}} & 40.45 & 74.98  & 33.51 & 34.15 & 42.06 \\
		\cline{2-7}
		%& BGNN$^\ast$+SCR       &       &        &       &       &       \\
		& \multicolumn{1}{l}{\textbf{BGNN+SCR$\ssymbol{2}$ (ours)}}   & \textbf{42.43} & \textbf{75.21} & \textbf{33.98} & \textbf{35.13} & \textbf{42.66}  \\
		
		\bottomrule
	\end{tabular}
\end{adjustbox}
\label{table:openimage}
\end{table}

==> tables/4_main_sgg_performances.tex <==
\begin{table*}[t]
	\center
    \caption{The SGG performances of Relationship Retrieval on mean Recall@K and Recall@K. SCR$\ssymbol{2}$ denotes SCR of FREQ+EMB. %The SGG models re-implemented under our codebase are denoted by the superscript$^{\ast}.$ 
    Note the \textcolor{red}{best} and \textcolor{blue}{second best} methods under each setting are marked according to format.}
    \small 
    \begin{adjustwidth}{-0.6\extralength}{0cm}
	\begin{adjustbox}{width=1.2\textwidth}
		\begin{tabularx}{\fulllength}{cccccccc}
			\toprule
			\multicolumn{2}{c}{} & \multicolumn{2}{c}{\textbf{PredCls}}& \multicolumn{2}{c}{\textbf{SGCls}} & \multicolumn{2}{c}{\textbf{SGDet}} \\ \midrule
			\multicolumn{2}{l}{Model} & mR@20/50/100 & R@20/50/100 & mR@20/50/100 & R@20/50/100 & mR@20/50/100 & R@20/50/100 \\ \midrule
   
			\multicolumn{2}{l}{IMP+ \cite{xu2017scene}} &  ~-.-/ ~9.8/10.5 & 52.7/59.3/61.3 & ~~-.-/~5.8/~6.0 & 31.7/34.6/35.4 & ~~-.-/~3.8/~4.8  & 14.6/20.7/24.5 \\
			\multicolumn{2}{l}{FREQ \cite{zellers2018neural}} &  ~8.3/13.0/16.0 & 53.6/60.6/62.2 & ~5.1/~7.2/~8.5 & 29.3/32.3/32.9 & ~4.5/~6.1/~7.1  & 20.1/26.2/30.1 \\
			\multicolumn{2}{l}{KERN \cite{chen2019knowledge}} &  ~~-.-/17.7/19.2 & ~~-.-/65.8/67.6  & ~~-.-/~9.4/10.0 & ~~-.-/36.7/37.4  & ~~-.-/~6.4/~7.3  & ~~-.-/27.1/29.8  \\
			\multicolumn{2}{l}{MOTIFS \cite{zellers2018neural}} & 10.8/14.0/15.3 & 58.5/65.2/67.1 & ~6.3/~7.7/~8.2 & 32.9/35.8/36.5 & ~4.2/~5.7/~6.6 & 21.4/27.2/30.3 \\
			\multicolumn{2}{l}{VCTree \cite{tang2019learning}} & 14.0/17.9/19.4 & 60.1/66.4/68.1 & ~8.2/10.1/10.8 & 35.2/38.1/38.8 & ~5.2/~6.9/~8.0 & 22.0/27.9/31.3 \\ \midrule \midrule 

            %\multicolumn{2}{l|}{Bipartite-Graph \cite{li2021bipartite}$^{\ast}$} & 13.3/17.0/18.7 & %\multicolumn{1}{l|}{56.5/63.6/65.6} & 7.2/9.1/9.9  & \multicolumn{1}{l|}{32.8/36.6/37.8} & 4.9/6.8/8.2  & 23.3/30.4/34.9 \\  
			%\multicolumn{2}{l|}{Bipartite-Graph \cite{li2021bipartite}+CogTree$^{\ast}$} & 23.4/29.4/31.8 & \multicolumn{2}{l|}{43.8/49.8/51.4} & 11.9/14.4/15.5  & \multicolumn{2}{l|}{25.6/28.8/29.8} & 6.9/9.6/11.6  & 16.8/22.7/26.4 \\

            \multicolumn{2}{l}{MSDN \cite{Li_2017_ICCV}} & ~~-.-/15.9/17.5 & ~~-.-/64.6/66.6 & ~~-.-/~~9.3/~~9.7  & ~~-.-/38.4/39.8 & ~-.-/~~6.1/~~7.2  & ~~-.-/31.9/36.6 \\

            \multicolumn{2}{l}{G-RCNN \cite{yang2018graph}} & ~~-.-/16.4/17.2 & ~~-.-/64.8/66.7 & ~~-.-/~~9.0/~~9.5  & ~~-.-/38.5/37.0 & ~-.-/~~5.8/~~6.6  & ~~-.-/29.7/32.8 \\
   
			\multicolumn{2}{l}{BGNN \cite{li2021bipartite}} & ~~-.-/30.4/32.9 & ~~-.-/59.2/61.3 & ~~-.-/14.3/16.5  & ~~-.-/37.4/38.5 & ~-.-/10.7/12.6  & ~~-.-/31.0/35.8 \\

            \multicolumn{2}{l}{DT2-ACBS \cite{desai2021learning}} & ~~-.-/35.9/39.7 & ~~-.-/23.3/25.6 & ~~-.-/24.8/27.5  & ~~-.-/16.2/17.6 & ~-.-/22.0/24.4  & ~~-.-/15.0/16.3\\
            
			
			%\multicolumn{2}{l}{BGNN$^{\ast}$ + \textbf{SCR} }& ~~~-~~/~~~-~~/~~~-~~ & ~~~-~~/~~~-~~/~~~-~~ & ~~~-~~/~~~-~~/~~~-~~  & ~~~-~~/~~~-~~/~~~-~~ & ~~~-~~/~~~-~~/~~~-~~  & ~~~-~~/~~~-~~/~~~-~~ \\
			
			%\multicolumn{2}{l}{\textbf{BGNN + SCR}$\ssymbol{2}$ (ours) }& \textbf{27.1}/\textbf{31.6}/\textbf{33.7} & 51.2/58.6/60.8 & \textbf{13.4}/\textbf{15.8}/\textbf{16.9}  & 29.3/33.3/34.7 & \textbf{8.8}/\textbf{11.6}/\textbf{13.5}  & 21.0/27.9/32.4 \\
			
			%\multicolumn{1}{l|}{Bipartite-Graph + SCR$\ssymbol{2}$ (ours)}  & \textbf{26.0}/\textbf{31.5}/\textbf{33.8} & \multicolumn{1}{l|}{50.3/57.4/60.0} & \textbf{13.6}/\textbf{16.3}/\textbf{17.2}  & \multicolumn{1}{l|}{28.5/32.3/33.6} & \textbf{8.1}/\textbf{11.3}/\textbf{13.3} & 20.9/27.9/32.4 \\
            \midrule 

            % --------- MOTIFS ---------
			\multicolumn{2}{l}{MOTIFS \cite{zellers2018neural} } & 11.5/14.6/15.8 & \textcolor{red}{59.5}/\textcolor{red}{66.0}/\textcolor{red}{67.9} & ~6.5/~8.0/~8.5 & \textcolor{red}{35.8}/\textcolor{red}{39.1}/\textcolor{red}{39.9} & ~4.1/~5.5/~6.8  & \textcolor{red}{25.1}/\textcolor{red}{32.1}/\textcolor{red}{36.9} \\
			%\multicolumn{2}{l}{MOTIFS + Focal} & 10.9/13.9/15.0 & 59.2/65.8/67.7 & 6.3/7.7/8.3    & 36.0/39.3/40.1 & 3.9/5.3/6.6  & 24.7/31.7/36.7 \\
			%\multicolumn{2}{l}{~ + Reweight \cite{tang2020unbiased}} & 16.0/20.0/21.9 & 45.4/57.0/61.7 & 8.4/10.1/10.9 & 24.2/29.5/31.5 & 6.5/8.4/9.8 & 18.3/24.4/29.3 \\
			%\multicolumn{2}{l|}{MOTIFS + Resample}    & 14.7/18.5/20.0 & 57.6/64.6/66.7 & 9.1/11.0/11.8  & 34.5/37.9/38.8 & 5.9/8.2/9.7  & 23.2/30.5/35.4 \\
			\multicolumn{2}{l}{~ + TDE \cite{tang2020unbiased}} & 18.5/25.5/29.1 & 33.6/46.2/51.4 & ~9.8/13.1/14.9  & 21.7/27.7/29.9 & ~5.8/~8.2/~9.8  & 12.4/16.9/20.3 \\

            \multicolumn{2}{l}{~ + PCPL \cite{yan2020pcpl}}& ~~~-.-/24.3/26.1 & ~~~-.-/54.7/56.5 & ~~~-.-/12.0/12.7 & ~~~-.-/\textcolor{blue}{35.3}/\textcolor{blue}{36.1} & ~~-.-/10.7/12.6 & ~~~-.-/27.8/31.7 \\
            
			\multicolumn{2}{l}{~ + CogTree \cite{yu2020cogtree}}& 20.9/26.4/29.0 & 31.1/35.6/36.8 & 12.1/14.9/16.1 & 19.4/21.6/22.2 & 7.9/10.4/11.8 & 15.7/20.0/22.1 \\

            \multicolumn{2}{l}{~ + DLFE \cite{chiou2021recovering}}& 22.1/26.9/28.8 & ~~~-.-/52.5/54.2 & 12.8/15.2/15.9 & ~~~-.-/32.3/33.1 & 8.6/11.7/13.8 & ~~~-.-/25.4/29.4 \\

            \multicolumn{2}{l}{~ + BPL-SA \cite{guo2021general}}& \textcolor{blue}{24.8}/29.7/31.7 & ~~~-.-/50.7/52.5 & \textcolor{blue}{14.0}/16.5/17.5 & ~~~-.-/30.1/31.0 & \textcolor{red}{10.7}/13.5/15.6 & ~~~-.-/23.0/26.9 \\
            
			%\multicolumn{2}{c}{MOTIFS + CogTree \cite{yu2020cogtree}$^{\ast}$}& 21.5/26.9/29.5 & 44.3/49.5/50.8 & 11.9/14.3/15.7 & 26.5/29.4/30.3 & 7.2/10.3/12.4& 18.6/24.6/28.2 \

            \multicolumn{2}{l}{~ + PPDL \cite{li2022ppdl}}& ~~~-.-/\textcolor{red}{32.2}/\textcolor{blue}{33.3} & ~~~-.-/47.2/47.6 & ~~~-.-/\textcolor{red}{17.5}/18.2 & ~~~-.-/28.4/29.3 & ~~-.-/11.4/13.5& ~~~-.-/21.2/23.9 \\  

            \multicolumn{2}{l}{~ + NICE \cite{li2022devil}}& ~~~-.-/29.9/32.3 & ~~~-.-/55.1/57.2 & ~~~-.-/16.6/17.9 & ~~~-.-/33.1/34.0 & ~~-.-/12.2/14.4& ~~~-.-/\textcolor{blue}{27.8}/\textcolor{blue}{31.8} \\ 
            
			%\multicolumn{2}{l}{\textbf{~ + SCR}$\ssymbol{2}$ (ours)} & \textcolor{red}{25.6}/\textcolor{blue}{31.1}/\textcolor{blue}{33.2}& \textcolor{blue}{51.2}/\textcolor{blue}{58.2}/\textcolor{blue}{60.3} & \textcolor{red}{14.2}/\textcolor{blue}{17.1}/\textcolor{red}{18.2} & \textcolor{blue}{27.1}/31.0/32.3 & ~\textcolor{blue}{9.6}/\textcolor{red}{13.5}/\textcolor{red}{15.9} & \textcolor{blue}{18.1}/25.1/29.5  \\ \midrule

            \multicolumn{2}{l}{\textbf{~ + SCR$\ssymbol{2}$ (ours)}} & \textcolor{red}{25.9}/\textcolor{blue}{31.5}/\textcolor{red}{33.6}& \textcolor{blue}{51.0}/\textcolor{blue}{57.9}/\textcolor{blue}{60.1} & \textcolor{red}{14.2}/\textcolor{blue}{17.1}/\textcolor{red}{18.2} & \textcolor{blue}{27.1}/31.0/32.3 & ~\textcolor{blue}{9.6}/\textcolor{red}{13.5}/\textcolor{red}{15.9} & \textcolor{blue}{18.1}/25.1/29.5  \\ \midrule

            % --------- VCTree---------
			\multicolumn{2}{l}{VCTree \cite{tang2019learning} }         & 11.7/14.9/16.1 & \multicolumn{1}{l}{\textcolor{red}{59.8}/\textcolor{red}{66.2}/\textcolor{red}{68.1}} & ~6.2/~7.5/~7.9    & \multicolumn{1}{l}{\textcolor{red}{37.0}/\textcolor{blue}{40.5}/\textcolor{blue}{41.4}} & ~4.2/~5.7/~6.9  & \textcolor{red}{24.7}/\textcolor{red}{31.5}/\textcolor{red}{36.2} \\
			\multicolumn{2}{l}{~ + TDE \cite{tang2020unbiased}}            & 18.4/25.4/28.7 & \multicolumn{1}{l}{36.2/47.2/51.6} & ~8.9/12.2/14.0  & \multicolumn{1}{l}{19.9/25.4/27.9} & ~6.9/~9.3/11.1 & 14.0/19.4/23.2 \\

            \multicolumn{2}{l}{~ + PCPL \cite{yan2020pcpl}}& ~~~-.-/22.8/24.5 & ~~~-.-/\textcolor{blue}{56.9}/\textcolor{blue}{58.7} & ~~~-.-/15.2/16.1 & ~~~-.-/\textcolor{red}{40.6}/\textcolor{red}{41.7} & ~-.-/10.8/12.6 & ~~~-.-/26.6/30.3 \\
            
			\multicolumn{2}{l}{~ + CogTree \cite{yu2020cogtree}}     & 22.0/27.6/29.7 & \multicolumn{1}{l}{39.0/44.0/45.4} & 15.4/18.8/19.9 & \multicolumn{1}{l}{\textcolor{blue}{27.8}/30.9/31.7} & 7.8/10.4/12.1& 14.0/18.2/20.4 \\

            \multicolumn{2}{l}{~ + DLFE \cite{chiou2021recovering}}& 20.8/25.3/27.1 & ~~~-.-/51.8/53.5 & 15.8/18.9/20.0 & ~~~-.-/33.5/34.6 & 8.6/11.8/13.8 & ~~~-.-/22.7/26.3 \\

            \multicolumn{2}{l}{~ + BPL-SA \cite{guo2021general}}& \textcolor{blue}{26.2}/30.6/32.6 & ~~~-.-/50.0/51.8 & \textcolor{red}{17.2}/\textcolor{red}{20.1}/\textcolor{red}{21.2} & ~~~-.-/34.0/35.0 & \textcolor{red}{10.6}/\textcolor{blue}{13.5}/\textcolor{blue}{15.7} & ~~~-.-/21.7/25.5 \\
   
			%\multicolumn{1}{l|}{VCTree + CogTree \cite{yu2020cogtree}$^{\ast}$}     & 22.7/28.6/30.9 & \multicolumn{1}{l|}{45.9/51.2/52.6} & 13.1/15.7/16.9 & \multicolumn{1}{l|}{27.2/30.1/30.9} & 7.4/10.1/12.2& 17.1/23.0/26.8 \\
            \multicolumn{2}{l}{~ + PPDL \cite{li2022ppdl}}& ~~~-.-/\textcolor{blue}{33.3}/\textcolor{blue}{33.8} & ~~~-.-/47.6/48.0 & ~~~-.-/14.3/15.7 & ~~~-.-/32.1/33.0 & ~~-.-/11.3/13.3& ~~~-.-/20.1/22.9 \\  

            \multicolumn{2}{l}{~ + NICE \cite{li2022devil}}& ~~~-.-/30.7/33.0 & ~~~-.-/55.0/56.9 & ~~~-.-/\textcolor{blue}{19.9}/\textcolor{blue}{21.3} & ~~~-.-/37.8/39.0 & ~~-.-/11.9/14.1& ~~-.-/\textcolor{blue}{27.0}/\textcolor{blue}{30.8} \\ 
               
			%\multicolumn{2}{l}{~ + \textbf{SCR}$\ssymbol{2}$ (ours)} & \textcolor{blue}{26.4}/\textcolor{blue}{31.5}/\textcolor{blue}{33.7} & \multicolumn{1}{l}{\textcolor{blue}{51.3}/\textcolor{blue}{58.0}/\textcolor{blue}{60.0}} & 14.1/16.9/18.0 & \multicolumn{1}{l}{28.1/32.0/33.3}  &  ~\textcolor{blue}{8.7}/\textcolor{blue}{12.0}/\textcolor{blue}{14.4} & \multicolumn{1}{l}{\textcolor{blue}{19.7}/\textcolor{blue}{27.3}/\textcolor{blue}{31.9}} \\ \midrule

            \multicolumn{2}{l}{~ + \textbf{SCR$\ssymbol{2}$ (ours)}} & \textcolor{red}{27.7}/\textcolor{red}{33.5}/\textcolor{red}{35.5} & \multicolumn{1}{l}{\textcolor{blue}{49.7}/\textcolor{black}{56.4}/\textcolor{black}{58.3}} & 15.4/18.9/20.1 & \multicolumn{1}{l}{26.7/30.6/31.9}  &  \textcolor{blue}{10.3}/\textcolor{red}{13.8}/\textcolor{red}{16.3} & \multicolumn{1}{l}{\textcolor{blue}{18.1}/25.0/29.4} \\ \midrule
   

            % --------- SG-Transformer ---------
			\multicolumn{2}{l}{SG-Transformer \cite{yu2020cogtree}}  & 14.8/19.2/20.5 & \multicolumn{1}{l}{\textcolor{red}{58.5}/\textcolor{red}{65.0}/\textcolor{red}{66.7}} & ~8.9/11.6/12.6  & \multicolumn{1}{l}{\textcolor{red}{35.6}/\textcolor{red}{38.9}/\textcolor{red}{39.8}} & ~5.6/~7.7/~9.0  & \textcolor{red}{24.0}/\textcolor{red}{30.3}/\textcolor{red}{33.3} \\
			\multicolumn{2}{l}{~ + CogTree\cite{yu2020cogtree}} & \textcolor{blue}{22.9}/\textcolor{blue}{28.4}/\textcolor{blue}{31.0} & \multicolumn{1}{l}{34.1/38.4/39.7} & \textcolor{blue}{13.0}/\textcolor{blue}{15.7}/\textcolor{blue}{16.7} & 20.8/22.9/23.4 & ~\textcolor{blue}{7.9}/\textcolor{blue}{11.1}/\textcolor{blue}{12.7} & 15.1/19.5/21.7 \\
			%\multicolumn{1}{l|}{SG-Transformer + CogTree\cite{yu2020cogtree}$^{\ast}$} & 21.8/27.3/29.6 & \multicolumn{1}{l|}{45.9/51.6/53.3} & 12.5/15.5/16.5 & \multicolumn{1}{l|}{25.9/28.9/29.6} & 7.8/11.0/12.5& 18.2/21.2/25.3 \\
   
			\multicolumn{2}{l}{\textbf{~ + SCR$\ssymbol{2}$ (ours)}} & \textcolor{red}{27.0}/\textcolor{red}{32.2}/\textcolor{red}{34.5} & \textcolor{blue}{45.3}/\textcolor{blue}{52.7}/\textcolor{blue}{55.0} & \textcolor{red}{14.9}/\textcolor{red}{17.7}/\textcolor{red}{18.7}  & \textcolor{blue}{25.1}/\textcolor{blue}{28.9}/\textcolor{blue}{30.2} & \textcolor{red}{10.4} /\textcolor{red}{13.4}/\textcolor{red}{15.0}  & \textcolor{blue}{17.7}/\textcolor{blue}{23.2}/\textcolor{blue}{26.2}   \\ 
            \midrule 
			\bottomrule 
		\end{tabularx}
	\end{adjustbox}
    \end{adjustwidth}
	\label{table:m_recall}
\end{table*}
%\vspace{-0.1cm}

==> tables/4_main_sgg_zeroshot.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[hptb]
	\scriptsize
	\center
    \caption{The SGG Performances of Zero-shot Relationship Retrieval on Recall@K. SCR$\ssymbol{2}$ denotes SCR of FREQ+EMB. The SGG models re-implemented under our codebase are denoted by the superscript$^{\ast}.$}
	\begin{adjustbox}{width=0.88\textwidth}
		\begin{tabular}{c c cc cc cc}
			%\hlinewd{1.0pt}
			%\hlinewd{1.0pt}
			\toprule
			\multicolumn{2}{c}{\textbf{Zero-Shot Relationship Retrieval}} & 
			\multicolumn{2}{c}{\textbf{PredCls}} & \multicolumn{2}{c}{\textbf{SGCls}} & 
			\multicolumn{2}{c}{\textbf{SGDet}}  \\ \hline
			Model  & Method                                      
			& R@50 & R@100                                                     
			& R@50 & R@100                                                   
			& R@50 & R@100   \\ \midrule
			
			%\multirow{5}{*}{MOTIFS \cite{tang2020unbiased}} &
			%\begin{tabular}[c]{@{}l@{}}  MOTIFS\\ \cite{tang2020unbiased} \end{tabular} & 
			%& Baseline                                                            
			%& 10.9  & 14.5                                                      
			%&  2.2  &  3.0                                                     
			%&  0.1  &  0.2   \\ \cline{2-8} 
			
			%\begin{tabular}[c]{@{}l@{}} MOTIFS \\ \cite{tang2020unbiased} \end{tabular}& 
			%\begin{tabular}[c]{@{}l@{}}Focal\\ Reweight\\ Resample \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}}10.9\\ 0.7\\ 11.1 \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}}14.4\\ 0.9\\ 14.3 \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}} 2.2\\ 0.1\\  2.3 \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}} 3.1\\ 0.1\\  3.1 \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}} 0.1\\ 0.0\\  0.1 \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}} 0.3\\ 0.0\\  0.3 \end{tabular} \\ \cline{2-8}
			
			%\begin{tabular}[c]{@{}l@{}} MOTIFS \\ \cite{tang2020unbiased} \end{tabular}& 
			%\begin{tabular}[c]{@{}l@{}}Focal\\ Reweight \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}}10.9\\ 0.7 \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}}14.4\\ 0.9 \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}} 2.2\\ 0.1 \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}} 3.1\\ 0.1 \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}} 0.1\\ 0.0 \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}} 0.3\\ 0.0 \end{tabular} \\ \cline{2-8} 
			
			%MOTIFS \\ \cite{tang2020unbiased} & 
			\begin{tabular}[c]{@{}l@{}} MOTIFS  \cite{tang2020unbiased} \end{tabular}&
			\begin{tabular}[c]{@{}l@{}} baseline \cite{tang2020unbiased} \\ Reweight \cite{tang2020unbiased} \\ TDE \cite{tang2020unbiased} \\ CogTree \cite{yu2020cogtree}$^{\ast}$  \\ \textbf{SCR$\ssymbol{2}$ (ours)} \end{tabular}    & 
			\begin{tabular}[c]{@{}l@{}} 10.9 \\ 0.7 \\ 14.4 \\ 2.4 \\ \textbf{18.0} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 14.5 \\ 0.9 \\ 18.2 \\ 4.0 \\ \textbf{21.1} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 2.2 \\ 0.1 \\ 3.4 \\ 0.9 \\ \textbf{5.1}  \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 3.0 \\ 0.1 \\ 4.5 \\ 1.5 \\ \textbf{5.9}  \end{tabular}   &
			\begin{tabular}[c]{@{}l@{}} 0.1 \\ 0.0 \\ 2.3 \\ 0.3 \\ \textbf{2.4}  \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 0.2 \\ 0.0 \\ 2.9 \\ 0.6 \\ \textbf{3.8}  \end{tabular} \\ \midrule 
			
			%\multirow{2}{*}{VTransE \cite{tang2020unbiased}}        & 
			%\begin{tabular}[c]{@{}l@{}}Baseline\\ TDE\end{tabular}  & 
			%\begin{tabular}[c]{@{}l@{}}11.2\\ 13.3\end{tabular}     & 
			%\begin{tabular}[c]{@{}l@{}}14.7\\ 17.6\end{tabular}     & 
			%\begin{tabular}[c]{@{}l@{}} 2.5\\  2.9\end{tabular}     & 
			%\begin{tabular}[c]{@{}l@{}} 3.3\\  3.8\end{tabular}     & 
			%\begin{tabular}[c]{@{}l@{}} 0.8\\  2.0\end{tabular}     & 
			%\begin{tabular}[c]{@{}l@{}} 1.5\\  2.7\end{tabular}     \\ \hline %\cline{2-8} 
			
			%\multirow{2}{*}{VCTree \cite{tang2020unbiased}}         &
			\begin{tabular}[c]{@{}l@{}} VCTree   \cite{tang2020unbiased} \end{tabular} & 
			\begin{tabular}[c]{@{}l@{}}Baseline \cite{tang2020unbiased} \\ TDE \cite{tang2020unbiased} \\ CogTree \cite{yu2020cogtree}$^{\ast}$ \\ \textbf{SCR$\ssymbol{2}$ (ours)} \end{tabular} & 
			\begin{tabular}[c]{@{}l@{}}10.8\\ 14.3 \\ 3.3 \\ \textbf{17.6} \end{tabular}     & 
			\begin{tabular}[c]{@{}l@{}}14.3\\ 17.6 \\ 5.0 \\ \textbf{20.4} \end{tabular}     & 
			\begin{tabular}[c]{@{}l@{}} 1.9\\  3.2 \\ 2.1 \\ \textbf{4.5} \end{tabular}     & 
			\begin{tabular}[c]{@{}l@{}} 2.6\\  4.0 \\ 2.6 \\ \textbf{5.2} \end{tabular}     & 
			\begin{tabular}[c]{@{}l@{}} 0.2\\  2.6 \\ 0.4 \\ \textbf{2.5} \end{tabular}     & 
			\begin{tabular}[c]{@{}l@{}} 0.7\\  3.2 \\ 0.6 \\ \textbf{3.5} \end{tabular}     \\ \midrule 
			
			
			%\multirow{2}{*}{SG-Transformer \cite{yu2020cogtree}}         & 
			\begin{tabular}[c]{@{}l@{}} SG-Transformer  \cite{yu2020cogtree}$^{\ast}$ \end{tabular} &
			\begin{tabular}[c]{@{}l@{}}Baseline$^{\ast}$ \\ CogTree \cite{yu2020cogtree}$^{\ast}$ \\ \textbf{SCR$\ssymbol{2}$ (ours)} \end{tabular} & 
			\begin{tabular}[c]{@{}l@{}} 4.1 \\ 5.2\\ \textbf{16.4} \end{tabular}  & 
			\begin{tabular}[c]{@{}l@{}} 6.3 \\ 7.3\\ \textbf{19.6} \end{tabular}  & 
			\begin{tabular}[c]{@{}l@{}} 1.6 \\ 2.3\\ \textbf{4.6} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 2.3 \\ 3.0\\ \textbf{5.3} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 0.2 \\ 0.3\\ \textbf{2.0} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 0.5 \\ 0.5\\ \textbf{3.2} \end{tabular}   \\ \midrule
			
			
			%\multirow{2}{*}{Bipartite-Graph \cite{li2021bipartite}}         & 
			\begin{tabular}[c]{@{}l@{}} BGNN  \cite{li2021bipartite} \end{tabular} &
			\begin{tabular}[c]{@{}l@{}}BGNN$^{\ast}$ \\ CogTree \cite{yu2020cogtree}$^{\ast}$ \\ \textbf{SCR$\ssymbol{2}$ (ours)} \end{tabular} & 
			\begin{tabular}[c]{@{}l@{}} 15.0 \\ 13.4 \\ \textbf{16.3} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}} 18.0 \\ 16.1 \\ \textbf{19.5} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}}  4.5 \\ 5.0  \\  \textbf{4.9} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}}  5.4 \\ 5.7  \\  \textbf{5.9} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}}  4.5 \\ 0.5  \\  \textbf{1.9} \end{tabular}   & 
			\begin{tabular}[c]{@{}l@{}}  5.3 \\ 0.8  \\  \textbf{3.0} \end{tabular}   \\ 
			\bottomrule
			
			%\multirow{2}{*}{Bipartite-Graph \cite{li2021bipartite}}         & 
			%\begin{tabular}[c]{@{}l@{}} Bipartite-Graph \\ \cite{li2021bipartite} \end{tabular} &
			%\begin{tabular}[c]{@{}l@{}}Baseline$^{\ast}$ \\ CogTree \cite{yu2020cogtree}$^{\ast}$ \\ SCR$\ssymbol{2}$ (ours) \end{tabular} & 
			%\begin{tabular}[c]{@{}l@{}} 15.0 \\ 13.4 \\ \textbf{16.3} \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}} 18.0 \\ 16.1 \\ \textbf{19.5} \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}}  4.5 \\ 5.0  \\  \textbf{4.9} \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}}  5.4 \\ 5.7  \\  \textbf{5.9} \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}}  4.5 \\ 0.5  \\  \textbf{1.9} \end{tabular}   & 
			%\begin{tabular}[c]{@{}l@{}}  5.3 \\ 0.8  \\  \textbf{3.0} \end{tabular}   \\ \hline
			%\cline{2-8}  
			%\hlinewd{1.0pt}                                                    
		\end{tabular}
	\end{adjustbox}
	\label{table:zero_shot}
\end{table}
